Toward Operationalizing Pipeline-aware ML Fairness: A Research Agenda for Developing Practical Guidelines and Tools

While algorithmic fairness is a thriving area of research, in practice, mitigating issues of bias often gets reduced to enforcing an arbitrarily chosen fairness metric, either by enforcing fairness constraints during the optimization step, post-processing model outputs, or by manipulating the training data. Recent work has called on the ML community to take a more holistic approach to tackle fairness issues by systematically investigating the many design choices made through the ML pipeline, and identifying interventions that target the issue's root cause, as opposed to its symptoms. While we share the conviction that this pipeline-based approach is the most appropriate for combating algorithmic unfairness on the ground, we believe there are currently very few methods of \emph{operationalizing} this approach in practice. Drawing on our experience as educators and practitioners, we first demonstrate that without clear guidelines and toolkits, even individuals with specialized ML knowledge find it challenging to hypothesize how various design choices influence model behavior. We then consult the fair-ML literature to understand the progress to date toward operationalizing the pipeline-aware approach: we systematically collect and organize the prior work that attempts to detect, measure, and mitigate various sources of unfairness through the ML pipeline. We utilize this extensive categorization of previous contributions to sketch a research agenda for the community. We hope this work serves as the stepping stone toward a more comprehensive set of resources for ML researchers, practitioners, and students interested in exploring, designing, and testing pipeline-oriented approaches to algorithmic fairness.

==> intro.tex <==
\section{Introduction} 

%As AI systems proliferate in socially high-stakes domains, concerns around balancing their potential for benefiting society versus harming already marginalized and underserved communities have been mounting~\cite{dastin2018amazon,obermeyer2019dissecting,buolamwini2018gender,compas}. 
Through years of work by a variety of stakeholder groups, including activists, journalists, lawmakers, researchers, and AI practitioners, we now witness a growing appetite for building high-stakes AI systems with harm prevention in mind~\cite{room2021executive,jobin2019global}. 
Aside from the rising public pressure on technology companies and governments to create more equitable systems, recent legal developments, such as those from the Federal Trade Commission (FTC)~\cite{ftcproposed}, the White House~\cite{house2022blueprint,room2021executive} and various other agencies~\cite{ai2023artificial} suggest an uptick in enforcement surrounding discriminatory algorithms. These recent movements give a point of leverage for technologically equipped activists and plaintiffs to challenge discriminatory algorithms and further incentivize companies to thoroughly explore the space of possible algorithms to find the least discriminatory one within those with sufficient business utility. %Against this backdrop, we believe it is increasingly imperative to operationalize a pipeline-based approach by constructing and validating practical tools and resources for bias detection and mitigation. 
As a result, professionals across industry, government, and nonprofits have been turning to algorithmic fairness expertise to guide their implementation of AI systems~\cite{holstein2019improving}. 
%



\begin{figure}
    \centering
    %\includegraphics[scale=0.5]{pics/base_pipeline.png}
    \includegraphics[width=\textwidth]{pics/pipeline_redone.png}
    
    \caption{A simplified view of the ML pipeline, its key stages, and instances of design choices made at each stage.}
    \label{fig:pipeline}
\end{figure}

\xhdr{The pipeline-aware approach to algorithmic fairness.}
While there has been extensive work in the service of preventing algorithmic unfairness~\cite{pessach2022review,agarwal2018reductions,hardt2016equality,petersenneurips21,kamiran2012data}, mitigation in practice often gets reduced to enforcing a somewhat arbitrarily formulated fairness metric on top of a pre-developed or deployed system~\cite{madaio2020co}. 
Practitioners often make ad-hoc mitigation choices to improve fairness metrics, such as removing sensitive attributes, changing the data distribution, 
%training with synthetic data, 
enforcing fairness constraints, or post-processing model predictions. While these techniques may improve selected fairness metrics, they often have little practical impact; at worst, they can even exacerbate the same disparity metrics they aim to alleviate~\cite{wang2021fair,li2022more}. 
Prior scholarship has attributed these problematic trends to the fact that the traditional approach to fairness fails to take a system-wide view of the problem. They narrow bias mitigation to a restricted set of points along the ML pipeline (e.g., the choice of optimization function). This is despite the well-established fact that \emph{numerous} choices there can impact the model's behavior~\citep{suresh2021framework}. Assessing viability/functionality of AI~\citep{raji2022fallacy}, problem formulation~\cite{passi2019problem}, data collection, data pre-processing, %statistical
modeling, testing and validation, and organizational integration are all key stages of the ML pipeline consisting of consequential design choices (see Figure~\ref{fig:pipeline} for an overview).
By abstracting away the ML pipeline and selecting an ad-hoc mitigation strategy, the mainstream approach misses the opportunity to identify, isolate, and mitigate the underlying \emph{sources} of unfairness, which can in turn lead to fairness-accuracy tradeoffs due to intervening at the wrong place~\cite{black2022algorithmic},  
or even worse,``[hide] the real problem while creating an illusion of
fairness''~\cite{akpinar2022sandbox}. 
%This work heeds the growing calls to take a \emph{pipeline-aware} approach to fairness~\cite{akpinar2022sandbox,suresh2021framework}. 
 We join prior calls advocating for an alternate \emph{pipeline-aware} approach to fairness~\cite{akpinar2022sandbox,suresh2021framework}.
At a high level, this approach works as follows: given a model with undesirable fairness behavior, the ML team must search for ways in which the variety of choices made across the ML creation pipeline may have contributed to the behavior (e.g., the choice of prediction target~\cite{obermeyer2019dissecting}). Once plausible causes are identified, the team should evaluate whether other choices could abate the problem (e.g. changing a model's prediction target and re-training~\cite{black2022algorithmic}).\footnote{This description is taking an auditing perspective: when building a fair model from scratch, fairness desiderata would be described, and the practitioners would enumerate choices that can be made at each step of the ML creation pipeline and avoid choices that work against this desired behavior.} This process should take place iteratively, and the model should be re-evaluated until it is deemed satisfactory, whereupon bias testing and model updates would continue throughout deployment.

\xhdr{The need for operationalizing the pipeline-aware approach} While prior work has clearly established the benefits of the pipeline-aware view toward fairness, we contend that \emph{conceptual awareness} of this approach alone won't be sufficient for \emph{operationalizing} it in practice. In Section~\ref{sec:challeneges}, we provide evidence suggesting that making informed hypotheses about the root causes of unfairness in the ML pipeline is a challenging task, even for individuals with specialized ML knowledge and skills. For example, based on qualitative data gathered from a graduate-level fair-ML class at an R1 institution, students with significant ML background struggle to conceptualize sources of harmful model behavior and suggest appropriately chosen bias mitigation strategies. This observation is, indeed, consistent with our experience working with ML practitioners and system developers across a wide range of public policy settings.
This evidence motivates our focus on ``operationalization'':
to \emph{find} less discriminatory models, we argue that practitioners need usable tools to measure the discrimination from, identify the underlying sources of, unfairness in the pipeline, and then match those underlying sources with appropriately designed interventions. 


Such tools would be instrumental in taking advantage of the legal systems already in place to reduce discrimination---such as the disparate impact doctrine, which requires searching for mod

es for ``Less Discriminatory Alternative'' models (LDAs) to establish ---one of the first publicized instances of which was recently conducted to replace a discriminatory credit allocation system at the private lending platform, Upstart~\cite{naacp_statement}. A practical toolkit can significantly expand the space of methods currently in use~\cite{colfax2021report2}, and offer additional points of interventions earlier in the pipeline, which can in turn ease legal concern over the use of protected attributes during training and deployment~\cite{colfax2021report1,colfax2021report2}. %In addition, a growing number of scholars~\cite{black2022model,akpinar2022sandbox,suresh2021framework} suggest a pipeline-based approach will be the most effective method of finding less discriminatory models in practice by interrogating the pipeline to find the most effective places to search for interventions--however, to our knowledge, no tools to instantiate such an approach currently exist.

\begin{figure}
    \centering
    %\includegraphics[scale=0.5]{pics/base_pipeline.png}
    % \includegraphics[width=0.75\textwidth]{pics/Screenshot 2023-05-10 at 2.37.27 AM.png}
    \includegraphics[width=\textwidth]{pics/papers_vs_stages (2).pdf}
    \vspace{-2.5em}
    \caption{The distribution of research efforts dedicated to different stages of the ML pipeline among the papers we surveyed.}
    \label{fig:distribution}
\end{figure}


\xhdr{A snapshot of progress toward operationalization.} Having established the need for practical implementation of the pipeline-aware approach to fairness, we seek to understand the progress made so far, and ask: how far along are we toward operationalizing the pipeline-aware approach? Do we currently have useful methods and guidelines to inspect and modify the variety of design choices made throughout the ML pipeline in practice? To respond to these questions, we consult the literature on algorithmic fairness in search of methods that identify, measure, or mitigate biases arising from specific ML design choices. Through an extensive survey of the Fair-ML literature, we collect and synthesize existing pipeline-aware fairness work and map them to specific stages of the pipeline (Section~\ref{sec:litreview}). While we identify numerous gaps in the existing arsenal of tools, we hope the resource we have curated offers practitioners a one-stop shop for identifying potential causes of unfairness in their use cases and getting an overview of the state of the art to detect, measure, and mitigate those issues. In the near future, our goal is to turn this catalog into a comprehensive, interactive, and community-maintained set of resources and tools for Fair-ML researchers, practitioners, and students interested in exploring, designing, and testing system-level approaches to algorithmic fairness.


\xhdr{Sketching a path forward for the research community.}
Figure~\ref{fig:distribution} depicts the relative effort the research community has allocated to different stages of the ML pipeline. As evident in this picture, the focus of the ML community has been largely on the statistical modeling stage, with an out-sized emphasis on mitigation strategies. 
This finding generalizes recent observations that ``Everyone wants to do the model work, not the data work''~\citep{sambasivan2021everyone}. 
Key stages of the pipeline, including viability assessment, problem formulation, and deployment and monitoring, have been understudied---we hypothesize due to lack of potential for novel, quantitative contributions or theoretical analysis~\citep{birhane2021values}. Moreover, we observe that the majority of algorithmic mitigation techniques are left at the proof-of-concept level and are not backed by any application-grounded evaluation of usability and utility. While the HCI community has made significant progress toward documenting the challenges and needs of ML practitioners, very few contributions investigate to use of specific measures and methods to meet these needs. To amplify their impact, we call on the ML and HCI research communities to invest in collaborations aimed at identifying, assessing, and improving concrete tools and guidelines for fairness. We contend that the ML pipeline is a complex system; understanding the interactions between various design choices in this system is a challenging task yet a potentially impactful avenue for quantitative analysis. Lastly, we acknowledge that practitioners often face choices between imperfect alternatives, each leading to its unique problematic consequences---developing normative guidelines to weigh these imperfect choices against each other is a crucial avenue for collaboration between ML experts and ethicists.

% lays out a research agenda outlining the gaps in the existing body of work, calling on the Fair-ML research community to develop contextual processes and methods to support practitioners throughout the process of designing, developing, and deploying their systems (Section~\ref{sec:agenda}). 


==> operationalize.tex <==
\section{The Need to Operationalize the Pipeline-Aware Approach}
\label{sec:challeneges}
We draw on our experience working with Machine Learning students and practitioners, and recent examples of enforcing anti-discrimination law to highlight the difficulty in, and necessity for, \emph{operationalizing} a pipeline-aware approach to fairness. 
In Section~\ref{sec:regulation}, we discuss a recent case study of legal pressure leading to a search for a less discriminatory alternative algorithm in the credit context. We show how operationalizing a pipeline-aware approach to fairness is essential to expand the set of levers auditors have available 
%to search for less discriminatory models in order 
to take advantage of legal tools such as the disparate impact framework--especially as existing mitigation techniques run the risk of violating existing legal restrictions on the use of protected attributes. Despite this need, we observe in Section~\ref{sec:teaching_evidence} that a conceptual understanding of the pipeline and the variety of choices within it are by no means sufficient to inform good practice. Even well-informed students struggle to correctly hypothesize about the underlying causes of unfairness and suggest plausible remedies. 
%Moreover, existing mitigation techniques run the risk of violating existing legal restrictions on the use of protected attributes, so it is essential to expand the set of levers auditors have available to search for less discriminatory models. 

\subsection{Evidence from Regulatory Enforcement}\label{sec:regulation}
Recent developments in attempts to regulate the design and use of  ML systems have given a sense of urgency to support regulators and policymakers in these efforts~\cite{ai2023artificial,house2022blueprint,room2021executive,ftcANPR2023}. 
In this section, we focus on one of the first examples of enforcement of anti-discrimination law in AI systems~\cite{colfax2021report1} to show how a pipeline-aware approach may be particularly helpful in establishing legal liability in, and providing remedies for, discrimination in regulated AI systems. 

In particular, we note that when searching for less discriminatory alternatives to deployed models, a pipeline-aware approach may elide some of the potential legal problems that apply to using more traditional algorithmic fairness approaches~\cite{ho2020affirmative, bent2019algorithmic}. Many traditional algorithmic fairness techniques that intervene at the modeling stage often use protected attributes to change model behavior by learning new prediction thresholds or modifying the training procedure~\cite{agarwal2018reductions,hardt2016equality}, leading regulators to dismiss such approaches due to legal restrictions around the use of protected attributes in decision-making~\cite{ho2020affirmative, bent2019algorithmic}. However, pipeline-aware techniques may use protected attribute labels to \emph{evaluate} different models and choose among them, but may not directly enforce a constraint using protected attributes, avoiding the same legal scrutiny applied to other algorithmic fairness techniques.
%, and become more widely adopted by the regulatory community. 
Thus, it is imperative that we build pipeline-aware tools to empower regulators, policymakers, and advocacy groups pushing for legal requirements surrounding bias reduction in public-facing AI systems to find, and enforce the use of, less discriminatory systems.

\xhdr{Case Study Background: Upstart Monitorship.} In 2020, the consumer finance firm Upstart, the NAACP, and Relman Colfax, a civil rights law firm, entered a legal agreement to investigate racial discrimination in Upstart's lending model due to the NAACP's concerns over the use of attributes related to educational attainment, such as the name of the college applicants attended if they had a college degree~\cite{naacp_statement}. The goal of the agreement was to first to determine if there was a legally relevant difference in selection rate between Black and white applicants using Upstart's model, which they found there was~\cite{colfax2021report2}. Once this was established, Relman Colfax followed the disparate impact doctrine~\cite{disp_impact_doctrine} to determine whether Upstart would be legally required to change their model: to do so, they search for a "less discriminatory alternative" model, or LDA, with equivalent performance but less disparate impact across racial groups. Under the disparate impact law, once discrimination is established, if such a model exists, then the company using the discriminatory model \emph{must} replace their model with this less discriminatory alternative~\cite{disp_impact_doctrine}. 


\xhdr{Searching for a Less Discriminatory Alternatives: Suboptimal Approaches.} 
After establishing discriminatory model behavior, third-party investigators developed and implemented a strategy to find a less discriminatory model with similar predictive performance to Upstart's original algorithm. Notably, the third-party bias investigators discounted all algorithmic fairness techniques to search for discrimination out of hand, seemingly from concern over legal repercussions over the use of the protected attribute to influence model behavior, and a desire to ``align with traditional principles gleaned from antidiscrimination
jurisprudence''~\cite{colfax2021report1}. As the authors of the bias investigation report note:
\begin{displayquote}
A range of techniques for mitigating disparities is proposed in the algorithmic fairness literature. \textit{Some of these proposals could raise independent fair lending risks, such as the use of different
models for different protected classes or the improper use of prohibited bases as predictive variables}...While [the algorithmic fairness]
conversation is valuable, many “fairness” proposals do not engage or align with the established three-step disparate
impact analysis reflected in case law and regulatory materials.~\cite{colfax2021report1}
\end{displayquote}
The procedure that was taken instead was intervening at the feature selection step, and searching the feature space for a model with a subset of features that was less discriminatory. That is, the practitioners created a model for several different feature combinations, and tested the disparate impact of each one~\cite{colfax2021report2}. While a less discriminatory alternative was likely discovered,\footnote{The model discovered was less discriminatory but also suffered performance drop, which Relman Colfax argued was within an acceptable range to be an ``equivalent performance'', but the exact rules around this have yet to be established---so it is unclear if this model would in fact suffice as an LDA~\cite{colfax2022report3}.}, this procedure took sufficiently long that Upstart updated its model before the investigations were completed~\cite{colfax2022report3}. We note that the blind, exhaustive search for a less discriminatory model at just one intervention point in the machine learning pipeline is almost certainly expensive, inefficient, and leads to suboptimal outcomes. If pipeline-aware tools had been available to better isolate sources of bias in the \textit{entire} pipeline, beyond feature choice, it is likely they would have found a less discriminatory model with acceptable predictive performance more efficiently.
 
It is imperative that the approach taken in the Upstart monitorship does not become standard or accepted in the credit industry. The disparate impact framework gives advocates and model practitioners a way to challenge the use of discriminatory algorithms, and further incentivize companies to thoroughly explore the space of possible algorithms to find the least discriminatory one within those with sufficient business utility---but using ineffective methods to enforce these regulatory tools weaken their power. We suggest that in order to effectively leverage the disparate impact doctrine, we must operationalize a pipeline-aware approach to ML fairness. And, even beyond searching for LDA models, tools informed by a pipeline-based approach may also aid in creating more standard and rigorous approaches to algorithmic audits more broadly. 


\subsection{Evidence from the Classroom}\label{sec:teaching_evidence}
Our team has documented the challenges of instilling the pipeline-centric view of ML harms in students using traditional teaching methods (e.g., lectures containing real-world examples). The classroom activity outlined in this section was conducted by one of us at an R1 educational institution as part of a graduate-level course focused on the ethical and societal considerations around the use of ML in socially high-stakes domains. Our IRB approved the activity, and students had the option of opting out of data collection for research purposes (IRB included in the appendix.)
%.\footnote{To maintain author anonymity during the review phase, we will share our IRB approval letter and if our paper is recommended for publication after the review process.} 

\xhdr{Population and sampling. }
In total, 37 students participated in the class activity. 
 Prior completion of at least one Machine Learning course was a prerequisite for enrollment. So all participants had a non-negligible background in Machine Learning. Specifically, $\sim 80\%$ characterized the familiarity with ML as intermediate, $\sim 14\%$ as advances, and $\sim 5\%$ as elementary. All students enrolled in the course took it as an elective. This fact implies that compared to a random sample of students with ML knowledge, our participants were likely more aware of ML harms and more motivated to address them. 

\xhdr{Study design.} Students were introduced to the ML pipeline through an approximately 45-minutes long lecture. The lecture focused on the supervised learning paradigm and broke down the supervised learning pipeline into the following five stages: problem formulation, data collection and processing, model specification, model fitting/training, and deployment in the real world.
\iffalse
\begin{enumerate}
    \item \textbf{Task definition} corresponding to the choice of features and predictive targets.
    \item \textbf{Data collection and processing} corresponding to the choice and processing of the input data $D = \{(x_i,y_i)\}_{i=1}^n$
    \item \textbf{Model specification} corresponding to the choice of the hypothesis class, $H$.
    \item \textbf{Model fitting/training:} choosing a specific loss function, $L$, and optimizing it via existing optimization techniques to obtain a model $h \in H$
    \item \textbf{Deployment in real-world}, corresponding to the deployment of $h$ in real-world practice, and its predictions $\hat{y}$ translating into decisions that can harm/benefit certain individuals and communities
\end{enumerate}
\fi
For each stage, students were presented with multiple examples of how choices at that stage can lead to harmful outcomes, such as unfairness, at the end of the pipeline (see Figure~\ref{fig:pipeline}). %For example, \hhcomment{TBC.}
They were then asked to team up with 3-4 classmates and pick a societal domain as the focus of their group activity. Examples offered to them included employment (e.g., hiring employees); 
education (e.g., admitting students); 
medicine (e.g., diagnosing skin cancer); 
housing (e.g., allocating limited housing units
child welfare (e.g., investigating referral calls); 
criminal justice (e.g., pretrial sentencing);
public safety (e.g., allocating patrol resources in policing 
e-commerce (e.g., advertising; ranking sellers on Amazon); 
social media (e.g., news recommendation; content moderation);
and transportation (e.g., autonomous vehicles). One team suggested finance (e.g., credit lending) as their topic.
Third, students were given 30 minutes to discuss the following questions about their application domain with teammates and submit their written responses individually:
\begin{itemize}
    \item Characterizing the specific \textbf{predictive task} their team focused on. %Please briefly describe how you came across this task.	
    \item The \textbf{type of harm} observed. %Please briefly describe whether you know of precedence for this type of harm in your domain of choice.	
    \item Their \textbf{hypotheses around the sources} of this harm in through the ML pipeline. %Please be comprehensive to the extent possible.	
    \item Their\textbf{hypotheses around potentially effective remedies} for addressing those sources. %Please be comprehensive to the extent possible.
\end{itemize}
 
\input{classroom_table.tex}

\xhdr{Findings. }
A thematic analysis of submitted responses revealed several challenges: 

\xhdr{Theme 1: Specifying how a real-world problem gets translated into a predictive task was not straightforward.} Table~\ref{tab:classroom} overviews how each team defined their predictive tasks. For example, the finance team defined the task as \textit{assessing the \emph{creditworthiness} of individuals using their demographic and socio-economic data}. The public safety team defined the predictive task as \textit{allocating police presence to \emph{high-risk} areas}. The social media team defined the task as \textit{predicting whether a news article is fake}. Note that notions of applicant's \emph{creditworthiness} or neighborhood's safety \emph{risk}, or \emph{fakeness} of an article's content are not well-defined targets. Other teams did not adequately distinguish between the construct of interest and its operationalization as the target of prediction. For example, some members of the organ transplant team characterized the task as deciding \textit{which people \emph{should} receive an organ transplant}. In contrast, others characterized it as \textit{predicting whether an individual would receive an organ transplant in a given hospital}. Note the difference between \emph{``should''} and \emph{``would''}.


\xhdr{Theme 2: harms were characterized in broad strokes.}
Some teams described harm without specifying the groups or communities that could be impacted by it and the baseline of comparison. For example, the housing team stated \textit{price discrepancies} due to property location as the harm occurring in their domain but did not specify who could be negatively impacted by price discrepancies and in comparison with what reference group this should be considered a harm. Another example was \textit{spread of fake news} as the harm without mentioning whom it can impact negatively and how.

\xhdr{Theme 3: Students had difficulty mapping the observed harm to a plausible underlying cause.} For example, the child welfare group attempted to explain the harm against Black communities by noting that the feature, Race, was not quantified with sufficient granularity. The tool allowed only three racial categories: White, Black, and Other, and they hypothesized that that could be the cause of the disparity. Note that there is no plausible mechanism through which this lack of granularity might have led to disparities in child welfare risk assessments against Black communities. As another example, the finance team offered \textit{biases of developers} as the potential source of disparity in lending practices.


\xhdr{Theme 4: Students had difficulty mapping their hypothesized causes to plausible remedies.} For example, the Child Welfare team proposed randomly selecting instances for inclusion in the training data. The online exam proctoring group suggested further transparency (e.g., telling students what behavior results in a cheating flag) to reduce errors. 

\xhdr{Theme 5: Students used broad-stroke language to describe causes and remedies of harm.} For example, several teams referred to \textit{biased data} as the underlying cause of harm and offered \textbf{more comprehensive data collection} as the remedy. While correct, such high-level assessments are unlikely to lead to concrete actions in practice. Another commonly proposed remedy was \textit{human oversight} of decisions without specifying the efficiency ramifications of leaving the final call to human decision-makers.

In a session after the data collection and analysis, the instructor led a class-wide discussion in which students were encouraged to reflect on the activity and some of the gaps in the arguments presented by student teams. 


\iffalse
% \subsection{Evidence from Practice}
\subsection{Lessons from Applying ML in Practice}\label{sec:practice}
In addition to educating students on developing fair ML systems, there is a need to support practitioners involved in similar work. This work has spanned a wide range of policy domains including health \cite{Ramachandran2020,potash2015predictive,somanchi2015early,Potash2020}, criminal justice \cite{ Bauman2018ReducingInterventions,Rodolfa2020CaseInterventions}, social services \cite{pan2017machine}, housing \cite{Ye2019UsingCity}, urban infrastructure \cite{Kumar2018UsingBreaks}, and education \cite{lakkaraju2015machine, mvescblog, tulsaposter} and has spanned federal agencies to city government. For instance, identifying households with small children at risk for lead poisoning to allocate limited remediation resources \cite{potash2015predictive,Potash2020}, evaluating the fairness of algorithms used to target audits of tax returns \cite{black2022algorithmic}, predicting water mains at risk of breaking \cite{Kumar2018UsingBreaks}, or intervening with social services and mental health outreach to break the cycle of incarceration \cite{ Bauman2018ReducingInterventions,Rodolfa2020CaseInterventions}. \krcomment{might need to check if we need to suppress citations here for anonymous review since we refer to our previous work?}


These projects are generally high-stakes in nature, with the potential for both significant impact on a given individual's life as well as the scale to affect large populations. As a matter of course, therefore, fairness is a key element of the conversation from the very earliest stages of project scoping as we understand the partner's goals and constraints. Although we haven't made a quantitative assessment of these perceptions, across this wide-ranging work in partnership with government agencies and non-profits, we have found two misconceptions about algorithmic fairness to be nearly universal. First is the perception that most or all disparities in model outputs can be attributed to underlying biases in the training data, with little appreciation for the role played by choices made by the system developers. For example, the concept of model cards\cite{mitchell2019model} or audit tools\cite{saleiro2018aequitas} frequently come up in these conversations, yet they tend to over-focus on understanding the training data that was used to develop a system without much regard for the model development process itself. Understanding potential disparities in the training data is important, but as discussed above, certainly not sufficient for understanding model fairness. And, second, is the unfounded belief that simply excluding sensitive attributes from a model's feature set will produce an unbiased model. Unfortunately, we've frequently seen that cited by practitioners and vendors as an assertion of model fairness without any actual measurement of the model's outputs --- in the worst cases, regarding deployed systems in very sensitive contexts such as predictive policing and other criminal justice and financial services applications.

Notably, we've found these misconceptions to be quite common regardless of the amount of technical experience of the partner, ranging from policymakers to data scientists with training in machine learning. These observations, while anecdotal in nature, have helped form our opinion about the urgent need for making a pipeline-centric view of ML fairness more commonplace. \krcomment{I realize this is a bit high-level and not sure if we want to try to add some more specific stories/details, though given the page limit, we might also want to keep things a bit shorter.}

\krcomment{@rayid -- I'm not sure how much the fairness tree work with Lingwei has progressed, but if you've done more structured interviews with government partners, would it make sense to include anything from them here? Plus it only seems natural to have Lingwei as an author here given the RegLab/CMU overlap...}
\fi


==> research_agenda.tex <==
%\section{Research Agenda}
%\label{sec:agenda}

Reflecting on the state of fairness literature from a pipeline-aware perspective, we offer five key insights to start operationalizing a pipeline-aware approach to fairness. Namely, we identify (1) the need to investigate and document choices made along real-world pipelines, including those related to bias mitigation; (2) the need to bridge the gap across literatures which \emph{identify} ways the bias enters ML pipeliens on-the-ground, such as HCI, and literatures which build operational mitigation techniques, such as FairML; (3) the need to study interaction effects across decisions made along the pipeline; (4) the need to address holes in the current research--paying attention to neglected areas of the pipeline such as viability assessment, and entire modes of research such as producing \emph{measurement} techniques to catch many of the entry points for bias identified along the pipeline; and (5) finally, the need to produce guidance on how to choose among several biased building choices.

\xhdr{Investigation of Real-World Pipelines}
The algorithmic fairness literature has a dearth of knowledge about what on-the-ground pipelines look like. Although many papers outline abstracted pipelines (including our own), the actual model creation steps taken by practitioners for a variety of real-world systems (e.g. in consumer finance, healthcare, hiring systems) are at the very least not cataloged in any centralized place. Bias entering from choices along the pipeline cannot be studied, measured, and mitigated if we do not know what choices are being made---thus mapping out actual pipeline choices is a necessary step to operationalize a pipeline-aware approach to fairness.\\
%Relatedly, there are few case studies of bias mitigation in the fairness literature. 
\textbf{Action Items:}  (1) We encourage exploration and documentation of pipeline decisions made in a variety of machine learning pipelines in different applications; and (2) centralization of this information so that researchers can study how pipeline decisions they may have been unaware of impact fairness behavior.

\xhdr{Disconnect between Problem Identification and Mitigation}
Bias problems are often discovered in disciplines on the fringe or outside of machine learning, such as human-computer interaction literature and database management~\cite{sambasivan2021everyone}. 
Since many papers which point to problems along the AI pipeline, especially in the earlier stages, are structured around interviews---they may elide more low-level technical sources of pipeline choices leading to bias, e.g. such as record linkage issues leading to non-IID data dropping. 
While they are helpful in the important first step of identifying problems, they provide little direction for creating operationalizable solutions to these problems, or often even sufficiently detailed information about each system studied to be able to understand the mapping between data collection problems and model behavior. 

Symmetrically, many papers in the mainstream algorithmic fairness literature do not test their techniques on real decision-making systems–or even on datasets beyond Adult, German Credit, and a few others. Though case studies may often be disregarded as implementing old methods and thus not novel, it is crucial that we give them more attention so that we learn about the failure modes of the techniques that we create. While there are papers about the overall problems production teams face when implementing fairness goals, e.g. ~\cite{richardson2021towards, madaio2020co,holstein2019improving,sambasivan2021everyone}, these do not provide an in-depth catalogue of the successes and failures of all pipeline intervention techniques in practice. Proposed methods to intervene on the machine learning pipeline should be tested in a variety of real-world systems to see where they fail and succeed. \\
\textbf{Action Items:}  (1) We encourage bridging the problems identified by the HCI, CSCW, and other literatures, with the technical detail of the algorithmic fairness literature to introduce mitigation techniques for data collection harms; (2) In particular, we encourage AI Fairness researchers to build off of tools for addressing generalized data and modeling pipeline issues, i.e. not specialized to fairness problems, and adapt them for debiasing ML systems--for example, extending Breck et al.~\cite{breck2019data}'s data validation pipeline to address fairness concerns; 
(3) We encourage testing the pipeline-based bias mitigation methods proposed to date in on-the-ground ML systems. This is necessary to uncover which perform best under various circumstances, determine  failure modes, and learn how to integrate these techniques into actual ML systems.

\xhdr{Interaction Effects}
Most fairness-related papers focus on \emph{one issue} in the pipeline: they present a bias problem, then often give a mitigation method, implicitly assuming that the identified source of bias is the only one of interest to the model practitioner, and the suggested intervention will not lead to other effects on the model, including other forms of bias. That is, much of the literature fails to provide insight into how different biases and mitigation techniques along the pipeline interact. Does solving each issue in isolation work, or does a pipeline-aware approach to fairness need to engage with interaction effects to work in practice? There are a few papers that show the impacts of the intersection between multiple sources of bias has on the effectiveness of interventions--e.g., Li et al.~\cite{li2022more} point to how active sampling techniques to address sampling bias can make models \emph{more} unfair when label bias is present. However, any set of choices on the machine learning pipeline may have interaction effects, suggesting many paths for exploration.
Beyond studying interaction effects, there are very few papers (with some exceptions~\cite{10.1145/3531146.3533132,10.1145/3351095.3372874}) 
%\footnote{Though there are some, e.g.~\cite{10.1145/3531146.3533132,10.1145/3351095.3372874}} 
which engage with the entire pipeline: taking fairness into account when making every modeling decision, and testing along the way---which is the end goal of a pipeline-based approach to fairness. \\
\textbf{Action Items:} We recommend (1) investigating interaction effects of various sources of bias, \textit{and} bias mitigation strategies across the ML pipeline, and (2) developing tools that allow for such exploration (for example, extending~\citep{akpinar2022sandbox}.)

\xhdr{Holes in Research: Measurement Methods and Others}
Within the few papers that do discuss pipeline-aware approaches to fairness, most are problem identification or mitigation techniques— only 17\%\footnote{We calculate this by taking all of the measurement papers identified (67) and subtracting the number that simply introduce new fairness metrics (15), and dividing this number (52) by the total number of pipeline fairness papers identified.} of the papers that we identified are actually providing techniques to measure whether or not a given pipeline choice will lead to downstream unfairness ex-ante. But measurement is key because it may allow us to decide when or when not to take an action. How can we effectively measure algorithmic harms? Relatedly, there are many proposed solutions of how to solve a problem once it has already happened--e.g. unrepresentative data, etc.---but how can we develop tests to \emph{prevent} choices that lead to algorithmic harms? For example, can we predict beforehand whether and how fairness problems will result from the way in which a model is integrated into a given decision structure? 
Additionally, we find that research on \emph{how} bias can enter machine learning decision systems via choices made along the pipeline is unevenly distributed across the pipeline. There are some areas of the pipeline that are well-studied in this regard, such as data collection; but the majority of the pipeline has light-to-no coverage: e.g. viability assessments, problem formulation, and large parts of organizational integration. These areas must be prioritized for searching for fairness failure modes and mitigation techniques.
Finally, the majority of the research to date measures the effect of various pipeline choices on common definitions, e.g. demographic disparity,  accuracy disparity, etc. How can we map the pipeline in a general enough fashion that we may be able to understand how more contextualized notions of fairness are impacted by pipeline decisions? \\
\textbf{Action Items} (1) We encourage building methods for \emph{measuring} the harms introduced by decisions along the machine learning pipeline; (2) Exploring pipeline decisions that have received little attention; and (3) exploring the fairness effects of pipeline decisions beyond the most common metrics. \vspace{0.2em}

\xhdr{Guidance on Choosing Among Imperfect Design Alternatives}
ML practitioners often face choices between imperfect/biased alternatives.
It will almost always be the case that with adequate effort, they can produce fairer, but not perfectly fair models. Any choice a designer makes will likely lead to some form of bias, some more and some less problematic in the given decision-making domain. However, there is little guidance in the literature on deciding when one alternative is better than another in light of all contextual considerations, when certain biases are conditionally acceptable, and how the answers to these questions depend on the context. \\
%will stiHowever, there is  little discussion on how to choose the lesser of several evils, in a situation where every viable choice in front of a model practitioner leads to bias of a different type, as is often the case. We 
%little guidance on what to do when you realize a choice will lead to bias: often no matter what choice you use will lead to bias, often of different types. We need guidance: when is one alternative better than the other? \\
\textbf{Action Items}: (1) Developing normative guidelines to weigh a variety of imperfect/biased design choices against each other is a crucial avenue for collaboration between ML experts and ethicists; (2) Exploring how different types of bias are currently traded off in practice when they are discovered; and (3) Understanding if there are any relationships or couplings of different sources or forms of bias that often go together, or have opposing relationships. %; (3) developing guidelines on how to face bias when it arises in practice.


% Lots of papers about a few problems/examples of specific problems within each part of the pipeline; we know there are more potential problems and the literature does not reflect that
% E.g.: non iid data dropping during linkage
% Other ideas?

% Most fairness-related papers focus on \emph{one issue} in the pipeline, but fail to provide insight into how these different aspects of the pipeline interact. Does solving each issue in isolation work, or does a pipeline-aware approach to fairness need to engage with interaction effects?
% De-arteaga paper points to this: https://ojs.aaai.org/index.php/HCOMP/article/view/21994 

% Disconnect between finding problems and mitigating them: 
% Usable, worth applying in real world.
% No measurement methods

% Beyond studying interaction effects, there are very few papers which engage with the entire pipeline: taking fairness into account when making every modeling decision, and testing along the way. The closest we’ve seen to such approaches are:
% Feminism paper

% Very little guidance on what to do when you realize a choice will lead to bias: often no matter what choice you use will lead to bias, often of different types. We need guidance: when is one alternative better than the other?

% Many of the pipeline papers still engage with one particular notion of fairness (often demographic disparity). It would be helpful to create a more generalized mapping of how modeling choices change prediction behavior, beyond a single metric.

%  Need for documenting current practices and standards; usability of proposed techniques.


% \hhcomment{
% \begin{itemize}
%     \item Research focuses on method development, as opposed to best practices and standards that can be used on the ground.
%     \item Unclear how to assess when a biased choice warrants a design change, and when it can be accommodated.
%     \item Focus on the ML pipeline, as opposed to its broader social context.
%     \item Need for documenting current practices and standards; usability of proposed techniques.
% \end{itemize}

% }

% \begin{enumerate}
%     \item There are some areas of the pipeline which are well-studied, such as data collection; but the majority of the pipeline has light-to-no coverage in the fairness literature: e.g. viability assessments, problem formulation, and large parts of organizational integration. These areas must be prioritized for searching for fairness failure modes and mitigation techniques.
%     \item The majority of the research that has been done measures the effect of various pipeline choices (e.g. feature selection, data preprocessing) on demographic disparity, TPR/FPR/EO, or accuracy disparity. How can we map the pipeline in a general enough fashion that we may be able to understand how more contextualized notions of fairness are impacted by pipeline decisions?
%     \item Most pipeline-related papers focus on \emph{one issue} in the pipeline. How do they interact? Does solving each issue in isolation work? Relatedly, we do not have almost any examples of algorithmic fairness work which holistically considers the entire pipeline in its creation and deployment. This is a pressing area for future work.
 
    
% \end{enumerate}

% Action items:
% \begin{itemize}
%     \item We must map end-to-end pipelines in a variety of domains (credit, criminal justice, education, ad delivery, etc etc) and across different instantiations of those domains (geography) to get a fuller understanding of the \emph{full} suite of decisions that go in to making machine learning models.
%     \item We must proactively delve into other literatures---HCI, database management, software development, and many others---to build off of the tools they already have operationalized for these generalized (i.e. not specialized to fairness problems) and see how we can adopt them for algorithmic harms. [E.g. Breck et al.~\cite{breck2019data}'s data validation pipeline for ML]
%     \item For the many promising methods already proposed in the literature, we must test them on a variety of real systems, and understand their failure modes IRL.
% \end{itemize}


% We encourage AI Fairness researchers to delve into other literatures---HCI, database management, software development, and many others---to build off of the tools they already have operationalized for these generalized (i.e. not specialized to fairness problems) and see how we can adopt them for algorithmic harms--e.g. Breck et al.~\cite{breck2019data}'s data validation pipeline for ML.





% Some important questions to explore include:
% \begin{itemize}
%     \item What are the typical steps for algorithmic-decision-to-human-decisionmaker-handoff in a variety of applications? (E.g. credit, criminal justice, other federal agencies using AI systems in ACUS report, etc). 
%     \item What documented examples exist of algorithms not being used as intended by the developers, or policymakers, within an organization? Some famous examples include LAPD having complete discretion to add individuals to the recommendations of person-based predictive policing models~\cite{}, or of facial recognition models used in law enforcement offices used as the main form of evidence to incarcerate someone~\cite{}, or facial recognition models used at certainty thresholds less than recommended by their developers~\cite{}. What more exist, and what can we learn from these systems?
%     \item Can we predict beforehand whether and how fairness problems will result from the way in which a model is integrated into a given decision structure?
%     \item How can model-makers more clearly specify the correct use of their system, and how can organizations adopt these protocols?
%     \item Given the theoretical work introduced in Donahue et al.~\cite{donahue2022human}, to what extent do these patterns appear in systems on the ground? How can regimes of overlapping error be mitigated?
%     \item How does how a model's outputs are presented to a human decision-maker change the fairness of the outcome, if at all?
%     \item \textcolor{blue}{Other important questions, guys?}
% \end{itemize}

% Some important questions to explore include:
% \begin{itemize}
% \item What does the process of feature creation look like in a variety of domains? What decision processes do modelers go through when creating features from raw data?
% \item 
% \end{itemize}

==> versions/intro_01_26.tex <==
\section{Introduction} 

%Algorithmic fairness is no longer a nascent field. Through years of work from activists, journalists, researchers, and AI practitioners, professionals across industry, government, and the nonprofit sectors rely on algorithmic fairness expertise to guide their implementation of AI systems. However, while algorithmic fairness scholarship is broad, in practice, it often gets simplified into enforcing
%a mathematically abstracted definition of fairness on top of a pre-made system, either by enforcing fairness constraints within the optimization function, post-processing model outputs, or occasionally by manipulating data. Indeed, as this paper points out, the plurality of fairness research falls into either creating abstracted definitions to enforce, or finding ways to enforce a fairness constraint on top of an already constructed system. 

\begin{itemize}
    \item Prevalence of ML harms, chief among them issues of unfairness
    \item lots of work to deal with it by offering frameworks and mitigation strategies
   , but this hasn't lead to concrete guidelines and tools
   
    \item typical approach by researchers, practitioners, academia: select an adhoc method to ``fix'' fairness without understanding or knowing how this view will help with appropriate mitigation in practice.
    \item Recently research community has honed in on the importance of a pipeline view of fairness
    \item To support the above, mention our documented experience as teachers and practitioners observing this issue first hand
    \item our proposal: use a pipeline-centric view that can provide methodologies and tools to support a more structured and targeted approach to reducing harms that be caused by the use of ML systems 
    \item: our goal: to work with the community to operationalize ... and create .... that can result in ...
    \item our contributions here: toward this goal we do a systematic review of the relevant literature, offering a research agenda, and a set of requirements for tools and methodologies needed.
    \item this is the first step toward a broader agenda in which we co-design guidelines and processes for students and practitioners to understand the ML pipeline/lifecycle to detect and mitigate harms appropriately.
\end{itemize}


Faithful to its roots within computer science literature, many well-known conceptions of algorithmic fairness are highly abstracted from the details of any one system implementation. Most formalizations of fairness in the AI literature abstract the problem of unfair model behavior to generic model inputs, model outputs, and the ground truth label. The most common fairness definitions, such as demographic parity, equalized false and/or true positive rates, and equal accuracy, can be expressed only with ``observed features V [i.e., input features], outcomes Y [i.e., ground truth labels] ... and decisions D [i.e., model outputs]''~\citep{mitchell2021algorithmic}. Even slightly less common notions, such as counterfactual fairness or individual fairness, are expressed as a constraint on model inputs and outputs in relation to additional information about the data distribution, such as a given similarity metric or causal graph~\cite{mitchell2021algorithmic}. 

This level of abstraction has many merits: abstraction to the basic elements of a system leads to transportability across implementations, and so these definitions, and the methods used to enforce them, can be applied to fairness problems in a variety of application contexts. Further, the abstraction of these metrics adds to their simplicity, so they can be easily intuited and computed. Beyond these merits, in many contexts, such fairness definitions are also fundamentally important: for example, extreme demographic disparity is of legal consequence in areas such as hiring~\cite{griggs1971}. 

However, as others have pointed out~\cite{akpinar2022sandbox, suresh2021framework}, %this abstracted approach has pitfalls, 
the approach of enforcing an abstracted definition on top of a pre-built machine learning system has pitfalls---
often based on the fact it does not pay attention to the details of the system over which it is enforced. Indeed, details about the AI system and its context---such as the data or model type used, or how the predictions are used in practice-- can even render enforcing these definitions harmful from an equity standpoint~\cite{wang2021fair,black2022algorithmic}. For example, Wang et al. find that enforcing fairness constraints on systems where there is asymmetric noise on training labels across demographic groups can actually increase performance disparities~\cite{wang2021fair}.
Additionally, many commonly used approaches for enforcing fairness constraints in practice have been shown to be ill-suited for many policy-related problems due to incompatibility with relevant implementation setups such as selecting up to a budget~\cite{black2022algorithmic}, or generally brittle to small changes in modeling setup~\cite{friedler2019comparative}. 
%Some works even suggest that 

More broadly, this abstracted approach inherently ignores situations where sources of bias are embedded in choices made in the model-building process, i.e., the choices made along the \emph{AI pipeline}. 
All of the choices made at each step of the AI pipeline have impacts on the model’s behavior. Thus, we can leverage the pipeline to change and understand AI model behavior: if we believe a model is acting unfairly, certainly, one way to change that behavior is to change some choices we made along the way to making that model.
In these situations, fairness problems may be mitigated by \emph{changing} certain modeling choices, i.e. via a targeted intervention, rather than by adding a constraint on top of a model. In some cases, taking such an approach can also reduce the oft-discussed fairness-performance tradeoff. Previous work suggests that \emph{not} taking such a pipeline-based approach when possible ``hide[s] the real problem while creating an illusion of
fairness''~\cite{akpinar2022sandbox}. 

%Symmetrically, the choices we make along the machine learning pipeline may lead to fairness problems themselves--potentially inexpressible through definitions abstracted to input and output.

In this paper, we draw attention to an alternate approach to tackling algorithmic fairness problems, which we call \textit{pipeline fairness}. In pipeline-based fairness, practitioners interrogate choices made at each step of the AI creation pipeline to search for ways in which these choices impact model fairness behavior, and then, when possible, change the relevant modeling choices to abate this effect. 
Importantly, those modeling choices are often practically changeable. While modeling choices are often made in search of the most accurate possible model, recent work has shown that there are usually many potential models--made with different modeling choices---with equivalent performance that can be created for any given prediction problem, while displaying considerably different fairness behavior~\cite{black2022model,blackleave2021,marx2019,rodolfa2021empirical}. Thus, it may often be the case that changing relevant modeling choices can mitigate bias at a decreased cost to other performance metrics, or indeed, may even improve the model~\cite{black2022algorithmic}. 
%This technique is inherently contextualized to a model's specific application and implementation; it promotes building systems with equity in 
%This technique takes into account many principles that the algorithmic fairness community has suggested for building systems as equitably as possible, such as, building with equity in mind from the beginning, and creating contextualized fairness interventions. (should go elsewhere)

Importantly, we suggest the pipeline-based approach to algorithmic fairness not as a replacement or improvement upon the literature to date, but rather as an additional, largely unexplored, toolbox, which holds promise for expanding our ability to tackle fairness problems on the ground. Indeed, the ``abstraction-based approach'' to fairness can be understood as a subset of the pipeline based approach: the majority of algorithmic fairness literature to date concentrates on changing a subset of the decisions made along the pipeline, namely, choosing a model's optimization or loss functions, and evaluation metrics. Additionally, we do not claim to introduce the idea of pipeline fairness: instead, we suggest that pipeline fairness is simply a name for a (dispersed) pattern of algorithmic fairness work that is ongoing, but has yet to be collected into one thread--however, we argue that it is beneficial to do so. 

A pipeline approach to fairness relies on a mapping of the relationships between choices made at each step of the \emph{AI pipeline} to its effects on a model's fairness behavior, for a given fairness goal. This mapping is not something that exists in any level of detail at the moment, nor is housed in any specific place---examples of how modeling choices influence fairness behavior are few and far between in the literature in relation to abstraction-based techniques, as this paper demonstrates. 
The goals of this paper are  threefold: first, to define, and draw attention to, a pipeline-based approach to algorithmic fairness; second, to collect and synthesize the fairness literature that embodies this approach, in an attempt to map out which areas of the pipeline are better understood, and which are less; and finally, to create a research agenda for filling out our map of how modeling choices can lead to fairness pitfalls, in service of creating a robust roadmap for practitioners of how we can build systems as free from bias as possible.%, drawing from examples

%\textbf{The goal of this paper is to show 
%what parts of this mapping have received attention, which are relatively untouched, and outline a research agenda to collaboratively can leverage the information and techniques we have to develop a full understanding of pipeline fairness.}

As a whole, this work aims to remind researchers of the immense flexibility that the AI creation pipeline gives practitioners with respect to how to reach the goals they set out to achieve with machine learning models---but also, how the choices made along the AI pipeline have to be carefully considered in terms of their impact on desired model behaviors, as even seemingly small choices can have a large impact.
We hope that together as a research community, we can learn to leverage all the choices made along the AI pipeline---from data collection and feature engineering, to hypothesis class selection, to the objective functions---as places where decision can be made to improve fairness behavior, we thus greatly expand our arsenal of unfairness-fighting tools.

The rest of this paper proceeds as follows: in Section~\ref{sec:pipfair}, we define the AI pipeline and pipeline fairness in detail. In Section~\ref{sec:litreview}, we categorize the fairness literature (fairness papers from top five fairness and ML conferences from the past five years) from the perspective of pipeline fairness, and point out areas where there has been less and more attention, and finally, in Section~\ref{sec:agenda}, we construct our research agenda for a fuller understanding of pipeline fairness moving forward.

\color{red}{Emily: should I have a brief discussion of what the AI pipeline is in the intro, and if so, where?}
\color{black}
% The main contributions of this paper are :
% \begin{itemize}
%     \item Defining pipeline fairness
%     \item Synthesizing the work on pipeline fairness to date in the literature in a community-updatable document 
%     \item Creating a research agenda in order to flesh out our understanding of how modeling choices along the pipeline impact fairness behavior of AI systems, so that we may guide practitioners through creating more equitable systems in the future.
% \end{itemize}





%More broadly, considering more aspects of the modeling process as an intervention point simp

%More broadly, this abstracted approach inherently ignores situations where a root cause of bias is embedded in lower-level modeling choices of the system: and thus, may be mitigated by changing that modeling choice. 

%Importantly, those modeling choices are often practically changeable. While modeling choices are often made in search of the most accurate possible model, recent work has shown that there are usually many potential models--made with different modeling choices---with equivalent performance that can be created for any given prediction problem, while displaying considerably different fairness behavior~\cite{black2022model,blackleave2021,marx2019,rodolfa2021empirical}. 

%In this paper, we draw attention to an alternate approach to tackling algorithmic fairness problems, which we call \textit{pipeline fairness}. A pipeline approach to fairness relies on mapping the relationships between choices made at each step of the \emph{AI pipeline} to its effects on a model's fairness behavior, for a given fairness goal. 


% By approaching bias mitigation through changing a modeling choice rather than adding an additional 

% Thus, completely abstracting fairness problems---and in so doing, ignoring modeling choices when tackling fairness issues--- can lead to ignoring situations where direct interventions on the root cause of bias can be performed, rather than placing a constraint on top of a system. Taking the approach of ignoring the underlying system and adding constraints on top of a model can (sometimes unnecessarily) introduce ``fairness’’-performance tradeoffs. 
% Sometimes (but rarely), the (only) way to mitigate bias in a system is to add constraints on top of a model to force it to adhere to a given notion of fairness. 
% However, often, there are decisions made during the system building process that exacerbate unfair behavior. 






% %Algorithmic Fairness is no longer a nascent field. 
% While interest in, and scholarship of, algorithmic fairness is broad, it often gets simplified, and packaged in practice, into simply enforcing
% mathematically abstracted fairness definitions onto
% %statistical group-based fairness notions on a 
% pre-made ML system, often through adding relevant constraints. 

% Notably, most formalizations of fairness in the AI literature abstract the problem of unfair model behavior to model inputs, model outputs, and the ground truth label. The most common fairness definitions, such as demographic parity, equalized false and/or true positive rates, and equal accuracy, can be expressed only with ``observed features V [i.e., input features], outcomes Y [i.e., ground truth labels] ... and decisions D [i.e., model outputs]''~\citep{mitchell2021algorithmic}. Even slightly less common notions, such as counterfactual fairness or individual fairness, are expressed as a constraint on model inputs and outputs in relation to additional information about the data distribution, such as a given similarity metric or causal graph~\cite{mitchell2021algorithmic}. 

% This abstraction has many merits: abstraction to basic elements of a system leads to transportability, and so these definitions can be applied to a large variety of fairness problems. Further, these metrics can be easily computed and tested no matter the model implementation. Beyond these merits, in many contexts, such fairness definitions are also fundamentally important: for example, extreme demographic disparity is of legal consequence in areas such as hiring~\cite{griggs1971}. 


% While this abstracted approach is useful in certain contexts, many works over the years have pointed to its pitfalls [CITE HERE]: some have argued that enforcing abstract definitions on top of a pre-made system  can exclude countless notions of what unfairness means, particularly ones that are especially relevant to the given application context [CITE], others have shown how details about the ML system---the data or model type used, or how the predictions are used in practice--render enforcing these definitions useless at best and harmful at worst. 

% Indeed, 

% Through years of work from activists, journalists, researchers, and AI practitioners, professionals across industry, government, and the nonprofit sectors engage with, and rely on, algorithmic fairness expertise to guide their implementation of AI systems.



% While this approach is useful in certain contexts, many works over the years have pointed to the pitfalls of this approach [CITE HERE]: some have argued this one-size-fits all approach can exclude countless notions of what unfairness means, particularly ones that are especially relevant to the given application context [CITE], others have shown how details about the ML system---the data or model type used, or how the predictions are used in practice--render enforcing these definitions useless at best and harmful at worst. 

% In this paper, we draw attention to an alternate approach to tackling algorithmic fairness problems, which we call \textit{pipeline fairness}. We argue that pipeline fairness is simply a name for a (dispersed) pattern of algorithmic fairness work that is ongoing, and holds promise for directing the field towards creating another set of useful tools for fighting fairness problems on the ground. In this work, we define the pipeline-based approach to fairness; collect and organize the work to date which uses this approach; and create a research agenda outlining the next steps required to create an pipeline-fairness based arsenal of techniques to address unfairness in practice. 
% %but has not been collected under one umbrella---however, we argue it should be, due to its promise for directing the field towards creating another set of useful tools for fighting fairness problems on the ground. 



 

% In this work, we call this series of decisions model practitioners have to make the \emph{AI creation pipeline}, or the pipeline. 
% %As the pipeline determines how models reach their decision-making schema, we will also refer to the \emph{AI decision pipeline}, or the process by which a model makes a decision about a given input, as the pipeline, differentiating between the creation and decision pipelines when necessary.\footnote{We will also interchangeably refer to the AI pipeline as the machine learning pipeline, training pipeline, or learning pipeline.} 
% While choices are often made along the creation pipeline in search of the most accurate possible model, as this paper and other recent work shows, many of the potential models that could be created among these choices are equally viable (i.e. have equivalent performance) in the given context, while displaying considerably different fairness behavior~\cite{black2022model,blackleave2021,marx2019,rodolfa2021empirical}. 

% This work aims to present the benefits of explicitly considering the creation pipeline in our conceptualization of, and mitigation of, fairness problems in AI systems, which we call a \emph{pipeline-based approach} to algorithmic fairness. We suggest that, while useful in many ways, the abstraction of fairness problems in the AI literature can narrow the field's perspective both on what can constitute unfair behavior, as well as on how unfair behavior can be mitigated in AI systems. By \emph{also} considering a pipeline-based approach in our fairness conceptualization and mitigation, we can uncover and prevent a wider variety of undesirable model behavior, as well as learn to use a larger array of techniques to prevent and stop unfair model behavior in practice. We suggest the pipeline-based approach to algorithmic fairness not as a replacement or improvement upon the literature to date, but rather as an additional, largely unexplored, toolbox. 

% \paragraph{Expanding Notions of Fairness: Procedural versus Outcomes-Based Fairness.} 
% By reducing the problem of unfairness to a question of inputs and outputs, we may narrow our perception of what unfair behavior means to only include those factors. By using a pipeline-based approach, we can uncover unfairness which may arise not only from a system's outcomes, but also by the process by which it reaches a given decision.  For example, a decision process may rely on attributes that seem normatively or legally dubious--- such as a recidivism prediction model which determines a defendant's ability to walk free between their arrest and their court date based on the criminal history of their parents and friends~\cite{angwin2016machine}. %An ad-targeting model might 
% %over-rely on spurious correlations to make its decisions—such as those between shopping habits and potential job qualifications~\cite{feat}. 
% Or, as we will explore in depth in this thesis, a decision process may be unfair because it is highly
% arbitrary or unstable—--such as a bank effectively flipping a coin to determine who gets a loan~\cite{blackleave2021}. Even if such models performed admirably on outcomes-based fairness measures, they may still be seen as unfair by many. Further, while the transportability between contexts which comes from abstraction is useful, as we explore in Chapter~\ref{chap:IRS}, this generality can come at a cost to specificity, thus at times harming the applicability of common fairness metrics in real-world contexts. %Contrastingly, using pipeline-based fairness \emph{interventions} can be more flexible to contextual model behavior requirements, as we 
% %More broadly, the focus on generalizability and abstraction in many fairness metrics may create pressure to only consider model behaviors which are \emph{always} undesirable as unfairness. However, the meaning of fair behavior varies greatly from context to context, and thus some behaviors which are unfair in one circumstance are perfectly acceptable in others (pick up on this?)

% %By explicitly considering the machine learning pipeline as we consider what behaviors may constitute unfair treatment in various contexts, we can recognize a larger variety of behaviors which may be unfair in certain contexts. 

% \paragraph{Pipeline-based Fairness Interventions.} This abstraction does not only exist in fairness definitions, but also in common unfairness mitigation techniques. %Perhaps influenced by the input-output view of the fairness problem, 
% Common fairness mitigation techniques 
% %often cast fairness desiderata as extra objectives in model optimization. That is, many common techniques to promote fairness 
% are often constructed as \emph{constraints} put on top of a model's decision or optimization process~\cite{agarwal2018reductions,hardtequality2016,zafar2017fairness-aistats}. This approach has many merits: abstracting the problem of fairness to an optimization constraint over a problem with inputs and outputs is the only way to make a fully generalizable solution to a given fairness problem. However, mitigating unfair behavior in this way obfuscates the choices made along the AI pipeline and their effect on the fairness behavior of the model---and thus the potential fairness benefits of changing some of these choices. As we demonstrate in this thesis, decisions made along the AI pipeline have a huge impact on model behavior, from influencing a model's individual predictions, to changing the distribution of the individuals it selects~\cite{feat,blackleave2021,blackIRS2022}. %cite IRS, feature-wise, LUF, future work,
% While these generalized methods of alleviating fairness problems are extremely useful, attacking fairness problems \emph{only} with these tools may leave some stones unturned.

% We can, in addition to using commonly available bias mitigation techniques, also explicitly investigate the choices made along the AI pipeline---even seemingly fairness-unrelated ones---as intervention points to improve model fairness behavior. Given that the decisions made along the AI pipeline determine a model and its behavior, if a model is acting unfairly, one way to change that behavior may be to change some choices made along its creation pipeline, rather than adding an additional constraint on top of the model.  For example, as we demonstrate in Chapter~\ref{chap:ensemble}, changing model type to an ensemble model over a singleton model can be preferable for fairness-related stability concerns. Or, as we show in Chapter~\ref{chap:IRS}, we can modify a model's prediction target to acheive fairness gains: in that case, changing from a classification to a regression model. 
% Given that, as we show in Chapter~\ref{chap:mod_mult}, there are often myriad equally viable (accurate) models for a given prediction task made with different pipelines, changing decisions made along the AI pipeline, as opposed to adding an additional constraint on top of a model's optimization or decision process, can also lead to fairness gains which come at a lower cost to performance. We demonstrate this phenomenon empirically in Chapter~\ref{chap:IRS}. Finally, as pipeline-based fairness interventions are not tied to any one definition of fairness, they can be more flexible to contextual model behavior requirements in real-world systems, as we explore in Chapter~\ref{chap:IRS} as well.


% As a whole, this thesis aims to show the immense flexibility that the AI creation pipeline gives practitioners with respect to how to reach the goals they set out to acheive with machine learning models---but also, how the choices made along the AI pipeline have to be carefully considered in terms of their impact on desired model behaviors, as even seemingly small choices can have a large impact.
% By considering all the choices made along the AI pipeline---from feature selection, to model type, to the objective functions---as places where changes can be made to improve fairness behavior, we can greatly expand our arsenal of unfairness-fighting tools.


% The rest of this work proceeds as follows:



==> versions/intro_1.tex <==

Algorithmic Fairness is no longer a nascent field. 
Through years of work from activists, journalists, researchers, and AI practitioners, professionals across industry, government, and the nonprofit sectors engage with, and rely on, algorithmic fairness expertise to guide their implementation of AI systems. While interest, and scholarship, is broad, algorithmic fairness often gets simplified and packaged into enforcing
mathematically abstracted fairness definitions onto
%statistical group-based fairness notions on a 
pre-made ML system, often through adding relevant constraints. While this approach is useful in certain contexts, many works over the years have pointed to the pitfalls of this approach [CITE HERE]: some have argued this one-size-fits all approach can exclude countless notions of what unfairness means, particularly ones that are especially relevant to the given application context [CITE], others have shown how details about the ML system---the data or model type used, or how the predictions are used in practice--render enforcing these definitions useless at best and harmful at worst. 

In this paper, we draw attention to an alternate approach to tackling algorithmic fairness problems, which we call \textit{pipeline fairness}. We argue that pipeline fairness is simply a name for a (dispersed) pattern of algorithmic fairness work that is ongoing, and holds promise for directing the field towards creating another set of useful tools for fighting fairness problems on the ground. In this work, we define the pipeline-based approach to fairness; collect and organize the work to date which uses this approach; and create a research agenda outlining the next steps required to create an pipeline-fairness based arsenal of techniques to address unfairness in practice. 
%but has not been collected under one umbrella---however, we argue it should be, due to its promise for directing the field towards creating another set of useful tools for fighting fairness problems on the ground. 


Notably, most formalizations of fairness in the AI literature abstract the problem of unfair model behavior to model inputs, model outputs, and the ground truth label. The most common fairness definitions, such as demographic parity, equalized false and/or true positive rates, and equal accuracy, can be expressed only with ``observed features V [i.e., input features], outcomes Y [i.e., ground truth labels] ... and decisions D [i.e., model outputs]''~\citep{mitchell2021algorithmic}. Even slightly less common notions, such as counterfactual fairness or individual fairness, are expressed as a constraint on model inputs and outputs in relation to additional information about the data distribution, such as a given similarity metric or causal graph~\cite{mitchell2021algorithmic}. 

This abstraction has many merits: abstraction leads to transportability, and so these definitions can be applied to a large variety of fairness problems. Further, these metrics can be easily computed and tested no matter the model implementation. Beyond these merits, in many contexts, such fairness definitions are also fundamentally important: for example, extreme demographic disparity is of legal consequence in areas such as hiring~\cite{griggs1971}. 

\paragraph{The AI Pipeline.} However, this abstracted view of fairness can draw attention away from the fact that each step made along the \emph{AI model creation pipeline} can influence the fairness of a model's behavior.
The process of creating AI models for a given application is complex: %, and can have a large impact on a model's fairness behavior. 
myriad choices are made during model creation, from the profound to the seemingly inconsequential. For example, in order to construct a loan decision model for a bank, a decision has to be made about how to translate the bank's objective, i.e., deciding who to grant loans to,  into a prediction target: e.g., predicting the probability of the client's default, or the amount of money gained by the bank per client, or something else entirely. Decisions also have to be made about how to use the available data, such as which features are to be used, and, if the data is unprocessed, how these features should be defined and constructed~\cite{passi2019problem}. %solon's paper about translation
On a lower level, model practitioners must decide what type of model will be used, the learning rule and objective function, the values of hyper-parameters determining normalization and training procedures, among many other decisions made continuously throughout model development~\cite{lehr2017playing, kim2022race}. All of these decisions then impact how the model is constructed, and therefore, how it makes its own decisions. 

In this work, we call this series of decisions model practitioners have to make the \emph{AI creation pipeline}, or the pipeline. 
%As the pipeline determines how models reach their decision-making schema, we will also refer to the \emph{AI decision pipeline}, or the process by which a model makes a decision about a given input, as the pipeline, differentiating between the creation and decision pipelines when necessary.\footnote{We will also interchangeably refer to the AI pipeline as the machine learning pipeline, training pipeline, or learning pipeline.} 
While choices are often made along the creation pipeline in search of the most accurate possible model, as this paper and other recent work shows, many of the potential models that could be created among these choices are equally viable (i.e. have equivalent performance) in the given context, while displaying considerably different fairness behavior~\cite{black2022model,blackleave2021,marx2019,rodolfa2021empirical}. 

This work aims to present the benefits of explicitly considering the creation pipeline in our conceptualization of, and mitigation of, fairness problems in AI systems, which we call a \emph{pipeline-based approach} to algorithmic fairness. We suggest that, while useful in many ways, the abstraction of fairness problems in the AI literature can narrow the field's perspective both on what can constitute unfair behavior, as well as on how unfair behavior can be mitigated in AI systems. By \emph{also} considering a pipeline-based approach in our fairness conceptualization and mitigation, we can uncover and prevent a wider variety of undesirable model behavior, as well as learn to use a larger array of techniques to prevent and stop unfair model behavior in practice. We suggest the pipeline-based approach to algorithmic fairness not as a replacement or improvement upon the literature to date, but rather as an additional, largely unexplored, toolbox. 

\paragraph{Expanding Notions of Fairness: Procedural versus Outcomes-Based Fairness.} 
By reducing the problem of unfairness to a question of inputs and outputs, we may narrow our perception of what unfair behavior means to only include those factors. By using a pipeline-based approach, we can uncover unfairness which may arise not only from a system's outcomes, but also by the process by which it reaches a given decision.  For example, a decision process may rely on attributes that seem normatively or legally dubious--- such as a recidivism prediction model which determines a defendant's ability to walk free between their arrest and their court date based on the criminal history of their parents and friends~\cite{angwin2016machine}. %An ad-targeting model might 
%over-rely on spurious correlations to make its decisions—such as those between shopping habits and potential job qualifications~\cite{feat}. 
Or, as we will explore in depth in this thesis, a decision process may be unfair because it is highly
arbitrary or unstable—--such as a bank effectively flipping a coin to determine who gets a loan~\cite{blackleave2021}. Even if such models performed admirably on outcomes-based fairness measures, they may still be seen as unfair by many. Further, while the transportability between contexts which comes from abstraction is useful, as we explore in Chapter~\ref{chap:IRS}, this generality can come at a cost to specificity, thus at times harming the applicability of common fairness metrics in real-world contexts. %Contrastingly, using pipeline-based fairness \emph{interventions} can be more flexible to contextual model behavior requirements, as we 
%More broadly, the focus on generalizability and abstraction in many fairness metrics may create pressure to only consider model behaviors which are \emph{always} undesirable as unfairness. However, the meaning of fair behavior varies greatly from context to context, and thus some behaviors which are unfair in one circumstance are perfectly acceptable in others (pick up on this?)

%By explicitly considering the machine learning pipeline as we consider what behaviors may constitute unfair treatment in various contexts, we can recognize a larger variety of behaviors which may be unfair in certain contexts. 

\paragraph{Pipeline-based Fairness Interventions.} This abstraction does not only exist in fairness definitions, but also in common unfairness mitigation techniques. %Perhaps influenced by the input-output view of the fairness problem, 
Common fairness mitigation techniques 
%often cast fairness desiderata as extra objectives in model optimization. That is, many common techniques to promote fairness 
are often constructed as \emph{constraints} put on top of a model's decision or optimization process~\cite{agarwal2018reductions,hardtequality2016,zafar2017fairness-aistats}. This approach has many merits: abstracting the problem of fairness to an optimization constraint over a problem with inputs and outputs is the only way to make a fully generalizable solution to a given fairness problem. However, mitigating unfair behavior in this way obfuscates the choices made along the AI pipeline and their effect on the fairness behavior of the model---and thus the potential fairness benefits of changing some of these choices. As we demonstrate in this thesis, decisions made along the AI pipeline have a huge impact on model behavior, from influencing a model's individual predictions, to changing the distribution of the individuals it selects~\cite{feat,blackleave2021,blackIRS2022}. %cite IRS, feature-wise, LUF, future work,
While these generalized methods of alleviating fairness problems are extremely useful, attacking fairness problems \emph{only} with these tools may leave some stones unturned.

We can, in addition to using commonly available bias mitigation techniques, also explicitly investigate the choices made along the AI pipeline---even seemingly fairness-unrelated ones---as intervention points to improve model fairness behavior. Given that the decisions made along the AI pipeline determine a model and its behavior, if a model is acting unfairly, one way to change that behavior may be to change some choices made along its creation pipeline, rather than adding an additional constraint on top of the model.  For example, as we demonstrate in Chapter~\ref{chap:ensemble}, changing model type to an ensemble model over a singleton model can be preferable for fairness-related stability concerns. Or, as we show in Chapter~\ref{chap:IRS}, we can modify a model's prediction target to acheive fairness gains: in that case, changing from a classification to a regression model. 
Given that, as we show in Chapter~\ref{chap:mod_mult}, there are often myriad equally viable (accurate) models for a given prediction task made with different pipelines, changing decisions made along the AI pipeline, as opposed to adding an additional constraint on top of a model's optimization or decision process, can also lead to fairness gains which come at a lower cost to performance. We demonstrate this phenomenon empirically in Chapter~\ref{chap:IRS}. Finally, as pipeline-based fairness interventions are not tied to any one definition of fairness, they can be more flexible to contextual model behavior requirements in real-world systems, as we explore in Chapter~\ref{chap:IRS} as well.


As a whole, this thesis aims to show the immense flexibility that the AI creation pipeline gives practitioners with respect to how to reach the goals they set out to acheive with machine learning models---but also, how the choices made along the AI pipeline have to be carefully considered in terms of their impact on desired model behaviors, as even seemingly small choices can have a large impact.
By considering all the choices made along the AI pipeline---from feature selection, to model type, to the objective functions---as places where changes can be made to improve fairness behavior, we can greatly expand our arsenal of unfairness-fighting tools.


The rest of this work proceeds as follows:

==> versions/intro_1_27.tex <==
\section{Introduction} 

% \begin{itemize}
%     \item Prevalence of ML harms, chief among them issues of unfairness
%     \item lots of work to deal with it by offering frameworks and mitigation strategies
%    , but this hasn't lead to concrete guidelines and tools
   
%     \item typical approach by researchers, practitioners, academia: select an adhoc method to ``fix'' fairness without understanding or knowing how this view will help with appropriate mitigation in practice.
    
    
%     \item Recently research community has honed in on the importance of a pipeline view of fairness
%     \item But it's not clear how this view will help with appropriate mitigation in pratice

%     \item To support the above, mention our documented experience as teachers and practitioners observing this issue first hand
%     \item our proposal: use a pipeline-centric view that can provide methodologies and tools to support a more structured and targeted approach to reducing harms that be caused by the use of ML systems 
%     \item: our goal: to work with the community to operationalize ... and create .... that can result in ...
%     \item our contributions here: toward this goal we do a systematic review of the relevant literature, offering a research agenda, and a set of requirements for tools and methodologies needed.
%     \item this is the first step toward a broader agenda in which we co-design guidelines and processes for students and practitioners to understand the ML pipeline/lifecycle to detect and mitigate harms appropriately.
% \end{itemize}

As AI systems have become more and more commonplace in public-facing contexts, we have seen a proliferation in the harms caused by such systems: from gender bias in hiring systems to racial bias in healthcare distribution systems~\cite{dastin2018amazon,obermeyer2019dissecting,buolamwini2018gender,compas}. Through years of work from activists, stakeholders, journalists, lawmakers, researchers, and AI practitioners, there now seems to be appetite for building systems in ways that prevent such harms~\cite{room2021executive,jobin2019global}. Recently, professionals across industry, government, and the nonprofit sectors have been turning to algorithmic fairness expertise to guide their implementation of AI systems~\cite{holstein2019improving}. 

While algorithmic fairness scholarship is broad, in practice, mitigating unfairness often gets simplified into enforcing a somewhat arbitrarily chosen fairness metric on top of a pre-made system, either by enforcing fairness constraints within the optimization function, post-processing model outputs, or occasionally by manipulating data to remove information about the protected attribute[CITE]. 
Many have begun to point to the weaknesses of this approach. Firstly, studies interviewing practitioners on the ground report feelings of anxiety about not choosing the correct metric for a given fairness issue~\cite{madaio2020co}. Once a metric is chosen, there are many technical drawbacks: Friedler et al.~\cite{friedler2019comparative} find that several common algorithms for mitigating bias are sensitive to small changes in training set-up such as train-test splits and preprocessing steps. Others find that the implementation structure of these techniques does not translate well to a variety of policy problems, which have complications such as only being able to select predictions up to a budget~\cite{black2022algorithmic, singh2022fair}. %Others still have pointed to the fact that these methods of enforcing fairness constraints on a static system do not guarantee the fairness of that system over time[CITE]. 
Some have even shown that naively enforcing fairness metrics, such as demographic parity, on data with certain types of label noise can decrease those very same metrics in the true population~\cite{wang2021fair}.

%More generally, this 
Many of these problems may stem from the fact that the
traditional approach to fairness 
%does not take into account a given model's end-to-end creation pipeline. Much of the fairness literature
is myopic---it hyper-focuses on mitigating bias through making changes at just a few places along the AI creation pipeline, namely, choice of optimization function, loss function, or particular aspects of data preprocessing. 
However, \emph{all} of the choices %made at each step of 
along the AI pipeline have impacts on a model’s behavior: problem formulation~\cite{passi2019problem}; data sampling, data labeling, data cleaning; feature creation, feature selection; hypothesis class, optimization function, regularizer and hyperparameter choice; the selection of evaluation metrics and pre-deployment validation; as well as human-machine handoff and other organizational intricacies. Thus, as prior works have noted~\cite{akpinar2022sandbox,suresh2021framework} we can leverage the pipeline to change and understand AI model behavior: if we believe a model is acting unfairly, certainly, one way to change that behavior is to change some choices we made along the way to making that model.

%By effectively ignoring the rest of the AI pipeline, 
By abstracting away the rest of the AI pipeline and enforcing a given metric on top of a system during training or prediction, the more mainstream approach ignores situations where we can actually isolate some of the \emph{sources} of bias----as they are a result of other choices made in the model-building process. 
Disregarding underlying sources of bias in the modeling setup and instead enforcing fairness metrics at training or prediction time can %Beyond potentially 
needlessly increasing a fairness-accuracy tradeoff due to intervening at the wrong place~\cite{black2022algorithmic}, or, at worst, 
%the traditional approach of simply adding a fairness constraint during training or prediction 
 ``[hide] the real problem while creating an illusion of
fairness''~\cite{akpinar2022sandbox}. 

Thus, we join others in suggesting it is often be preferable to take an alternate approach~\cite{akpinar2022sandbox,suresh2021framework}, which we call a pipeline-based approach to fairness. In a pipeline-based fairness approach, practitioners interrogate choices made at each step of the AI creation pipeline to search for ways in which these choices impact model fairness behavior, and then, when possible, change the relevant modeling choices to abate this effect. This process takes place iteratively after performing an intervention: the model will be tested again, until it is deemed satisfactory for deployment given its specific behavioral desiderata, whereupon testing and model updates will continue through deployment.
%And, importantly, it should reflect the lifecycle of the system: i.e. testing and updating continues during deployment.
Beyond the benefit of finding and directly tackling some of a model's sources of unfairness, a pipeline-based approach adheres to other calls for change within the discipline from the fairness literature. Interrogating a model's pipeline inherently forces a practitioner to enforcing fairness desiderata in a contextualized manner~\cite{}, and also responds to the call to build models with fairness in mind from the beginning~\cite{}. 

However, as rosy as a pipeline-based approach may sound, it is unclear how to  \emph{operationalize} a pipeline-based approach to fairness detection and mitigation: intuitively guessing what choices made along the pipeline may lead to bias is a difficult task even for those with specialized computer science knowledge. 
In fact, as we discuss in Section~\ref{sec:teaching}, we find that populations with highly specialized technical understanding, such as computer science PhD students, have difficulty conceptualizing what ML modeling choices may lead to bias, and how to mitigate bias that occurs along the pipeline.  Based on survey data from computer science (CS) PhD students enrolled in an algorithmic fairness class, we show that ..... \textcolor{red}{[Hoda and Rayid Here]}.
We suspect that given that computer science students with degrees in computer science cannot understand how to search for, and mitigate, bias as a result of ML modeling choices, practitioners making models in public-facing contexts find this difficult as well.

%To the authors knowledge, there are no toolkits or public code bases which help practitioners actively isolate, measure, and mitigate bias that occurs due to choices made along the pipeline. Indeed, there are challenges in creating such tools: due to its attention to the details of a given model's data and implementation, pipeline-based fairness techniques are hard to generalize, and therefore hard to create and implement in a generalized manner. 

Despite the difficulty in operationalizing a pipeline-based approach to bias detection and mitigation, it is becoming increasingly imperative to construct tools which do so. 
%Beyond the general impetus for tech companies in all applications to produce models as equitably as possible,
Recent developments from the Federal Trade Comission (FTC) and Consumer Finance Protection Bureau suggest an uptick in enforcement surrounding violations of the Disparate Impact Standard---allowing for more opportunities to replace biased systems with ones that produce less harm\footnote{Specifically, a recent advanced notice of proposed rulemaking (ANPR) from the Federal Trade Comission (FTC) suggests the possibility of stricter rules around the deployment of discriminatory systems~\cite{}.
One of the questions of the ANPR asks: "Should [the commission] consider new trade regulation rules that bar or somehow limit the deployment of any system that produces discrimination, irrespective of the data or processes on which those outcomes are based? ". Additionally, a recent update to the Consumer Finance Protection Bureau (CFPB) examination manuals  suggests discrimination can now be seen unfair as it’s defined under the Dodd-Frank Act, again suggesting a turn towards more enforcement of reducing discrimination in algorithmic systems: ''Discrimination may meet the criteria for ``unfairness'' by causing substantial harm to consumers that they cannot reasonably avoid, where that harm is not outweighed by countervailing benefits to consumers or competition.''~\cite{}}. 
%suggesting an uptick in litigation surrounding the Disparate Impact Standard, specifically around the possibility of \emph{less discriminatory alternative} models (LDAs). 
This means that companies which use machine learning systems relating to credit, housing, employment and other applications covered by the disparate impact standard may be more likely to be held legally responsible if a model is shown to be discriminatory. Additionally, if a \emph{less discriminatory alternative} (LDA)---an alternate model which meets business needs but displays less discriminatory behavior against protected groups--- is found, it may be legally required to use this model. 
%if an alternate model is discovered which meets business needs but displays less discriminatory behavior against protected groups.
As prior work surrounding model multiplicity has shown~\cite{black2022model}, there are often many models with equivalent accuracy for a given prediction task which differ in certain modeling choices~\cite{rodolfa2021empirical,blackleave2021, marx2019, semenova2019study}. 
%This fact is relevant to the search for LDAs, as it suggests that they may be relatively easy to find---given the correct tools.
This fact gives a point of leverage for technologically equipped plaintiffs to challenge discriminatory algorithms used in practice, and means it is in companies' interest to thoroughly explore the space of possible algorithms to find the least discriminatory one within those with sufficient business utility. 
However, to \emph{find} LDAs, we must have the correct tools.
Black et al.~\cite{black2022model} suggest a  pipeline-based approach to finding less discriminatory models in practice, by interrogating the pipeline to find the most effective places to search for interventions--however, as we have noted, no tools to instantiate such an approach currently exist.

A pipeline approach to fairness relies on a mapping of the relationships between choices made at each step of the \emph{AI pipeline} to its effects on a model's fairness behavior, for a given fairness goal. To the author's knowledge, this mapping is not something that exists in any level of detail at the moment, nor is housed in any specific place---examples of how modeling choices influence fairness behavior are few and far between in the literature in relation to traditional techniques, as this paper demonstrates. 
There are also few toolkits or public code bases which help practitioners actively isolate, measure, and mitigate bias that occurs due to choices made along the pipeline. Indeed, while there may be problems with the more traditional, myopic approach to bias mitigation, it is much more easily available to implement~\cite{AIF360,bird2020fairlearn,hardt2021amazon}.
%Indeed, there are challenges in creating such tools: due to its attention to the details of a given model's data and implementation, pipeline-based fairness techniques are hard to generalize, and therefore hard to create and implement in a generalized manner. 


%Importantly, those modeling choices are often practically changeable. While modeling choices are often made in search of the most accurate possible model, recent work has shown that there are usually many potential models--made with different modeling choices---with equivalent performance that can be created for any given prediction problem, while displaying considerably different fairness behavior~\cite{black2022model,blackleave2021,marx2019,rodolfa2021empirical,semenova2019study}. Thus, it may often be the case that changing relevant modeling choices can mitigate bias at a decreased cost to other performance metrics, or indeed, may even improve the model~\cite{black2022algorithmic}.


The goals of this paper are  threefold: first, to collect and synthesize the fairness literature that embodies the pipeline fairness approach, in an attempt to map out which areas of the pipeline are better understood, and which are less; secondly, to create a research agenda for filling out our map of how modeling choices can lead to fairness pitfalls, in service of our third goal of  creating (a first version of) a tool for practitioners to access the work currently available for detecting, measuring, and mitigating harm along the AI pipeline. 
This paper is the first step toward a broader agenda in which we co-design guidelines and processes for students and practitioners to understand the ML pipeline and lifecycle to detect and mitigate harms appropriately.

The rest of this paper proceeds as follows: in Section~\ref{sec:pipfair}, we define the AI pipeline and pipeline fairness in detail. In Section~\ref{sec:teaching}, we outline how our collective experience teaching classes on algorithmic fairness has shed light on some of the challenges to understanding, and by extension, operationalizing, a pipeline-based approach to fairness. Next, in 
Section~\ref{sec:litreview}, we categorize the fairness literature (fairness papers from top five fairness and ML conferences from the past five years) from the perspective of pipeline fairness, and point out areas where there has been less and more attention, and finally, in Section~\ref{sec:agenda}, we construct our research agenda for a fuller understanding of pipeline fairness moving forward, and describe our first instantiation of our pipeline-based bias mitigation toolkit.



==> versions/intro_2.tex <==
Algorithmic fairness is no longer a nascent field. Through years of work from activists, journalists, researchers, and AI practitioners, professionals across industry, government, and the nonprofit sectors rely on algorithmic fairness expertise to guide their implementation of AI systems. 

However, while algorithmic fairness scholarship is broad, in practice, it often gets simplified into enforcing
a mathematically abstracted definition of fairness on top of a pre-made system, either by enforcing fairness constraints within the optimization function, post-processing model outputs, or occasionally by manipulating data. Indeed, as this paper points out, the plurality of fairness research falls into either creating abstracted definitions to enforce, or finding ways to enforce a fairness constraint on top of an already constructed system. 

Most formalizations of fairness in the AI literature abstract the problem of unfair model behavior to just model inputs, model outputs, and the ground truth label. The most common fairness definitions, such as demographic parity, equalized false and/or true positive rates, and equal accuracy, can be expressed only with ``observed features V [i.e., input features], outcomes Y [i.e., ground truth labels] ... and decisions D [i.e., model outputs]''~\citep{mitchell2021algorithmic}. Even slightly less common notions, such as counterfactual fairness or individual fairness, are expressed as a constraint on model inputs and outputs in relation to additional information about the data distribution, such as a given similarity metric or causal graph~\cite{mitchell2021algorithmic}. 

This level of abstraction has many merits: abstraction to basic elements of a system leads to transportability, and so these definitions can be applied to a large variety of fairness problems. Further, these metrics can be easily computed and tested no matter the model implementation. Beyond these merits, in many contexts, such fairness definitions are also fundamentally important: for example, extreme demographic disparity is of legal consequence in areas such as hiring~\cite{griggs1971}. 

However, as countless others have pointed out[CITE], this abstracted approach has pitfalls, often based on the fact it does not pay attention to the details of the system over which it is enforced. Indeed, details about the AI system and its context---such as the data or model type used, or how the predictions are used in practice-- can even render enforcing these definitions harmful from an equity standpoint [cite]. Additionally, the most commonly used approaches for enforcing fairness constraints in practice, have been shown to be ill-suited for problems on the ground~\cite{}, or brittle~\cite{haverfordladysorell}.

More broadly, this abstracted approach inherently ignores situations where sources of bias are embedded in choices made in the model-building process, i.e., the choices made along the \emph{AI pipeline}. In these situations, fairness problems may be mitigated by changing certain modeling choices, i.e. via a targeted intervention, rather than by adding a constraint on top of a model. In some cases, taking such an approach can also reduce the oft-discussed fairness-performance tradeoff.


Importantly, those modeling choices are often practically changeable. While modeling choices are often made in search of the most accurate possible model, recent work has shown that there are usually many potential models--made with different modeling choices---with equivalent performance that can be created for any given prediction problem, while displaying considerably different fairness behavior~\cite{black2022model,blackleave2021,marx2019,rodolfa2021empirical}.
%More broadly, this abstracted approach inherently ignores situations where a root cause of bias is embedded in lower-level modeling choices of the system: and thus, may be mitigated by changing that modeling choice. 

\paragraph{The AI Pipeline.} The abstraction-based view of fairness can draw attention away from the fact that each step made along the \emph{AI model creation pipeline} can influence the fairness of a model's behavior.
The process of creating AI models for a given application is complex:
myriad choices are made during model creation, from the profound to the seemingly inconsequential. For example, in order to construct a loan decision model for a bank, a decision has to be made about how to translate the bank's objective, i.e., deciding who to grant loans to,  into a prediction target: e.g., predicting the probability of the client's default, or the amount of money gained by the bank per client, or something else entirely, also known as \emph{problem formulation}. The data to train the model has to be chosen, including choices about how to sample, label, and link data; how to construct features from available information for use in the model, and which of the constructed features to for prediction.  On a lower level, model practitioners must decide what type of model will be used, the learning rule and objective function, regularizers, the values of hyper-parameters determining normalization and training procedures, how the dataset will be split into train-test- and validation folds, among many other decisions made continuously throughout model development~\cite{lehr2017playing, kim2022race}. Practitioners will also have to decide what performance metrics will be used to evaluate models, and finally, how the model will be used in practice (e.g., with or without human involvement, how model predictions will be communicated and integrated into a larger decision system). (We define the steps of the AI pipeline in more detail in Section~\ref{pipeline}). 
All of these decisions then impact how it makes its own decisions, and thus its prediction behavior. 

%Importantly, those modeling choices are often practically changeable. While modeling choices are often made in search of the most accurate possible model, recent work has shown that there are usually many potential models--made with different modeling choices---with equivalent performance that can be created for any given prediction problem, while displaying considerably different fairness behavior~\cite{black2022model,blackleave2021,marx2019,rodolfa2021empirical}. 

In this paper, we draw attention to an alternate approach to tackling algorithmic fairness problems, which we call \textit{pipeline fairness}. A pipeline approach to fairness relies on mapping the relationships between choices made at each step of the \emph{AI pipeline} to its effects on a model's fairness behavior, for a given fairness goal. 


By approaching bias mitigation through changing a modeling choice rather than adding an additional 

Thus, completely abstracting fairness problems---and in so doing, ignoring modeling choices when tackling fairness issues--- can lead to ignoring situations where direct interventions on the root cause of bias can be performed, rather than placing a constraint on top of a system. Taking the approach of ignoring the underlying system and adding constraints on top of a model can (sometimes unnecessarily) introduce ``fairness’’-performance tradeoffs. 
Sometimes (but rarely), the (only) way to mitigate bias in a system is to add constraints on top of a model to force it to adhere to a given notion of fairness. 
However, often, there are decisions made during the system building process that exacerbate unfair behavior. 






% %Algorithmic Fairness is no longer a nascent field. 
% While interest in, and scholarship of, algorithmic fairness is broad, it often gets simplified, and packaged in practice, into simply enforcing
% mathematically abstracted fairness definitions onto
% %statistical group-based fairness notions on a 
% pre-made ML system, often through adding relevant constraints. 

% Notably, most formalizations of fairness in the AI literature abstract the problem of unfair model behavior to model inputs, model outputs, and the ground truth label. The most common fairness definitions, such as demographic parity, equalized false and/or true positive rates, and equal accuracy, can be expressed only with ``observed features V [i.e., input features], outcomes Y [i.e., ground truth labels] ... and decisions D [i.e., model outputs]''~\citep{mitchell2021algorithmic}. Even slightly less common notions, such as counterfactual fairness or individual fairness, are expressed as a constraint on model inputs and outputs in relation to additional information about the data distribution, such as a given similarity metric or causal graph~\cite{mitchell2021algorithmic}. 

% This abstraction has many merits: abstraction to basic elements of a system leads to transportability, and so these definitions can be applied to a large variety of fairness problems. Further, these metrics can be easily computed and tested no matter the model implementation. Beyond these merits, in many contexts, such fairness definitions are also fundamentally important: for example, extreme demographic disparity is of legal consequence in areas such as hiring~\cite{griggs1971}. 


% While this abstracted approach is useful in certain contexts, many works over the years have pointed to its pitfalls [CITE HERE]: some have argued that enforcing abstract definitions on top of a pre-made system  can exclude countless notions of what unfairness means, particularly ones that are especially relevant to the given application context [CITE], others have shown how details about the ML system---the data or model type used, or how the predictions are used in practice--render enforcing these definitions useless at best and harmful at worst. 

% Indeed, 

% Through years of work from activists, journalists, researchers, and AI practitioners, professionals across industry, government, and the nonprofit sectors engage with, and rely on, algorithmic fairness expertise to guide their implementation of AI systems.



% While this approach is useful in certain contexts, many works over the years have pointed to the pitfalls of this approach [CITE HERE]: some have argued this one-size-fits all approach can exclude countless notions of what unfairness means, particularly ones that are especially relevant to the given application context [CITE], others have shown how details about the ML system---the data or model type used, or how the predictions are used in practice--render enforcing these definitions useless at best and harmful at worst. 

% In this paper, we draw attention to an alternate approach to tackling algorithmic fairness problems, which we call \textit{pipeline fairness}. We argue that pipeline fairness is simply a name for a (dispersed) pattern of algorithmic fairness work that is ongoing, and holds promise for directing the field towards creating another set of useful tools for fighting fairness problems on the ground. In this work, we define the pipeline-based approach to fairness; collect and organize the work to date which uses this approach; and create a research agenda outlining the next steps required to create an pipeline-fairness based arsenal of techniques to address unfairness in practice. 
% %but has not been collected under one umbrella---however, we argue it should be, due to its promise for directing the field towards creating another set of useful tools for fighting fairness problems on the ground. 



 

% In this work, we call this series of decisions model practitioners have to make the \emph{AI creation pipeline}, or the pipeline. 
% %As the pipeline determines how models reach their decision-making schema, we will also refer to the \emph{AI decision pipeline}, or the process by which a model makes a decision about a given input, as the pipeline, differentiating between the creation and decision pipelines when necessary.\footnote{We will also interchangeably refer to the AI pipeline as the machine learning pipeline, training pipeline, or learning pipeline.} 
% While choices are often made along the creation pipeline in search of the most accurate possible model, as this paper and other recent work shows, many of the potential models that could be created among these choices are equally viable (i.e. have equivalent performance) in the given context, while displaying considerably different fairness behavior~\cite{black2022model,blackleave2021,marx2019,rodolfa2021empirical}. 

% This work aims to present the benefits of explicitly considering the creation pipeline in our conceptualization of, and mitigation of, fairness problems in AI systems, which we call a \emph{pipeline-based approach} to algorithmic fairness. We suggest that, while useful in many ways, the abstraction of fairness problems in the AI literature can narrow the field's perspective both on what can constitute unfair behavior, as well as on how unfair behavior can be mitigated in AI systems. By \emph{also} considering a pipeline-based approach in our fairness conceptualization and mitigation, we can uncover and prevent a wider variety of undesirable model behavior, as well as learn to use a larger array of techniques to prevent and stop unfair model behavior in practice. We suggest the pipeline-based approach to algorithmic fairness not as a replacement or improvement upon the literature to date, but rather as an additional, largely unexplored, toolbox. 

% \paragraph{Expanding Notions of Fairness: Procedural versus Outcomes-Based Fairness.} 
% By reducing the problem of unfairness to a question of inputs and outputs, we may narrow our perception of what unfair behavior means to only include those factors. By using a pipeline-based approach, we can uncover unfairness which may arise not only from a system's outcomes, but also by the process by which it reaches a given decision.  For example, a decision process may rely on attributes that seem normatively or legally dubious--- such as a recidivism prediction model which determines a defendant's ability to walk free between their arrest and their court date based on the criminal history of their parents and friends~\cite{angwin2016machine}. %An ad-targeting model might 
% %over-rely on spurious correlations to make its decisions—such as those between shopping habits and potential job qualifications~\cite{feat}. 
% Or, as we will explore in depth in this thesis, a decision process may be unfair because it is highly
% arbitrary or unstable—--such as a bank effectively flipping a coin to determine who gets a loan~\cite{blackleave2021}. Even if such models performed admirably on outcomes-based fairness measures, they may still be seen as unfair by many. Further, while the transportability between contexts which comes from abstraction is useful, as we explore in Chapter~\ref{chap:IRS}, this generality can come at a cost to specificity, thus at times harming the applicability of common fairness metrics in real-world contexts. %Contrastingly, using pipeline-based fairness \emph{interventions} can be more flexible to contextual model behavior requirements, as we 
% %More broadly, the focus on generalizability and abstraction in many fairness metrics may create pressure to only consider model behaviors which are \emph{always} undesirable as unfairness. However, the meaning of fair behavior varies greatly from context to context, and thus some behaviors which are unfair in one circumstance are perfectly acceptable in others (pick up on this?)

% %By explicitly considering the machine learning pipeline as we consider what behaviors may constitute unfair treatment in various contexts, we can recognize a larger variety of behaviors which may be unfair in certain contexts. 

% \paragraph{Pipeline-based Fairness Interventions.} This abstraction does not only exist in fairness definitions, but also in common unfairness mitigation techniques. %Perhaps influenced by the input-output view of the fairness problem, 
% Common fairness mitigation techniques 
% %often cast fairness desiderata as extra objectives in model optimization. That is, many common techniques to promote fairness 
% are often constructed as \emph{constraints} put on top of a model's decision or optimization process~\cite{agarwal2018reductions,hardtequality2016,zafar2017fairness-aistats}. This approach has many merits: abstracting the problem of fairness to an optimization constraint over a problem with inputs and outputs is the only way to make a fully generalizable solution to a given fairness problem. However, mitigating unfair behavior in this way obfuscates the choices made along the AI pipeline and their effect on the fairness behavior of the model---and thus the potential fairness benefits of changing some of these choices. As we demonstrate in this thesis, decisions made along the AI pipeline have a huge impact on model behavior, from influencing a model's individual predictions, to changing the distribution of the individuals it selects~\cite{feat,blackleave2021,blackIRS2022}. %cite IRS, feature-wise, LUF, future work,
% While these generalized methods of alleviating fairness problems are extremely useful, attacking fairness problems \emph{only} with these tools may leave some stones unturned.

% We can, in addition to using commonly available bias mitigation techniques, also explicitly investigate the choices made along the AI pipeline---even seemingly fairness-unrelated ones---as intervention points to improve model fairness behavior. Given that the decisions made along the AI pipeline determine a model and its behavior, if a model is acting unfairly, one way to change that behavior may be to change some choices made along its creation pipeline, rather than adding an additional constraint on top of the model.  For example, as we demonstrate in Chapter~\ref{chap:ensemble}, changing model type to an ensemble model over a singleton model can be preferable for fairness-related stability concerns. Or, as we show in Chapter~\ref{chap:IRS}, we can modify a model's prediction target to acheive fairness gains: in that case, changing from a classification to a regression model. 
% Given that, as we show in Chapter~\ref{chap:mod_mult}, there are often myriad equally viable (accurate) models for a given prediction task made with different pipelines, changing decisions made along the AI pipeline, as opposed to adding an additional constraint on top of a model's optimization or decision process, can also lead to fairness gains which come at a lower cost to performance. We demonstrate this phenomenon empirically in Chapter~\ref{chap:IRS}. Finally, as pipeline-based fairness interventions are not tied to any one definition of fairness, they can be more flexible to contextual model behavior requirements in real-world systems, as we explore in Chapter~\ref{chap:IRS} as well.


% As a whole, this thesis aims to show the immense flexibility that the AI creation pipeline gives practitioners with respect to how to reach the goals they set out to acheive with machine learning models---but also, how the choices made along the AI pipeline have to be carefully considered in terms of their impact on desired model behaviors, as even seemingly small choices can have a large impact.
% By considering all the choices made along the AI pipeline---from feature selection, to model type, to the objective functions---as places where changes can be made to improve fairness behavior, we can greatly expand our arsenal of unfairness-fighting tools.


% The rest of this work proceeds as follows:

==> versions/intro_3.tex <==
\section{Introduction} 

%Algorithmic fairness is no longer a nascent field. Through years of work from activists, journalists, researchers, and AI practitioners, professionals across industry, government, and the nonprofit sectors rely on algorithmic fairness expertise to guide their implementation of AI systems. However, while algorithmic fairness scholarship is broad, in practice, it often gets simplified into enforcing
%a mathematically abstracted definition of fairness on top of a pre-made system, either by enforcing fairness constraints within the optimization function, post-processing model outputs, or occasionally by manipulating data. Indeed, as this paper points out, the plurality of fairness research falls into either creating abstracted definitions to enforce, or finding ways to enforce a fairness constraint on top of an already constructed system. 

Faithful to its roots within computer science literature, many well-known conceptions of algorithmic fairness are highly abstracted from the details of any one system implementation. Most formalizations of fairness in the AI literature abstract the problem of unfair model behavior to generic model inputs, model outputs, and the ground truth label. The most common fairness definitions, such as demographic parity, equalized false and/or true positive rates, and equal accuracy, can be expressed only with ``observed features V [i.e., input features], outcomes Y [i.e., ground truth labels] ... and decisions D [i.e., model outputs]''~\citep{mitchell2021algorithmic}. Even slightly less common notions, such as counterfactual fairness or individual fairness, are expressed as a constraint on model inputs and outputs in relation to additional information about the data distribution, such as a given similarity metric or causal graph~\cite{mitchell2021algorithmic}. 

This level of abstraction has many merits: abstraction to basic elements of a system leads to transportability across implementations, and so these definitions, and the methods used to enforce them, can be applied to fairness problems in a variety of application contexts. Further, the abstraction of these metrics adds to their simplicity, so they can be easily intuited and computed. Beyond these merits, in many contexts, such fairness definitions are also fundamentally important: for example, extreme demographic disparity is of legal consequence in areas such as hiring~\cite{griggs1971}. 

However, as countless others have pointed out[CITE], %this abstracted approach has pitfalls, 
the approach of enforcing an abstracted definition on top of a pre-built machine learning system has pitfalls---
often based on the fact it does not pay attention to the details of the system over which it is enforced. Indeed, details about the AI system and its context---such as the data or model type used, or how the predictions are used in practice-- can even render enforcing these definitions harmful from an equity standpoint [cite]. %Additionally, the most commonly used approaches for enforcing fairness constraints in practice, have been shown to be ill-suited for problems on the ground~\cite{}, or brittle~\cite{haverfordladysorell}.
More broadly, this abstracted approach inherently ignores situations where sources of bias are embedded in choices made in the model-building process, i.e., the choices made along the \emph{AI pipeline}. In these situations, fairness problems may be mitigated by \emph{changing} certain modeling choices, i.e. via a targeted intervention, rather than by adding a constraint on top of a model. In some cases, taking such an approach can also reduce the oft-discussed fairness-performance tradeoff.

In this paper, we draw attention to an alternate approach to tackling algorithmic fairness problems, which we call \textit{pipeline fairness}. In pipeline-based fairness, practitioners interrogate choices made at each step of the AI creation pipeline to search for ways in which these choices impact model fairness behavior, and then, when possible, change the relevant modeling choices to abate this effect. 
%This technique is inherently contextualized to a model's specific application and implementation; it promotes building systems with equity in 
%This technique takes into account many principles that the algorithmic fairness community has suggested for building systems as equitably as possible, such as, building with equity in mind from the beginning, and creating contextualized fairness interventions. (should go elsewhere)
Importantly, we suggest the pipeline-based approach to algorithmic fairness not as a replacement or improvement upon the literature to date, but rather as an additional, largely unexplored, toolbox, which holds promise for expanding our ability to tackle fairness problems on the ground.

Thus, a pipeline approach to fairness relies on a mapping of the relationships between choices made at each step of the \emph{AI pipeline} to its effects on a model's fairness behavior, for a given fairness goal. This mapping is not something that exists in any level of detail at the moment, nor is housed in any specific place---examples of how modeling choices influence fairness behavior are few and far between in the literature in relation to abstraction-based techniques, as this paper demonstrates. 
The goals of this paper is threefold: first, to define, and draw attention to, a pipeline-based approach to algorithmic fairness; second, to collect and synthesize the fairness literature that embodies this approach, in an attempt to map out which areas of the pipeline are better understood, and which are less; and finally, to create a research agenda for filling out our map of how modeling choices can lead to fairness pitfalls, in service of creating a robust roadmap for practitioners of how we can build systems as free from bias as possible.%, drawing from examples

%\textbf{The goal of this paper is to show 
%what parts of this mapping have received attention, which are relatively untouched, and outline a research agenda to collaboratively can leverage the information and techniques we have to develop a full understanding of pipeline fairness.}

\subsection{Pipeline Fairness}

\paragraph{The AI Pipeline.} 
%The abstraction-based view of fairness can draw attention away from the fact that each step made along the \emph{AI model creation pipeline} can influence the fairness of a model's behavior.
To understand pipeline fairness, we need to understand the AI pipeline, or the process of creating an AI model for a given application. 
%The process of creating AI models for a given application 
This process is complex:
myriad choices are made during model creation, from the profound to the seemingly inconsequential. For example, in order to construct a loan decision model for a bank, a decision has to be made about how to translate the bank's objective, i.e., deciding who to grant loans to,  into a prediction target: e.g., predicting the probability of the client's default, or the amount of money gained by the bank per client, or something else entirely, also known as \emph{problem formulation}. The data to train the model has to be chosen, including choices about how to sample, label, and link data; how to construct features from available information for use in the model, and which of the constructed features to for prediction.  On a lower level, model practitioners must decide what type of model will be used, the learning rule and objective function, regularizers, the values of hyper-parameters determining normalization and training procedures, how the dataset will be split into train-test- and validation folds, among many other decisions made continuously throughout model development~\cite{lehr2017playing, kim2022race}. Practitioners will also have to decide what performance metrics will be used to evaluate models, and finally, how the model will be used in practice (e.g., with or without human involvement, how model predictions will be communicated and integrated into a larger decision system). (We define the steps of the AI pipeline in more detail in Section~\ref{pipeline}). 
All of these decisions then impact how it makes its own decisions, and thus its prediction behavior. 

\paragraph{Pipeline Fairness}
A pipeline-based view of fairness, then, considers each step of the AI pipeline as an intervention point to achieve a given fairness goal---and considers the effects of each choice during model creation on system behavior.
Importantly, those modeling choices are often practically changeable. While modeling choices are often made in search of the most accurate possible model, recent work has shown that there are usually many potential models--made with different modeling choices---with equivalent performance that can be created for any given prediction problem, while displaying considerably different fairness behavior~\cite{black2022model,blackleave2021,marx2019,rodolfa2021empirical}.

\paragraph{Benefits of Pipeline Fairness}
The pipeline approach to fairness is a method of augmenting our understanding of how to address fairness problems, not replacing the current most popular methods. 
Firstly, the pipeline approach to fairness can often unearth root causes of bias in a system, and thus point directly to mitigation techniques: e.g., if a faulty prediction target is chosen for a problem, choosing a different one can decrease discrimination~\cite{obermeyer2019dissecting,black}. Additionally, since the anti-bias intervention directly targets a source of bias, instead of putting an additional constraint on top of the system, this can lead to mitigation techniques that have lower performance-accuracy tradeoffs than abstraction-based methods~\cite{irs}. 
Further, while pipeline-based fairness mitigation is separate from creating definitions of fairness, many have pointed out that not all fairness problems are encapsulated by these abstracted, largely input/output based ideas of fairness. 
By reducing the problem of unfairness to a question of inputs and outputs, we may narrow our perception of what unfair behavior means to only include those factors. By using a pipeline-based approach, may naturally uncover unfairness which may arise not only from a system's outcomes, but also by the process by which it reaches a given decision. For example, a decision process may rely on attributes that seem normatively or legally dubious--- such as a recidivism prediction model which determines a defendant's ability to walk free between their arrest and their court date based on the criminal history of their parents and friends~\cite{angwin2016machine}; or a decision process may be unfair because it is highly
arbitrary or unstable—--such as a bank effectively flipping a coin to determine who gets a loan~\cite{blackleave2021}.
Further, while the transportability between contexts which comes from abstraction is useful, this generality can come at a cost to specificity, thus at times harming the applicability of common fairness metrics in real-world contexts---paying attention to the details of the system as pipeline fairness requires can also serve as a method of unearthing more contexutalized notions of fairness.

We note that ``pipeline fairness'' is simply a name for a mode of investigation that has already been underway in the algorithmic fairness literature since its inception---however, to the author's knowledge, there is no explicit paper tying the dispersed works that leverage the AI pipeline for fairness interventions together, connecting and collecting them under one roof. The goal of this paper is to do so, drawing attention to the phenomenon of pipeline fairness, as we believe that this technique is a promising future direction for expanding the algorithmic fairness toolbox, and deserves the focus and attention of the academic community. 

The main contributions of this paper are :
\begin{itemize}
    \item Defining pipeline fairness
    \item Synthesizing the work on pipeline fairness to date in the literature in a community-updatable document 
    \item Creating a research agenda in order to flesh out our understanding of how modeling choices along the pipeline impact fairness behavior of AI systems, so that we may guide practitioners through creating more equitable systems in the future.
\end{itemize}

The rest of this paper proceeds as follows: in Section~\ref{sec:pipfair}, we define the AI pipeline and pipeline fairness in detail. In Section~\ref{sec:litreview}, we categorize the fairness literature (fairness papers from top 4 ML conferences from the past five years) from the perspective of pipeline fairness, and point out areas where there has been less and more attention, and finally, in Section~\ref{sec:agenda}, we construct our research agenda for a fuller understanding of pipeline fairness moving forward.

As a whole, this work aims to show the immense flexibility that the AI creation pipeline gives practitioners with respect to how to reach the goals they set out to acheive with machine learning models---but also, how the choices made along the AI pipeline have to be carefully considered in terms of their impact on desired model behaviors, as even seemingly small choices can have a large impact.

We hope that together as a research community, we can learn to leverage all the choices made along the AI pipeline---from feature selection, to model type, to the objective functions---as places where decision can be made to improve fairness behavior, we thus greatly expand our arsenal of unfairness-fighting tools.



%More broadly, considering more aspects of the modeling process as an intervention point simp

%More broadly, this abstracted approach inherently ignores situations where a root cause of bias is embedded in lower-level modeling choices of the system: and thus, may be mitigated by changing that modeling choice. 

%Importantly, those modeling choices are often practically changeable. While modeling choices are often made in search of the most accurate possible model, recent work has shown that there are usually many potential models--made with different modeling choices---with equivalent performance that can be created for any given prediction problem, while displaying considerably different fairness behavior~\cite{black2022model,blackleave2021,marx2019,rodolfa2021empirical}. 

%In this paper, we draw attention to an alternate approach to tackling algorithmic fairness problems, which we call \textit{pipeline fairness}. A pipeline approach to fairness relies on mapping the relationships between choices made at each step of the \emph{AI pipeline} to its effects on a model's fairness behavior, for a given fairness goal. 


% By approaching bias mitigation through changing a modeling choice rather than adding an additional 

% Thus, completely abstracting fairness problems---and in so doing, ignoring modeling choices when tackling fairness issues--- can lead to ignoring situations where direct interventions on the root cause of bias can be performed, rather than placing a constraint on top of a system. Taking the approach of ignoring the underlying system and adding constraints on top of a model can (sometimes unnecessarily) introduce ``fairness’’-performance tradeoffs. 
% Sometimes (but rarely), the (only) way to mitigate bias in a system is to add constraints on top of a model to force it to adhere to a given notion of fairness. 
% However, often, there are decisions made during the system building process that exacerbate unfair behavior. 






% %Algorithmic Fairness is no longer a nascent field. 
% While interest in, and scholarship of, algorithmic fairness is broad, it often gets simplified, and packaged in practice, into simply enforcing
% mathematically abstracted fairness definitions onto
% %statistical group-based fairness notions on a 
% pre-made ML system, often through adding relevant constraints. 

% Notably, most formalizations of fairness in the AI literature abstract the problem of unfair model behavior to model inputs, model outputs, and the ground truth label. The most common fairness definitions, such as demographic parity, equalized false and/or true positive rates, and equal accuracy, can be expressed only with ``observed features V [i.e., input features], outcomes Y [i.e., ground truth labels] ... and decisions D [i.e., model outputs]''~\citep{mitchell2021algorithmic}. Even slightly less common notions, such as counterfactual fairness or individual fairness, are expressed as a constraint on model inputs and outputs in relation to additional information about the data distribution, such as a given similarity metric or causal graph~\cite{mitchell2021algorithmic}. 

% This abstraction has many merits: abstraction to basic elements of a system leads to transportability, and so these definitions can be applied to a large variety of fairness problems. Further, these metrics can be easily computed and tested no matter the model implementation. Beyond these merits, in many contexts, such fairness definitions are also fundamentally important: for example, extreme demographic disparity is of legal consequence in areas such as hiring~\cite{griggs1971}. 


% While this abstracted approach is useful in certain contexts, many works over the years have pointed to its pitfalls [CITE HERE]: some have argued that enforcing abstract definitions on top of a pre-made system  can exclude countless notions of what unfairness means, particularly ones that are especially relevant to the given application context [CITE], others have shown how details about the ML system---the data or model type used, or how the predictions are used in practice--render enforcing these definitions useless at best and harmful at worst. 

% Indeed, 

% Through years of work from activists, journalists, researchers, and AI practitioners, professionals across industry, government, and the nonprofit sectors engage with, and rely on, algorithmic fairness expertise to guide their implementation of AI systems.



% While this approach is useful in certain contexts, many works over the years have pointed to the pitfalls of this approach [CITE HERE]: some have argued this one-size-fits all approach can exclude countless notions of what unfairness means, particularly ones that are especially relevant to the given application context [CITE], others have shown how details about the ML system---the data or model type used, or how the predictions are used in practice--render enforcing these definitions useless at best and harmful at worst. 

% In this paper, we draw attention to an alternate approach to tackling algorithmic fairness problems, which we call \textit{pipeline fairness}. We argue that pipeline fairness is simply a name for a (dispersed) pattern of algorithmic fairness work that is ongoing, and holds promise for directing the field towards creating another set of useful tools for fighting fairness problems on the ground. In this work, we define the pipeline-based approach to fairness; collect and organize the work to date which uses this approach; and create a research agenda outlining the next steps required to create an pipeline-fairness based arsenal of techniques to address unfairness in practice. 
% %but has not been collected under one umbrella---however, we argue it should be, due to its promise for directing the field towards creating another set of useful tools for fighting fairness problems on the ground. 



 

% In this work, we call this series of decisions model practitioners have to make the \emph{AI creation pipeline}, or the pipeline. 
% %As the pipeline determines how models reach their decision-making schema, we will also refer to the \emph{AI decision pipeline}, or the process by which a model makes a decision about a given input, as the pipeline, differentiating between the creation and decision pipelines when necessary.\footnote{We will also interchangeably refer to the AI pipeline as the machine learning pipeline, training pipeline, or learning pipeline.} 
% While choices are often made along the creation pipeline in search of the most accurate possible model, as this paper and other recent work shows, many of the potential models that could be created among these choices are equally viable (i.e. have equivalent performance) in the given context, while displaying considerably different fairness behavior~\cite{black2022model,blackleave2021,marx2019,rodolfa2021empirical}. 

% This work aims to present the benefits of explicitly considering the creation pipeline in our conceptualization of, and mitigation of, fairness problems in AI systems, which we call a \emph{pipeline-based approach} to algorithmic fairness. We suggest that, while useful in many ways, the abstraction of fairness problems in the AI literature can narrow the field's perspective both on what can constitute unfair behavior, as well as on how unfair behavior can be mitigated in AI systems. By \emph{also} considering a pipeline-based approach in our fairness conceptualization and mitigation, we can uncover and prevent a wider variety of undesirable model behavior, as well as learn to use a larger array of techniques to prevent and stop unfair model behavior in practice. We suggest the pipeline-based approach to algorithmic fairness not as a replacement or improvement upon the literature to date, but rather as an additional, largely unexplored, toolbox. 

% \paragraph{Expanding Notions of Fairness: Procedural versus Outcomes-Based Fairness.} 
% By reducing the problem of unfairness to a question of inputs and outputs, we may narrow our perception of what unfair behavior means to only include those factors. By using a pipeline-based approach, we can uncover unfairness which may arise not only from a system's outcomes, but also by the process by which it reaches a given decision.  For example, a decision process may rely on attributes that seem normatively or legally dubious--- such as a recidivism prediction model which determines a defendant's ability to walk free between their arrest and their court date based on the criminal history of their parents and friends~\cite{angwin2016machine}. %An ad-targeting model might 
% %over-rely on spurious correlations to make its decisions—such as those between shopping habits and potential job qualifications~\cite{feat}. 
% Or, as we will explore in depth in this thesis, a decision process may be unfair because it is highly
% arbitrary or unstable—--such as a bank effectively flipping a coin to determine who gets a loan~\cite{blackleave2021}. Even if such models performed admirably on outcomes-based fairness measures, they may still be seen as unfair by many. Further, while the transportability between contexts which comes from abstraction is useful, as we explore in Chapter~\ref{chap:IRS}, this generality can come at a cost to specificity, thus at times harming the applicability of common fairness metrics in real-world contexts. %Contrastingly, using pipeline-based fairness \emph{interventions} can be more flexible to contextual model behavior requirements, as we 
% %More broadly, the focus on generalizability and abstraction in many fairness metrics may create pressure to only consider model behaviors which are \emph{always} undesirable as unfairness. However, the meaning of fair behavior varies greatly from context to context, and thus some behaviors which are unfair in one circumstance are perfectly acceptable in others (pick up on this?)

% %By explicitly considering the machine learning pipeline as we consider what behaviors may constitute unfair treatment in various contexts, we can recognize a larger variety of behaviors which may be unfair in certain contexts. 

% \paragraph{Pipeline-based Fairness Interventions.} This abstraction does not only exist in fairness definitions, but also in common unfairness mitigation techniques. %Perhaps influenced by the input-output view of the fairness problem, 
% Common fairness mitigation techniques 
% %often cast fairness desiderata as extra objectives in model optimization. That is, many common techniques to promote fairness 
% are often constructed as \emph{constraints} put on top of a model's decision or optimization process~\cite{agarwal2018reductions,hardtequality2016,zafar2017fairness-aistats}. This approach has many merits: abstracting the problem of fairness to an optimization constraint over a problem with inputs and outputs is the only way to make a fully generalizable solution to a given fairness problem. However, mitigating unfair behavior in this way obfuscates the choices made along the AI pipeline and their effect on the fairness behavior of the model---and thus the potential fairness benefits of changing some of these choices. As we demonstrate in this thesis, decisions made along the AI pipeline have a huge impact on model behavior, from influencing a model's individual predictions, to changing the distribution of the individuals it selects~\cite{feat,blackleave2021,blackIRS2022}. %cite IRS, feature-wise, LUF, future work,
% While these generalized methods of alleviating fairness problems are extremely useful, attacking fairness problems \emph{only} with these tools may leave some stones unturned.

% We can, in addition to using commonly available bias mitigation techniques, also explicitly investigate the choices made along the AI pipeline---even seemingly fairness-unrelated ones---as intervention points to improve model fairness behavior. Given that the decisions made along the AI pipeline determine a model and its behavior, if a model is acting unfairly, one way to change that behavior may be to change some choices made along its creation pipeline, rather than adding an additional constraint on top of the model.  For example, as we demonstrate in Chapter~\ref{chap:ensemble}, changing model type to an ensemble model over a singleton model can be preferable for fairness-related stability concerns. Or, as we show in Chapter~\ref{chap:IRS}, we can modify a model's prediction target to acheive fairness gains: in that case, changing from a classification to a regression model. 
% Given that, as we show in Chapter~\ref{chap:mod_mult}, there are often myriad equally viable (accurate) models for a given prediction task made with different pipelines, changing decisions made along the AI pipeline, as opposed to adding an additional constraint on top of a model's optimization or decision process, can also lead to fairness gains which come at a lower cost to performance. We demonstrate this phenomenon empirically in Chapter~\ref{chap:IRS}. Finally, as pipeline-based fairness interventions are not tied to any one definition of fairness, they can be more flexible to contextual model behavior requirements in real-world systems, as we explore in Chapter~\ref{chap:IRS} as well.


% As a whole, this thesis aims to show the immense flexibility that the AI creation pipeline gives practitioners with respect to how to reach the goals they set out to acheive with machine learning models---but also, how the choices made along the AI pipeline have to be carefully considered in terms of their impact on desired model behaviors, as even seemingly small choices can have a large impact.
% By considering all the choices made along the AI pipeline---from feature selection, to model type, to the objective functions---as places where changes can be made to improve fairness behavior, we can greatly expand our arsenal of unfairness-fighting tools.


% The rest of this work proceeds as follows:

==> versions/intro_4.tex <==
\section{Introduction} 

%Algorithmic fairness is no longer a nascent field. Through years of work from activists, journalists, researchers, and AI practitioners, professionals across industry, government, and the nonprofit sectors rely on algorithmic fairness expertise to guide their implementation of AI systems. However, while algorithmic fairness scholarship is broad, in practice, it often gets simplified into enforcing
%a mathematically abstracted definition of fairness on top of a pre-made system, either by enforcing fairness constraints within the optimization function, post-processing model outputs, or occasionally by manipulating data. Indeed, as this paper points out, the plurality of fairness research falls into either creating abstracted definitions to enforce, or finding ways to enforce a fairness constraint on top of an already constructed system. 

Faithful to its roots within computer science literature, many well-known conceptions of algorithmic fairness are highly abstracted from the details of any one system implementation. Most formalizations of fairness in the AI literature abstract the problem of unfair model behavior to generic model inputs, model outputs, and the ground truth label. The most common fairness definitions, such as demographic parity, equalized false and/or true positive rates, and equal accuracy, can be expressed only with ``observed features V [i.e., input features], outcomes Y [i.e., ground truth labels] ... and decisions D [i.e., model outputs]''~\citep{mitchell2021algorithmic}. Even slightly less common notions, such as counterfactual fairness or individual fairness, are expressed as a constraint on model inputs and outputs in relation to additional information about the data distribution, such as a given similarity metric or causal graph~\cite{mitchell2021algorithmic}. 

This level of abstraction has many merits: abstraction to the basic elements of a system leads to transportability across implementations, and so these definitions, and the methods used to enforce them, can be applied to fairness problems in a variety of application contexts. Further, the abstraction of these metrics adds to their simplicity, so they can be easily intuited and computed. Beyond these merits, in many contexts, such fairness definitions are also fundamentally important: for example, extreme demographic disparity is of legal consequence in areas such as hiring~\cite{griggs1971}. 

However, as countless others have pointed out[CITE], %this abstracted approach has pitfalls, 
the approach of enforcing an abstracted definition on top of a pre-built machine learning system has pitfalls---
often based on the fact it does not pay attention to the details of the system over which it is enforced. Indeed, details about the AI system and its context---such as the data or model type used, or how the predictions are used in practice-- can even render enforcing these definitions harmful from an equity standpoint [cite]. %Additionally, the most commonly used approaches for enforcing fairness constraints in practice, have been shown to be ill-suited for problems on the ground~\cite{}, or brittle~\cite{haverfordladysorell}.

More broadly, this abstracted approach inherently ignores situations where sources of bias are embedded in choices made in the model-building process, i.e., the choices made along the \emph{AI pipeline}. 
All of these choices at all of the steps of the AI pipeline have impacts on the model’s behavior. Thus, we can leverage the pipeline to change and understand AI model behavior: if we believe a model is acting unfairly, certainly, one way to change that behavior is to change some choices we made along the way to making that model.
In these situations, fairness problems may be mitigated by \emph{changing} certain modeling choices, i.e. via a targeted intervention, rather than by adding a constraint on top of a model. In some cases, taking such an approach can also reduce the oft-discussed fairness-performance tradeoff.

%Symmetrically, the choices we make along the machine learning pipeline may lead to fairness problems themselves--potentially inexpressible through definitions abstracted to input and output.

In this paper, we draw attention to an alternate approach to tackling algorithmic fairness problems, which we call \textit{pipeline fairness}. In pipeline-based fairness, practitioners interrogate choices made at each step of the AI creation pipeline to search for ways in which these choices impact model fairness behavior, and then, when possible, change the relevant modeling choices to abate this effect. 
%This technique is inherently contextualized to a model's specific application and implementation; it promotes building systems with equity in 
%This technique takes into account many principles that the algorithmic fairness community has suggested for building systems as equitably as possible, such as, building with equity in mind from the beginning, and creating contextualized fairness interventions. (should go elsewhere)
Importantly, we suggest the pipeline-based approach to algorithmic fairness not as a replacement or improvement upon the literature to date, but rather as an additional, largely unexplored, toolbox, which holds promise for expanding our ability to tackle fairness problems on the ground. Additionally, we do not claim to introduce the idea of pipeline fairness: instead, we suggest that pipeline fairness is simply a name for a (dispersed) pattern of algorithmic fairness work that is ongoing, but has yet to be collected into one thread--however, we argue that it is beneficial to do so. 

Thus, a pipeline approach to fairness relies on a mapping of the relationships between choices made at each step of the \emph{AI pipeline} to its effects on a model's fairness behavior, for a given fairness goal. This mapping is not something that exists in any level of detail at the moment, nor is housed in any specific place---examples of how modeling choices influence fairness behavior are few and far between in the literature in relation to abstraction-based techniques, as this paper demonstrates. 
The goals of this paper are  threefold: first, to define, and draw attention to, a pipeline-based approach to algorithmic fairness; second, to collect and synthesize the fairness literature that embodies this approach, in an attempt to map out which areas of the pipeline are better understood, and which are less; and finally, to create a research agenda for filling out our map of how modeling choices can lead to fairness pitfalls, in service of creating a robust roadmap for practitioners of how we can build systems as free from bias as possible.%, drawing from examples

%\textbf{The goal of this paper is to show 
%what parts of this mapping have received attention, which are relatively untouched, and outline a research agenda to collaboratively can leverage the information and techniques we have to develop a full understanding of pipeline fairness.}

As a whole, this work aims to remind researchers of the immense flexibility that the AI creation pipeline gives practitioners with respect to how to reach the goals they set out to achieve with machine learning models---but also, how the choices made along the AI pipeline have to be carefully considered in terms of their impact on desired model behaviors, as even seemingly small choices can have a large impact.
We hope that together as a research community, we can learn to leverage all the choices made along the AI pipeline---from data collection and feature engineering, to hypothesis class selection, to the objective functions---as places where decision can be made to improve fairness behavior, we thus greatly expand our arsenal of unfairness-fighting tools.

The rest of this paper proceeds as follows: in Section~\ref{sec:pipfair}, we define the AI pipeline and pipeline fairness in detail. In Section~\ref{sec:litreview}, we categorize the fairness literature (fairness papers from top 4 ML conferences from the past five years) from the perspective of pipeline fairness, and point out areas where there has been less and more attention, and finally, in Section~\ref{sec:agenda}, we construct our research agenda for a fuller understanding of pipeline fairness moving forward.

\subsection{Pipeline Fairness}

\paragraph{The AI Pipeline.} 
%The abstraction-based view of fairness can draw attention away from the fact that each step made along the \emph{AI model creation pipeline} can influence the fairness of a model's behavior.
To understand pipeline fairness, we need to understand the AI pipeline, or the process of creating an AI model for a given application. 
%The process of creating AI models for a given application 
This process is complex:
myriad choices are made during model creation, from the profound to the seemingly inconsequential. For example, in order to construct a loan decision model for a bank, a decision has to be made about how to translate the bank's objective, i.e., deciding who to grant loans to,  into a prediction target: e.g., predicting the probability of the client's default, or the amount of money gained by the bank per client, or something else entirely, also known as \emph{problem formulation}. The data to train the model has to be chosen, including choices about how to sample, label, and link data; how to construct features from available information for use in the model, and which of the constructed features to for prediction.  On a lower level, model practitioners must decide what type of model will be used, the learning rule and objective function, regularizers, the values of hyper-parameters determining normalization and training procedures, how the dataset will be split into train-test- and validation folds, among many other decisions made continuously throughout model development~\cite{lehr2017playing, kim2022race}. Practitioners will also have to decide what performance metrics will be used to evaluate models, and finally, how the model will be used in practice (e.g., with or without human involvement, how model predictions will be communicated and integrated into a larger decision system). (We define the steps of the AI pipeline in more detail in Section~\ref{pipeline}). 
All of these decisions then impact how it makes its own decisions, and thus its prediction behavior. 

\paragraph{Pipeline Fairness}
A pipeline-based view of fairness, then, considers each step of the AI pipeline as an intervention point to achieve a given fairness goal---and considers the effects of each choice during model creation on system behavior.
Importantly, those modeling choices are often practically changeable. While modeling choices are often made in search of the most accurate possible model, recent work has shown that there are usually many potential models--made with different modeling choices---with equivalent performance that can be created for any given prediction problem, while displaying considerably different fairness behavior~\cite{black2022model,blackleave2021,marx2019,rodolfa2021empirical}.

\paragraph{Benefits of Pipeline Fairness}
The pipeline approach to fairness is a method of augmenting our understanding of how to address fairness problems, not replacing the current most popular methods. 
Firstly, the pipeline approach to fairness can often unearth root causes of bias in a system, and thus point directly to mitigation techniques: e.g., if a faulty prediction target is chosen for a problem, choosing a different one can decrease discrimination~\cite{obermeyer2019dissecting,black}. Additionally, since the anti-bias intervention directly targets a source of bias, instead of putting an additional constraint on top of the system, this can lead to mitigation techniques that have lower performance-accuracy tradeoffs than abstraction-based methods~\cite{irs}. 
Further, while pipeline-based fairness mitigation is separate from creating definitions of fairness, many have pointed out that not all fairness problems are encapsulated by these abstracted, largely input/output based ideas of fairness. 
By reducing the problem of unfairness to a question of inputs and outputs, we may narrow our perception of what unfair behavior means to only include those factors. By using a pipeline-based approach, may naturally uncover unfairness which may arise not only from a system's outcomes, but also by the process by which it reaches a given decision. For example, a decision process may rely on attributes that seem normatively or legally dubious--- such as a recidivism prediction model which determines a defendant's ability to walk free between their arrest and their court date based on the criminal history of their parents and friends~\cite{angwin2016machine}; or a decision process may be unfair because it is highly
arbitrary or unstable—--such as a bank effectively flipping a coin to determine who gets a loan~\cite{blackleave2021}.
Further, while the transportability between contexts which comes from abstraction is useful, this generality can come at a cost to specificity, thus at times harming the applicability of common fairness metrics in real-world contexts---paying attention to the details of the system as pipeline fairness requires can also serve as a method of unearthing more contexutalized notions of fairness.

We note that ``pipeline fairness'' is simply a name for a mode of investigation that has already been underway in the algorithmic fairness literature since its inception---however, to the author's knowledge, there is no explicit paper tying the dispersed works that leverage the AI pipeline for fairness interventions together, connecting and collecting them under one roof. The goal of this paper is to do so, drawing attention to the phenomenon of pipeline fairness, as we believe that this technique is a promising future direction for expanding the algorithmic fairness toolbox, and deserves the focus and attention of the academic community. 

The main contributions of this paper are :
\begin{itemize}
    \item Defining pipeline fairness
    \item Synthesizing the work on pipeline fairness to date in the literature in a community-updatable document 
    \item Creating a research agenda in order to flesh out our understanding of how modeling choices along the pipeline impact fairness behavior of AI systems, so that we may guide practitioners through creating more equitable systems in the future.
\end{itemize}





%More broadly, considering more aspects of the modeling process as an intervention point simp

%More broadly, this abstracted approach inherently ignores situations where a root cause of bias is embedded in lower-level modeling choices of the system: and thus, may be mitigated by changing that modeling choice. 

%Importantly, those modeling choices are often practically changeable. While modeling choices are often made in search of the most accurate possible model, recent work has shown that there are usually many potential models--made with different modeling choices---with equivalent performance that can be created for any given prediction problem, while displaying considerably different fairness behavior~\cite{black2022model,blackleave2021,marx2019,rodolfa2021empirical}. 

%In this paper, we draw attention to an alternate approach to tackling algorithmic fairness problems, which we call \textit{pipeline fairness}. A pipeline approach to fairness relies on mapping the relationships between choices made at each step of the \emph{AI pipeline} to its effects on a model's fairness behavior, for a given fairness goal. 


% By approaching bias mitigation through changing a modeling choice rather than adding an additional 

% Thus, completely abstracting fairness problems---and in so doing, ignoring modeling choices when tackling fairness issues--- can lead to ignoring situations where direct interventions on the root cause of bias can be performed, rather than placing a constraint on top of a system. Taking the approach of ignoring the underlying system and adding constraints on top of a model can (sometimes unnecessarily) introduce ``fairness’’-performance tradeoffs. 
% Sometimes (but rarely), the (only) way to mitigate bias in a system is to add constraints on top of a model to force it to adhere to a given notion of fairness. 
% However, often, there are decisions made during the system building process that exacerbate unfair behavior. 






% %Algorithmic Fairness is no longer a nascent field. 
% While interest in, and scholarship of, algorithmic fairness is broad, it often gets simplified, and packaged in practice, into simply enforcing
% mathematically abstracted fairness definitions onto
% %statistical group-based fairness notions on a 
% pre-made ML system, often through adding relevant constraints. 

% Notably, most formalizations of fairness in the AI literature abstract the problem of unfair model behavior to model inputs, model outputs, and the ground truth label. The most common fairness definitions, such as demographic parity, equalized false and/or true positive rates, and equal accuracy, can be expressed only with ``observed features V [i.e., input features], outcomes Y [i.e., ground truth labels] ... and decisions D [i.e., model outputs]''~\citep{mitchell2021algorithmic}. Even slightly less common notions, such as counterfactual fairness or individual fairness, are expressed as a constraint on model inputs and outputs in relation to additional information about the data distribution, such as a given similarity metric or causal graph~\cite{mitchell2021algorithmic}. 

% This abstraction has many merits: abstraction to basic elements of a system leads to transportability, and so these definitions can be applied to a large variety of fairness problems. Further, these metrics can be easily computed and tested no matter the model implementation. Beyond these merits, in many contexts, such fairness definitions are also fundamentally important: for example, extreme demographic disparity is of legal consequence in areas such as hiring~\cite{griggs1971}. 


% While this abstracted approach is useful in certain contexts, many works over the years have pointed to its pitfalls [CITE HERE]: some have argued that enforcing abstract definitions on top of a pre-made system  can exclude countless notions of what unfairness means, particularly ones that are especially relevant to the given application context [CITE], others have shown how details about the ML system---the data or model type used, or how the predictions are used in practice--render enforcing these definitions useless at best and harmful at worst. 

% Indeed, 

% Through years of work from activists, journalists, researchers, and AI practitioners, professionals across industry, government, and the nonprofit sectors engage with, and rely on, algorithmic fairness expertise to guide their implementation of AI systems.



% While this approach is useful in certain contexts, many works over the years have pointed to the pitfalls of this approach [CITE HERE]: some have argued this one-size-fits all approach can exclude countless notions of what unfairness means, particularly ones that are especially relevant to the given application context [CITE], others have shown how details about the ML system---the data or model type used, or how the predictions are used in practice--render enforcing these definitions useless at best and harmful at worst. 

% In this paper, we draw attention to an alternate approach to tackling algorithmic fairness problems, which we call \textit{pipeline fairness}. We argue that pipeline fairness is simply a name for a (dispersed) pattern of algorithmic fairness work that is ongoing, and holds promise for directing the field towards creating another set of useful tools for fighting fairness problems on the ground. In this work, we define the pipeline-based approach to fairness; collect and organize the work to date which uses this approach; and create a research agenda outlining the next steps required to create an pipeline-fairness based arsenal of techniques to address unfairness in practice. 
% %but has not been collected under one umbrella---however, we argue it should be, due to its promise for directing the field towards creating another set of useful tools for fighting fairness problems on the ground. 



 

% In this work, we call this series of decisions model practitioners have to make the \emph{AI creation pipeline}, or the pipeline. 
% %As the pipeline determines how models reach their decision-making schema, we will also refer to the \emph{AI decision pipeline}, or the process by which a model makes a decision about a given input, as the pipeline, differentiating between the creation and decision pipelines when necessary.\footnote{We will also interchangeably refer to the AI pipeline as the machine learning pipeline, training pipeline, or learning pipeline.} 
% While choices are often made along the creation pipeline in search of the most accurate possible model, as this paper and other recent work shows, many of the potential models that could be created among these choices are equally viable (i.e. have equivalent performance) in the given context, while displaying considerably different fairness behavior~\cite{black2022model,blackleave2021,marx2019,rodolfa2021empirical}. 

% This work aims to present the benefits of explicitly considering the creation pipeline in our conceptualization of, and mitigation of, fairness problems in AI systems, which we call a \emph{pipeline-based approach} to algorithmic fairness. We suggest that, while useful in many ways, the abstraction of fairness problems in the AI literature can narrow the field's perspective both on what can constitute unfair behavior, as well as on how unfair behavior can be mitigated in AI systems. By \emph{also} considering a pipeline-based approach in our fairness conceptualization and mitigation, we can uncover and prevent a wider variety of undesirable model behavior, as well as learn to use a larger array of techniques to prevent and stop unfair model behavior in practice. We suggest the pipeline-based approach to algorithmic fairness not as a replacement or improvement upon the literature to date, but rather as an additional, largely unexplored, toolbox. 

% \paragraph{Expanding Notions of Fairness: Procedural versus Outcomes-Based Fairness.} 
% By reducing the problem of unfairness to a question of inputs and outputs, we may narrow our perception of what unfair behavior means to only include those factors. By using a pipeline-based approach, we can uncover unfairness which may arise not only from a system's outcomes, but also by the process by which it reaches a given decision.  For example, a decision process may rely on attributes that seem normatively or legally dubious--- such as a recidivism prediction model which determines a defendant's ability to walk free between their arrest and their court date based on the criminal history of their parents and friends~\cite{angwin2016machine}. %An ad-targeting model might 
% %over-rely on spurious correlations to make its decisions—such as those between shopping habits and potential job qualifications~\cite{feat}. 
% Or, as we will explore in depth in this thesis, a decision process may be unfair because it is highly
% arbitrary or unstable—--such as a bank effectively flipping a coin to determine who gets a loan~\cite{blackleave2021}. Even if such models performed admirably on outcomes-based fairness measures, they may still be seen as unfair by many. Further, while the transportability between contexts which comes from abstraction is useful, as we explore in Chapter~\ref{chap:IRS}, this generality can come at a cost to specificity, thus at times harming the applicability of common fairness metrics in real-world contexts. %Contrastingly, using pipeline-based fairness \emph{interventions} can be more flexible to contextual model behavior requirements, as we 
% %More broadly, the focus on generalizability and abstraction in many fairness metrics may create pressure to only consider model behaviors which are \emph{always} undesirable as unfairness. However, the meaning of fair behavior varies greatly from context to context, and thus some behaviors which are unfair in one circumstance are perfectly acceptable in others (pick up on this?)

% %By explicitly considering the machine learning pipeline as we consider what behaviors may constitute unfair treatment in various contexts, we can recognize a larger variety of behaviors which may be unfair in certain contexts. 

% \paragraph{Pipeline-based Fairness Interventions.} This abstraction does not only exist in fairness definitions, but also in common unfairness mitigation techniques. %Perhaps influenced by the input-output view of the fairness problem, 
% Common fairness mitigation techniques 
% %often cast fairness desiderata as extra objectives in model optimization. That is, many common techniques to promote fairness 
% are often constructed as \emph{constraints} put on top of a model's decision or optimization process~\cite{agarwal2018reductions,hardtequality2016,zafar2017fairness-aistats}. This approach has many merits: abstracting the problem of fairness to an optimization constraint over a problem with inputs and outputs is the only way to make a fully generalizable solution to a given fairness problem. However, mitigating unfair behavior in this way obfuscates the choices made along the AI pipeline and their effect on the fairness behavior of the model---and thus the potential fairness benefits of changing some of these choices. As we demonstrate in this thesis, decisions made along the AI pipeline have a huge impact on model behavior, from influencing a model's individual predictions, to changing the distribution of the individuals it selects~\cite{feat,blackleave2021,blackIRS2022}. %cite IRS, feature-wise, LUF, future work,
% While these generalized methods of alleviating fairness problems are extremely useful, attacking fairness problems \emph{only} with these tools may leave some stones unturned.

% We can, in addition to using commonly available bias mitigation techniques, also explicitly investigate the choices made along the AI pipeline---even seemingly fairness-unrelated ones---as intervention points to improve model fairness behavior. Given that the decisions made along the AI pipeline determine a model and its behavior, if a model is acting unfairly, one way to change that behavior may be to change some choices made along its creation pipeline, rather than adding an additional constraint on top of the model.  For example, as we demonstrate in Chapter~\ref{chap:ensemble}, changing model type to an ensemble model over a singleton model can be preferable for fairness-related stability concerns. Or, as we show in Chapter~\ref{chap:IRS}, we can modify a model's prediction target to acheive fairness gains: in that case, changing from a classification to a regression model. 
% Given that, as we show in Chapter~\ref{chap:mod_mult}, there are often myriad equally viable (accurate) models for a given prediction task made with different pipelines, changing decisions made along the AI pipeline, as opposed to adding an additional constraint on top of a model's optimization or decision process, can also lead to fairness gains which come at a lower cost to performance. We demonstrate this phenomenon empirically in Chapter~\ref{chap:IRS}. Finally, as pipeline-based fairness interventions are not tied to any one definition of fairness, they can be more flexible to contextual model behavior requirements in real-world systems, as we explore in Chapter~\ref{chap:IRS} as well.


% As a whole, this thesis aims to show the immense flexibility that the AI creation pipeline gives practitioners with respect to how to reach the goals they set out to acheive with machine learning models---but also, how the choices made along the AI pipeline have to be carefully considered in terms of their impact on desired model behaviors, as even seemingly small choices can have a large impact.
% By considering all the choices made along the AI pipeline---from feature selection, to model type, to the objective functions---as places where changes can be made to improve fairness behavior, we can greatly expand our arsenal of unfairness-fighting tools.


% The rest of this work proceeds as follows:

==> versions/intro_5.tex <==
\section{Introduction} 

%Algorithmic fairness is no longer a nascent field. Through years of work from activists, journalists, researchers, and AI practitioners, professionals across industry, government, and the nonprofit sectors rely on algorithmic fairness expertise to guide their implementation of AI systems. However, while algorithmic fairness scholarship is broad, in practice, it often gets simplified into enforcing
%a mathematically abstracted definition of fairness on top of a pre-made system, either by enforcing fairness constraints within the optimization function, post-processing model outputs, or occasionally by manipulating data. Indeed, as this paper points out, the plurality of fairness research falls into either creating abstracted definitions to enforce, or finding ways to enforce a fairness constraint on top of an already constructed system. 

Faithful to its roots within computer science literature, many well-known conceptions of algorithmic fairness are highly abstracted from the details of any one system implementation. Most formalizations of fairness in the AI literature abstract the problem of unfair model behavior to generic model inputs, model outputs, and the ground truth label. The most common fairness definitions, such as demographic parity, equalized false and/or true positive rates, and equal accuracy, can be expressed only with ``observed features V [i.e., input features], outcomes Y [i.e., ground truth labels] ... and decisions D [i.e., model outputs]''~\citep{mitchell2021algorithmic}. Even slightly less common notions, such as counterfactual fairness or individual fairness, are expressed as a constraint on model inputs and outputs in relation to additional information about the data distribution, such as a given similarity metric or causal graph~\cite{mitchell2021algorithmic}. 

This level of abstraction has many merits: abstraction to the basic elements of a system leads to transportability across implementations, and so these definitions, and the methods used to enforce them, can be applied to fairness problems in a variety of application contexts. Further, the abstraction of these metrics adds to their simplicity, so they can be easily intuited and computed. Beyond these merits, in many contexts, such fairness definitions are also fundamentally important: for example, extreme demographic disparity is of legal consequence in areas such as hiring~\cite{griggs1971}. 

However, as countless others have pointed out[CITE], %this abstracted approach has pitfalls, 
the approach of enforcing an abstracted definition on top of a pre-built machine learning system has pitfalls---
often based on the fact it does not pay attention to the details of the system over which it is enforced. Indeed, details about the AI system and its context---such as the data or model type used, or how the predictions are used in practice-- can even render enforcing these definitions harmful from an equity standpoint [cite]. %Additionally, the most commonly used approaches for enforcing fairness constraints in practice, have been shown to be ill-suited for problems on the ground~\cite{}, or brittle~\cite{haverfordladysorell}.

More broadly, this abstracted approach inherently ignores situations where sources of bias are embedded in choices made in the model-building process, i.e., the choices made along the \emph{AI pipeline}. 
All of these choices at all of the steps of the AI pipeline have impacts on the model’s behavior. Thus, we can leverage the pipeline to change and understand AI model behavior: if we believe a model is acting unfairly, certainly, one way to change that behavior is to change some choices we made along the way to making that model.
In these situations, fairness problems may be mitigated by \emph{changing} certain modeling choices, i.e. via a targeted intervention, rather than by adding a constraint on top of a model. In some cases, taking such an approach can also reduce the oft-discussed fairness-performance tradeoff.

%Symmetrically, the choices we make along the machine learning pipeline may lead to fairness problems themselves--potentially inexpressible through definitions abstracted to input and output.

In this paper, we draw attention to an alternate approach to tackling algorithmic fairness problems, which we call \textit{pipeline fairness}. In pipeline-based fairness, practitioners interrogate choices made at each step of the AI creation pipeline to search for ways in which these choices impact model fairness behavior, and then, when possible, change the relevant modeling choices to abate this effect. 
%This technique is inherently contextualized to a model's specific application and implementation; it promotes building systems with equity in 
%This technique takes into account many principles that the algorithmic fairness community has suggested for building systems as equitably as possible, such as, building with equity in mind from the beginning, and creating contextualized fairness interventions. (should go elsewhere)
Importantly, we suggest the pipeline-based approach to algorithmic fairness not as a replacement or improvement upon the literature to date, but rather as an additional, largely unexplored, toolbox, which holds promise for expanding our ability to tackle fairness problems on the ground. Additionally, we do not claim to introduce the idea of pipeline fairness: instead, we suggest that pipeline fairness is simply a name for a (dispersed) pattern of algorithmic fairness work that is ongoing, but has yet to be collected into one thread--however, we argue that it is beneficial to do so. 

Thus, a pipeline approach to fairness relies on a mapping of the relationships between choices made at each step of the \emph{AI pipeline} to its effects on a model's fairness behavior, for a given fairness goal. This mapping is not something that exists in any level of detail at the moment, nor is housed in any specific place---examples of how modeling choices influence fairness behavior are few and far between in the literature in relation to abstraction-based techniques, as this paper demonstrates. 
The goals of this paper are  threefold: first, to define, and draw attention to, a pipeline-based approach to algorithmic fairness; second, to collect and synthesize the fairness literature that embodies this approach, in an attempt to map out which areas of the pipeline are better understood, and which are less; and finally, to create a research agenda for filling out our map of how modeling choices can lead to fairness pitfalls, in service of creating a robust roadmap for practitioners of how we can build systems as free from bias as possible.%, drawing from examples

%\textbf{The goal of this paper is to show 
%what parts of this mapping have received attention, which are relatively untouched, and outline a research agenda to collaboratively can leverage the information and techniques we have to develop a full understanding of pipeline fairness.}

As a whole, this work aims to remind researchers of the immense flexibility that the AI creation pipeline gives practitioners with respect to how to reach the goals they set out to achieve with machine learning models---but also, how the choices made along the AI pipeline have to be carefully considered in terms of their impact on desired model behaviors, as even seemingly small choices can have a large impact.
We hope that together as a research community, we can learn to leverage all the choices made along the AI pipeline---from data collection and feature engineering, to hypothesis class selection, to the objective functions---as places where decision can be made to improve fairness behavior, we thus greatly expand our arsenal of unfairness-fighting tools.

The rest of this paper proceeds as follows: in Section~\ref{sec:pipfair}, we define the AI pipeline and pipeline fairness in detail. In Section~\ref{sec:litreview}, we categorize the fairness literature (fairness papers from top 4 ML conferences from the past five years) from the perspective of pipeline fairness, and point out areas where there has been less and more attention, and finally, in Section~\ref{sec:agenda}, we construct our research agenda for a fuller understanding of pipeline fairness moving forward.

==> versions/intro_old.tex <==
\section{Introduction} 

There has been a recent increase in research focused on designing ML and ML systems that don't result in harm to the affected individuals and communities. This work has spanned various types of  harms that can result with the use of such systems (such as bias and inequity, lack of agency, lack of trust, etc.). While there has been extensive work in this area, practitioners, when faced with designing a fair ML system, often make ad-hoc design choices such as remove certain sensitive attributes, change the distribution of the data,create synthetic data, enforce fairness constraints within the optimization function, or post-process model outputs. While those techniques can sometimes result in improving the system, more often than not, they have marginal practical impact. 

\rgdelete{Many have begun to point to the weaknesses of this approach. Firstly, studies interviewing practitioners on the ground report feelings of anxiety about not choosing the correct metric for a given fairness issue~\cite{madaio2020co}. Once a metric is chosen, there are many technical drawbacks: Friedler et al.~\cite{friedler2019comparative} find that several common algorithms for mitigating bias are sensitive to small changes in training set-up such as train-test splits and preprocessing steps. Others find that the implementation structure of these techniques does not translate well to a variety of policy problems, which have complications such as only being able to select predictions up to a budget~\cite{black2022algorithmic, singh2022fair}.  Some have even shown that naively enforcing fairness metrics, such as demographic parity, on data with certain types of label noise can decrease those very same metrics in the true population~\cite{wang2021fair}.}

Based on our experience, we believe that many of these problems stem from the fact that the typical approach to dealing with fairness in ML is 
 myopic---it hyper-focuses on mitigating bias through making changes in one of just a few places along the ML system design pipeline, namely, choice of optimization function, loss function, model selection or particular aspects of data preprocessing.  However, \emph{all} of the choices made at each step  
along the ML pipeline have impacts on people being affected by the ML system: problem formulation~\cite{passi2019problem}; data: choice of data sources, data sampling, data labeling, data cleaning; feature creation and feature selection; hypothesis class, optimization function, regularizer and hyperparameter choice; model selection methodology: creation of train-validation splits, the selection of evaluation metrics and pre-deployment validation; as well as human-machine interaction, handoff, and other organizational intricacies. 

As prior works have noted~\cite{akpinar2022sandbox,suresh2021framework}, by abstracting away the rest of the ML pipeline and \rgdelete{enforcing a given metric on top of a system during training or prediction} selecting an ad-hoc mitigation strategy, the more mainstream approach ignores situations where we can actually identify, isolate, and mitigate the impact of some of the \emph{sources} of bias----as they are a result of other choices made in the system-building process. 
Disregarding underlying sources of bias in the modeling setup and instead enforcing fairness metrics at training or prediction time can  
needlessly increasing a fairness-accuracy tradeoff due to intervening at the wrong place~\cite{black2022algorithmic}, or, at worst, 
 ``[hide] the real problem while creating an illusion of
fairness''~\cite{akpinar2022sandbox}. 

Thus, we join others in advocating for an alternate approach~\cite{akpinar2022sandbox,suresh2021framework}, which we call a pipeline-based approach to fairness. In a pipeline-based fairness approach, practitioners enumerate choices that can be made at each step of the ML creation pipeline and search for ways in which these choices affect people impacted by the model, and then, when possible, change the relevant pipeline choices to abate this effect. This process \hhedit{should} take place iteratively after performing an intervention: the model \hhedit{should} be tested again, until it is deemed satisfactory for deployment given its specific behavioral desiderata, whereupon testing and model updates \hhedit{would} continue through deployment. %\marginpar{\hhcomment{I think we should distinguish between what \emph{should ideally} happen, and what \emph{does or will} happen. \ebcomment{do you mean beyond using the word should here(in red above)? If there is something specific you have in mind, feel free to draft:)}}} 
%And, importantly, it should reflect the lifecycle of the system: i.e. testing and updating continues during deployment.

However, as rosy as a pipeline-based approach may sound, it is unclear  how to  \emph{operationalize} a pipeline-based approach to fairness detection and mitigation: \hhedit{making informed hypotheses about} what choices made along the pipeline led to bias is a difficult task even for those with specialized \hhedit{ML} knowledge. 

In fact, as we discuss in Section~\ref{sec:teaching_evidence}, based on evidence from a graduate-level fairness class at an R2 institution  we find that populations with highly specialized technical understanding have difficulty conceptualizing what ML modeling choices may lead to bias, and how to mitigate bias through appropriately chosen mitigation strategies across the entire pipeline. This is, indeed, consistent with our experience working with ML practitioners and system developers across a wide range of public policy settings.


In this paper, we do...

Our contributions in this paper are:
\begin{enumerate}
\item highlighting the critical importance of viewing algorithmic fairness through a lens of the entire ML pipeline, and providing a structure for operationalizing this approach by enumerating the components and design choices in the pipeline that can contribute to disparities
\item providing a literature review contextualizing it within the broader pipeline fairness view.
\item  offer practitioners a resource to help address root causes of unfairness in ML systems using what's available in existing literature
\item  put out a call to the FairML research community to develop contextual approaches (methods and toolkits) that use the pipeline fairness structure and support users through each stage of the pipeline as they go through it in their system design,  development, and deployment process.
 \end{enumerate}




%Beyond the benefit of finding and directly tackling some of a model's sources of unfairness, a pipeline-based approach adheres to other calls for change within the discipline from the fairness literature. Interrogating a model's pipeline inherently forces a practitioner to enforcing fairness desiderata in a contextualized manner~\cite{madaio2020co}, and also responds to the call to build models with fairness in mind from the beginning~\cite{}. 


\rgdelete{We suspect that given that computer science students with degrees in computer science cannot understand how to search for, and mitigate, bias as a result of ML modeling choices, practitioners making models in public-facing contexts find this difficult as well. \hhedit{This is, indeed, consistent with our experience working with ML practitioners across a wide range of public policy settings.} \hhcomment{Rayid, please complete this paragraph as you see fit or remove the connecting sentence.}}

%Indeed, there are challenges in creating such tools: due to its attention to the details of a given model's data and implementation, pipeline-based fairness techniques are hard to generalize, and therefore hard to create and implement in a generalized manner. 

\hhcomment{The following paragraph should appear earlier--it is motivating the work. Maybe before "While algorithmic fairness is broad..."}
Despite the difficulty in operationalizing a pipeline-based approach to bias detection and mitigation, it is becoming increasingly imperative to construct tools which do so. Beyond rising pressure on technology companies and governments to create more equitable systems~\cite{}, 
recent legal developments, such as those from the Federal Trade Comission (FTC) and Consumer Finance Protection Bureau suggest an uptick in enforcement surrounding discriminatory algorithms.
%violations of the Disparate Impact Standard---allowing for more opportunities to replace biased systems with ones that produce less harm~\cite{ftcproposed,cfpb_2022}
\footnote{Specifically, a recent advanced notice of proposed rulemaking (ANPR) from the Federal Trade Comission (FTC) suggests the possibility of stricter rules around the deployment of discriminatory systems~\cite{ftcproposed}.
One of the questions of the ANPR asks: "Should [the commission] consider new trade regulation rules that bar or somehow limit the deployment of any system that produces discrimination, irrespective of the data or processes on which those outcomes are based? ". Additionally, a recent update to the Consumer Finance Protection Bureau (CFPB) examination manuals  suggests discrimination can now be seen unfair as it’s defined under the Dodd-Frank Act, again suggesting a turn towards more enforcement of reducing discrimination in algorithmic systems: ''Discrimination may meet the criteria for ``unfairness'' by causing substantial harm to consumers that they cannot reasonably avoid, where that harm is not outweighed by countervailing benefits to consumers or competition.''~\cite{cfpb_2022} This means that companies which use machine learning systems relating to credit, housing, employment and other applications covered by the disparate impact standard may be more likely to be held legally responsible if a model is shown to be discriminatory. Additionally, if a \emph{less discriminatory alternative} (LDA)---an alternate model which meets business needs but displays less discriminatory behavior against protected groups--- is found, it may be legally required to use this model.}.  
%As prior work surrounding model multiplicity has shown~\cite{black2022model}, there are often many models with equivalent accuracy for a given prediction task which differ in certain modeling choices~\cite{rodolfa2021empirical,blackleave2021, marx2019, semenova2019study}. 
This fact gives a point of leverage for technologically equipped activists and plaintiffs to challenge discriminatory algorithms used in practice, and means it is in companies' interest to thoroughly explore the space of possible algorithms to find the least discriminatory one within those with sufficient business utility. 
However, to \emph{find} less discriminatory models, we must have the correct tools.
A growing number of scholars~\cite{black2022model,akpinar2022sandbox,suresh2021framework} suggest a pipeline-based approach will be the most effective method of finding less discriminatory models in practice, by interrogating the pipeline to find the \kredit{best}\krdelete{ most effective} places to search for interventions--however, to our knowledge, no tools to completely instantiate such an approach currently exist.

In this paper, we aim to aid the operationalization of a pipeline-centric view of fairness by taking steps towards creating a mapping 
of the relationships between choices made at each step of the \emph{AI pipeline} to its effects on a model's fairness behavior, for a given fairness aim. That is, our eventual goal is to create a tool for practitioners and students to use which outlines the entire pipeline, and details \emph{how} a given choice may impact eventual model fairness behavior. 


To the authors' knowledge, this mapping is not something that exists in any level of detail at the moment, nor is housed in any specific place---examples of how modeling choices influence fairness behavior are few and far between in the literature in relation to traditional techniques, as this paper demonstrates. 
There are also few toolkits or public code bases which help practitioners actively isolate, measure, and mitigate bias that occurs due to choices made along the pipeline. The closest tool is in development by Akpinar et al.~\cite{akpinar2022sandbox}, but this tool is incomplete--it does not cover the mapping of practitoner decisions to model behavior across entire pipeline---nor does it organize or display known sources of bias in a variety of contexts from prior work, and proposed mitigation techniques. 
%\emph{inserts biases} into a system synthetically and allows users to test their fairness interventions on a system subject to those biases, instead of suggesting what may be the consequence of a given choice on the pipeline. \hhcomment{I don't think the previous sentence is a valid criticism (I am obviously biased :D); the point of bias injection is precisely to figure out the consequences. I think we should rewrite this sentence. The real problem with that work currently is that it is incomplete--it doesn't model all possible biases, and there is no evidence of usability for it.} 
Indeed, while there may be problems with the more traditional, myopic approach to bias mitigation, it is much more easily available to implement~\cite{AIF360,bird2020fairlearn,hardt2021amazon}.


In service of our goal to create a mapping from ML creation pipeline decisions to model behavior, we offer three main contributions: first, we collect and synthesize the fairness literature that embodies a pipeline-based approach, and organize the works in relation to which aspect of the pipeline they address; secondly, we identify the areas of the pipeline that have received less and more attention, and create a research agenda for filling out our map of how modeling choices can lead to fairness pitfalls; and finally, we create (a first version of) a tool for practitioners and students to easily access the work currently available for detecting, measuring, and mitigating harm along the ML pipeline. 
This paper is the first step toward a broader agenda in which we co-design guidelines and processes for students and practitioners to understand the ML pipeline and life cycle to detect and mitigate harms appropriately.

The rest of this paper proceeds as follows: in Section~\ref{sec:pipfair}, we define the ML pipeline and pipeline fairness in detail. In Section~\ref{sec:challeneges}, we outline how our collective experience teaching classes on algorithmic fairness has shed light on some of the challenges to understanding, and by extension, operationalizing, a pipeline-based approach to fairness. Next, in 
Section~\ref{sec:litreview}, we categorize the \hhedit{pipeline-aware} fairness literature (fairness papers from top five fairness and ML conferences from the past five years) from the perspective of pipeline fairness, and point out areas where there has been less and more attention, and finally, in Section~\ref{sec:agenda}, we construct our research agenda for a fuller understanding of pipeline fairness moving forward. %and describe our first instantiation of our pipeline-based bias mitigation toolkit.
Section~\ref{sec:related} outlines related work, and Section~\ref{sec:conclusion} concludes.



==> versions/intro_old_2.tex <==
\section{Introduction} 

As AI systems proliferate in socially high-stakes domains, concerns around balancing their potential for benefiting society versus harming already marginalized and underserved communities have been mounting: from gender bias in hiring systems to racial bias in healthcare distribution systems~\cite{dastin2018amazon,obermeyer2019dissecting,buolamwini2018gender,compas}. Through years of work by activists, stakeholders, journalists, lawmakers, researchers, and AI practitioners, we now witness a growing appetite for building these systems with harm prevention in mind~\cite{room2021executive,jobin2019global}. As a result, professionals across industry, government, and nonprofits have been turning to algorithmic fairness expertise to guide their implementation of AI systems~\cite{holstein2019improving}. 

While there has been extensive work in the service of preventing unintended algorithmic harms such as unfairness~\cite{}, mitigating unfairness in practice often gets reduced to enforcing a somewhat arbitrarily chosen fairness metric on top of a pre-developed or deployed system~\cite{madaio2020co}. 
Practitioners often make ad-hoc mitigation choices to improve fairness metrics, such as removing sensitive attributes, changing the data distribution, training with synthetic data, enforcing fairness constraints, or post-processing model predictions. While these techniques may, at times, improve selected fairness metrics, they often have little to no practical impact; at worst, they can even exacerbate the same disparity metrics they aim to alleviate~\cite{wang2021fair}.

Many of the above problems may stem from the fact that the traditional approach to fairness is myopic and ad-hoc---it narrowly and arbitrarily focuses on a restricted set of points along the ML lifecycle, namely, the choice of optimization function, model selection, or particular aspects of data preprocessing. However, \emph{all} choices made along the ML pipeline potentially impact the model's behavior and, subsequently, decision subjects and affected communities. Assessing viability/functionality of AI~\citep{raji2022fallacy}, problem formulation~\cite{passi2019problem}; data collection (choice of data sources, data sampling, data labeling); data preprocessing (data cleaning, feature creation, feature selection); statistical modeling (choice of hypothesis class, optimization procedure, the regularizer, and training hyperparameter); model selection methodology (design of train-validation splits, the selection of evaluation metrics, and pre-deployment validation); as well as deployment and organizational integration (human-machine interaction, model maintenance, and updates, as well as other organizational intricacies) are among consequential choices made along the ML lifecycle.
As prior works have noted~\cite{akpinar2022sandbox,suresh2021framework}, by abstracting away the rest of the ML pipeline and selecting an ad-hoc mitigation strategy, the mainstream approach misses the opportunity to identify, isolate, and mitigate the underlying \emph{sources} of unfairness---as they are a result of other choices made in the system-building process. Disregarding underlying sources of unfairness  in the modeling pipeline can lead to needlessly increasing a fairness-accuracy tradeoff due to intervening at the wrong place~\cite{black2022algorithmic},
%interventions at the wrong place~\cite{black2022algorithmic}, or, 
at worst, 
 ``[hiding] the real problem while creating an illusion of
fairness''~\cite{akpinar2022sandbox}.

%This work heeds the growing calls to take a \emph{pipeline-aware} approach to fairness~\cite{akpinar2022sandbox,suresh2021framework}. 
Thus, we join others in advocating for an alternate approach~\cite{akpinar2022sandbox,suresh2021framework}, which we call a \emph{pipeline-aware} approach to fairness. 
At a high level, this approach works as follows: given a model with undesirable fairness behavior, the ML team must search for ways in which the variety of choices made across the ML creation pipeline may have contributed to the behavior: for example, the choice of prediction target~\cite{obermeyer2019dissecting,black2022algorithmic}, or the feature encodings~\cite{wan2022fairness}. Once plausible causes are identified, the team should evaluate whether alternatives along those dimensions could abate this effect.\footnote{This description is taking an auditing perspective: when building a fair model from scratch, fairness desiderata would be described, and the practitioners would enumerate choices that can be made at each step of the ML creation pipeline and avoid choices that work against this desired behavior.} This process should take place iteratively, and the model should be re-evaluated until it is deemed satisfactory, whereupon testing and model updates would continue for deployment.
While prior work has pointed out the potential benefits of such an approach, we contend that \emph{awareness} alone won't be sufficient for \emph{operationalizing} this approach to fairness detection and mitigation in practice. In Section~\ref{sec:challeneges}, we provide several pieces of evidence demonstrating that making informed hypotheses about the root causes of unfairness is a challenging task, even for those with specialized ML knowledge. For example, as discussed in Section~\ref{sec:teaching_evidence}, based on qualitative data gathered from a graduate-level fair-ML class at an R1 institution, students with significant ML background struggle to conceptualize sources of harmful model behavior and suggest appropriately chosen bias mitigation strategies. This observation is, indeed, consistent with our experience working with ML practitioners and system developers across a wide range of public policy settings (Section~\ref{sec:practice}).

Aside from the rising public pressure on technology companies and governments to create more equitable systems~\cite{}, as we discuss in Section~\ref{sec:regulation}, recent legal developments, such as those from the Federal Trade Commission (FTC), Consumer Finance Protection Bureau (CFPB), and various state and local agencies suggest an uptick in enforcement surrounding discriminatory algorithms. These recent movements give a point of leverage for technologically equipped activists and plaintiffs to challenge discriminatory algorithms used in practice and further incentivize companies to thoroughly explore the space of possible algorithms to find the least discriminatory one within those with sufficient business utility. Against this backdrop, we believe it is increasingly imperative to operationalize a pipeline-based approach by constructing and validating practical tools and resources for bias detection and mitigation. 

To \emph{find} less discriminatory models, we must have the appropriate tools to help us measure the discrimination, identify the underlying sources of unfairness in the pipeline, and then match those underlying sources with appropriately designed mitigation interventions. Based on the first known public search for a less discriminatory alternative model (LDA) to replace a discriminatory credit allocation system at the private lending platform, Upstart~\cite{naacp_statement}, pipeline-based approaches would be instrumental in this regard, due to several advantages, including the fact that (1) they significantly expand the space of methods currently in use~\cite{colfax2021report2}; and (2) interventions earlier in the pipeline ease legal concern over the use of protected attributes during training and deployment~\cite{colfax2021report1,colfax2021report2}. %In addition, a growing number of scholars~\cite{black2022model,akpinar2022sandbox,suresh2021framework} suggest a pipeline-based approach will be the most effective method of finding less discriminatory models in practice by interrogating the pipeline to find the most effective places to search for interventions--however, to our knowledge, no tools to instantiate such an approach currently exist.

This work takes an initial step toward operationalizing the pipeline-aware approach to fairness through the following key contributions:
\begin{enumerate}
\item We provide a blueprint for operationalizing the pipeline approach by enumerating the list of consequential design choices along the ML lifecycle (Section ~\ref{sec:pipfair})
\item We provide evidence establishing the need to go beyond mere \emph{awareness} of the pipeline approach and toward concrete resources and processes for practitioners (Section~\ref{sec:teaching_evidence})
\item We collect and synthesize existing pipeline-aware fairness work and map them to the stages of the pipeline they address (Section~\ref{sec:litreview}). This mapping can offer practitioners a one-stop shop to help understand possible causes of unfairness in their domains and evaluate the efficacy of existing methods to detect, measure, and mitigate them.
\item Last but not least, this mapping lays out a research agenda outlining the gaps in the existing body of work, calling on the FairML research community to develop contextual processes and methods to support practitioners throughout the process of designing, developing, and deploying their systems (Section~\ref{sec:agenda}). 
 \end{enumerate}
This work serves as the stepping stone toward a more comprehensive, interactive set of resources and tools for ML researchers, practitioners, students---and ultimately, other groups of stakeholders---to explore, evaluate, and contribute pipeline-aware methods designed to scrutinize and address fairness issues throughout the ML lifecycle.

==> versions/old_abs.tex <==
While the field of algorithmic fairness is diverse, in practice, the main thrust of research is often simplified into enforcing an abstracted definition of fairness on top of a pre-made system, either by enforcing fairness constraints within a model's optimization function, post-processing model outputs, or occasionally by manipulating input data. 
In this paper, we draw attention to an alternate approach to tackling algorithmic fairness problems, which we call \textit{pipeline fairness}. We argue that pipeline fairness is simply a name for a (dispersed) pattern of algorithmic fairness work that is ongoing within the literature, and holds promise for directing the field towards creating another set of useful tools for fighting fairness problems on the ground. In this work, we define the pipeline-based approach to fairness; collect and organize the fairness work to date which uses this approach; and create a research agenda outlining the next steps required to create an pipeline-fairness based arsenal of techniques to address unfairness in practice. 

==> versions/operationalize_old.tex <==
\section{The Need to Operationalize the Pipeline-Aware Approach}
\label{sec:challeneges}
%\rgcomment{need to add an intro here that highlights that it's not enough to talk about the pipeline and lists the sections below}
%Moving from mapping out the ML pipeline and its potential sources of bias, as we have done above, to actually testing to see which modeling choices may exacerbate bias and how, as well as using that understanding to mitigate the bias is not an easy task.
%As we see in Sections~\ref{sec:teaching_evidence} and ~\ref{sec:practice}, graduate students with prior background in machine learning, as well as ML pracitioners, have trouble conceptualizing how modeling choices can lead to bias, and how to leverage them for bias mitigation. In Section~\ref{sec:regulation}, we highlight how recent attempts to find less discriminatory models to replace biased models used in the lending firm Upstart performed an inexhaustive search of the space of 
%While it may seem simple to look for bias along the creation pipeline in ML systems based on 
In this section, we draw on evidence from teaching algorithmic fairness and machine learning in classrooms (Section~\ref{sec:teaching_evidence}) to students and professionals, our experience working with practitioners to develop ML systems% (Section~\ref{sec:practice})
, and recent examples of enforcing anti-discrimination law% (Section~\ref{sec:regulation})
, to highlight the difficulty in, and necessity for, \emph{operationalizing} a pipeline-aware approach to bias mitigation. We observe that a \emph{conceptual} understanding of the pipeline and the variety of choices designers make within it are by no means sufficient to inform good practice. For example, students struggle to correctly hypothesize about the underlying causes of unfairness and map them to plausible remedies. 

\subsection{Qualitative Evidence from the Classroom}\label{sec:teaching_evidence}
Our team has documented the challenges of instilling the pipeline-centric view of ML harms in students using traditional teaching methods (e.g., lectures containing real-world examples). The classroom activity outlined in this section was conducted by one of us at an R1 educational institution as part of a graduate-level course focused on the ethical and societal considerations around the use of ML in socially high-stakes domains. Our IRB approved the activity, and students had the option of opting out of data collection for research purposes.\footnote{To maintain author anonymity during the review phase, we will share our IRB approval letter if our paper is recommended for publication after the review process.} 

Details of the study are provided in the Appendix and we provide a summary of the setup as well as the findings that highlight the difficulty future developers and users of ML systems face in detecting and mitigating sources of bias. The study consisted of 37 students with a non-negligible background in Machine Learning and  aware of ML harms and more motivated to address them. Students were introduced to the ML pipeline as described above. For each stage, students were presented with multiple examples of how choices at that stage can lead to harmful outcomes (e.g., unfairness issues) at the end of the pipeline. They were then asked to team up with 3-4 classmates and pick a societal domain as the focus of their group activity  given 30 minutes to discuss questions about their application domain with teammates and submit their written responses individually on the following questions;
\begin{itemize}
    \item What is the specific \textbf{predictive task} in this domain that your team will focus on? Please briefly describe how you came across this task.	
    \item What \textbf{type of harm} did your team decide to focus on? Please briefly describe whether you know of precedence for this type of harm in your domain of choice.	
    \item What are your \textbf{hypotheses around the causes} of this type of harm manifesting through the ML pipeline? Please be comprehensive to the extent possible.	
    \item What are your \textbf{hypotheses around potentially effective remedies} for addressing this harm? Please be comprehensive to the extent possible.
\end{itemize}
 
\input{classroom_table.tex}

\subsubsection{Findings}
A thematic analysis of submitted responses revealed several challenges that are documented in detail in the Appendix. The highlights were: 
\rgcomment{I'll add a sentence for each of them from the longer text}

\xhdr{Theme 1: Specifying how a real-world problem gets translated into a predictive task was not straightforward.} 

\xhdr{Theme 2: harms were characterized in broad strokes.}

\xhdr{Theme 3: Students had difficulty mapping the observed harm to a plausible underlying cause.}

\xhdr{Theme 4: Students had difficulty mapping their hypothesized causes to plausible remedies.} 

\xhdr{Theme 5: Students used broad-stroke language to describe causes and remedies of harm.} 

\rgdelete{
\rgcomment{move to appendix}
\subsection{Qualitative Evidence from the Classroom}\label{sec:teaching_evidence}
\rgcomment{I think this section is a useful study in itself but for somewhat that's more of a motivation of our work, it takes up a lot of space. I suggest summarizing the study and findings and moving the rest to the appendix}
Our team has documented the challenges of instilling the pipeline-centric view of ML harms in students using traditional teaching methods (e.g., lectures containing real-world examples). The classroom activity outlined in this section was conducted by one of us at an R1 educational institution as part of a graduate-level course focused on the ethical and societal considerations around the use of ML in socially high-stakes domains. Our IRB approved the activity, and students had the option of opting out of data collection for research purposes.\footnote{To maintain author anonymity during the review phase, we will share our IRB approval letter and if our paper is recommended for publication after the review process.} 

\subsubsection{Population and sampling}
In total, 37 students participated in the class activity. 
 Prior completion of at least one Machine Learning course was a prerequisite for enrollment. So all participants had a non-negligible background in Machine Learning. Specifically, $\sim 80\%$ characterized the familiarity with ML as intermediate, $\sim 14\%$ as advances, and $\sim 5\%$ as elementary. All students enrolled in the course took it as an elective. This fact implies that compared to a random sample of students with ML knowledge, our participants were likely more aware of ML harms and more motivated to address them. 

\subsubsection{Data collection} Students were introduced to the ML pipeline through an approximately 45-minutes long lecture. The lecture focused on the supervised learning paradigm and broke down the supervised learning pipeline into the following five stages: 
\begin{enumerate}
    \item \textbf{Task definition:} corresponding to the choice of features, $\mathbf{x}$, and predictive target, $y$.
    \item \textbf{Data collection and processing} corresponding to the choice and processing of the input data $D = \{(x_i,y_i)\}_{i=1}^n$
    \item \textbf{Model specification} corresponding to the choice of the hypothesis class, $H$.
    \item \textbf{Model fitting/training:} choosing a specific loss function, $L$, and optimizing it via existing optimization techniques to obtain a model $h \in H$
    \item \textbf{Deployment in real-world}, corresponding to the deployment of $h$ in real-world practice, and its predictions $\hat{y}$ translating into decisions that can harm/benefit certain individuals and communities
\end{enumerate}
For each stage, students were presented with multiple examples of how choices at that stage can lead to harmful outcomes (e.g., unfairness issues) at the end of the pipeline. For example, \hhcomment{TBC.}

Second, they were asked to team up with 3-4 classmates and pick a societal domain as the focus of their group activity. Examples offered to them included employment (e.g., hiring employees); 
education (e.g., admitting students); 
medicine (e.g., diagnosing skin cancer); 
housing (e.g., allocating limited housing units
child welfare (e.g., investigating referral calls); 
criminal justice (e.g., pretrial sentencing);
public safety (e.g., allocating patrol resources in policing 
e-commerce (e.g., advertising; ranking sellers on Amazon…
social media (e.g., news recommendation; content moderation);
and transportation (e.g., autonomous vehicles). One team picked finance (e.g., credit lending) as their topic.
Third, students were given 30 minutes to discuss the following questions about their application domain with teammates and submit their written responses individually:
\begin{itemize}
    \item What is the specific \textbf{predictive task} in this domain that your team will focus on? Please briefly describe how you came across this task.	
    \item What \textbf{type of harm} did your team decide to focus on? Please briefly describe whether you know of precedence for this type of harm in your domain of choice.	
    \item What are your \textbf{hypotheses around the causes} of this type of harm manifesting through the ML pipeline? Please be comprehensive to the extent possible.	
    \item What are your \textbf{hypotheses around potentially effective remedies} for addressing this harm? Please be comprehensive to the extent possible.
\end{itemize}
 
\input{classroom_table.tex}

\subsubsection{Findings}
A thematic analysis of submitted responses revealed several challenges: 

\xhdr{Theme 1: Specifying how a real-world problem gets translated into a predictive task was not straightforward.} Table~\ref{tab:classroom} overviews how each team defined their predictive tasks. For example, the finance team defined the task as \textit{assessing the \emph{creditworthiness} of individuals using their demographic and socio-economic data}. The public safety team defined the predictive task as \textit{allocating police presence to \emph{high-risk} areas}. The social media team defined the task as \textit{predicting whether a news article is fake}. Note that notions of applicant's \emph{creditworthiness} or neighborhood's safety \emph{risk}, or \emph{fakeness} of an article's content are not well-defined targets. Other teams did not adequately distinguish between the construct of interest and its operationalization as the target of prediction. For example, some members of the organ transplant team characterized the task as deciding \textit{which people \emph{should} receive an organ transplant}. In contrast, others characterized it as \textit{predicting whether an individual would receive an organ transplant in a given hospital}. Note the difference between \emph{``should''} and \emph{``would''}.


\xhdr{Theme 2: harms were characterized in broad strokes.}
Some teams described harm without specifying the groups or communities that could be impacted by it and the baseline of comparison. For example, the housing team stated \textit{price discrepancies} due to property location as the harm occurring in their domain but did not specify who could be negatively impacted by price discrepancies and in comparison with what reference group this should be considered a harm. Another example was \textit{spread of fake news} as the harm without mentioning whom it can impact negatively and how.

\xhdr{Theme 3: Students had difficulty mapping the observed harm to a plausible underlying cause.} For example, the child welfare group attempted to explain the harm against Black communities by noting that the feature, Race, was not quantified with sufficient granularity. According to their source, the tool allowed only three racial categories: White, Black, and Other. Note that there is no plausible mechanism through which this lack of granularity might have led to disparities in child welfare risk assessments against Black communities. As another example, the finance team offered \textit{biases of developers} as the potential source of 


\xhdr{Theme 4: Students had difficulty mapping their hypothesized causes to plausible remedies.} For example, the Child Welfare team proposed randomly selecting instances for inclusion in the training data. The online exam proctoring group suggested providing transparency (e.g., telling students what behavior results in a cheating flag) to reduce errors. 

\xhdr{Theme 5: Students used broad-stroke language to describe causes and remedies of harm.} For example, several teams referred to \textit{biased data} as the underlying cause of harm and offered \textbf{more comprehensive data collection} as the remedy. While correct, such high-level assessments are unlikely to lead to concrete actions in practice. Another commonly proposed remedy was \textit{human oversight} of decisions without specifying the efficiency ramifications of leaving the final call to human decision-makers.

In a session after the data collection and analysis, the instructor led a class-wide discussion in which students were encouraged to reflect on the above issues. 
}

% \subsection{Evidence from Practice}
\subsection{Lessons from Applying ML in Practice}\label{sec:practice}
\ebcomment{@Rayid @Kit please fill out :) }
In addition to educating students on developing fair ML systems, there is a need to support practitioners involved in similar work. This work has spanned a wide range of policy domains including health \cite{Ramachandran2020,potash2015predictive,somanchi2015early,Potash2020}, criminal justice \cite{ Bauman2018ReducingInterventions,Rodolfa2020CaseInterventions}, social services \cite{pan2017machine}, housing \cite{Ye2019UsingCity}, urban infrastructure \cite{Kumar2018UsingBreaks}, and education \cite{lakkaraju2015machine, mvescblog, tulsaposter} and has spanned federal agencies to city government. For instance, identifying households with small children at risk for lead poisoning to allocate limited remediation resources \cite{potash2015predictive,Potash2020}, evaluating the fairness of algorithms used to target audits of tax returns \cite{black2022algorithmic}, predicting water mains at risk of breaking \cite{Kumar2018UsingBreaks}, or intervening with social services and mental health outreach to break the cycle of incarceration \cite{ Bauman2018ReducingInterventions,Rodolfa2020CaseInterventions}. \krcomment{might need to check if we need to suppress citations here for anonymous review since we refer to our previous work?}

% - diabetes?
% - child welfare (CA?)
% - joco or la?
%
These projects are generally high-stakes in nature, with the potential for both significant impact on a given individual's life as well as the scale to affect large populations. As a matter of course, therefore, fairness is a key element of the conversation from the very earliest stages of project scoping as we understand the partner's goals and constraints. Although we haven't made a quantitative assessment of these perceptions, across this wide-ranging work in partnership with government agencies and non-profits, we have found two misconceptions about algorithmic fairness to be nearly universal. First is the perception that most or all disparities in model outputs can be attributed to underlying biases in the training data, with little appreciation for the role played by choices made by the system developers. For example, the concept of model cards\cite{} or audit tools\cite{} frequently come up in these conversations, yet they tend to over-focus on understanding the training data that was used to develop a system without much regard for the model development process itself. Understanding potential disparities in the training data is important, but as discussed above, certainly not sufficient for understanding model fairness. And, second, is the unfounded belief that simply excluding sensitive attributes from a model's feature set will produce an unbiased model. Unfortunately, we've frequently seen that cited by practitioners and vendors as an assertion of model fairness without any actual measurement of the model's outputs --- in the worst cases, regarding deployed systems in very sensitive contexts such as predictive policing and other criminal justice and financial services applications.

Notably, we've found these misconceptions to be quite common regardless of the amount of technical experience of the partner, ranging from policymakers to data scientists with training in machine learning. These observations, while anecdotal in nature, have helped form our opinion about the urgent need for making a pipeline-centric view of ML fairness more commonplace. \krcomment{I realize this is a bit high-level and not sure if we want to try to add some more specific stories/details, though given the page limit, we might also want to keep things a bit shorter.}

\krcomment{@rayid -- I'm not sure how much the fairness tree work with Lingwei has progressed, but if you've done more structured interviews with government partners, would it make sense to include anything from them here? Plus it only seems natural to have Lingwei as an author here given the RegLab/CMU overlap...}

%\subsection{Evidence from Regulation}
\subsection{The Regulatory Environment}\label{sec:regulation}
Recent developments in attempts to regulate the design and use of  ML systems has given a sense of urgency to support regulators and policymakers in these efforts. Based on our interactions with both of these groups, similar to students and practitioners, they do not have a good sense of the underlying causes of bias in ML systems and often struggle to both audit the systems that they are charged with regulating as well as in giving concrete and actionable guidelines to organizations attempting to comply with the regulations.

\rgdelete{Recent developments in the regulation of algorithmic decision systems, particularly around the search for \emph{less discriminatory alternatives} (LDAs), give a sense to urgency to the search for understanding and control the effects of decisions made throughout the ML creation pipeline on model fairness behavior. 

In US law, the disparate impact doctrine~\cite{USDOJ2021} states that in certain applications, e.g. credit, housing, and employment, companies which use ML systems (e.g. a loan approval model) that can be shown to lead to disparate impact across protected groups such as race or gender may be held legally liable. Importantly, if an alternative model (an LDA) which ``meets business needs'' but leads to lesser discriminatory impacts is discovered, the company may be legally required to use this LDA model~\cite{USDOJ2021}. The fact that the discovery of an LDA may lead to legal repercussions for companies, as well as a requirement to adopt the model, has the possibility to give plaintiffs a point of leverage to combat discrimination in deployed models in a variety of contexts, and also further provides incentive companies to prevent the deployment of discriminatory algorithms for which an LDA could be easily found. Recent work suggests that LDAs may actually be quite plentiful~\cite{black2022model,rodolfa2020case}, but how to most effectively search for them is still an open question--which has lead to repercussions. }

An example is a recent legal agreement in 2020 between the consumer finance firm Upstart, the NAACP, and Relman Colfax, a civil rights law firm. Upstart is an ML-based lending platform that attempts to expand access to credit by including non-standard variables in its assessment of creditworthiness. %For years, the NAACP and other civil rights activists expressed concerns over the use of attributes related to educational attainment, such as the name of the college applicants attended if they had a college degree~\cite{naacp_statement}. 
In order to address concerns by NAACP over the use of attributes related to educational attainment, the NAACP and Upstart agreed for Upstart to enter a Monitorship under Relman Colfax, that found statistically significant differences in approval for Black and white applicants~\cite{colfax2021report2report3}. Instead of taking a pipeline-aware approach, they took yet another ad-hoc approach which simply intervened at the feature selection step, and searched the feature space for a model with a subset of features that was less discriminatory. That is, the practitioners created a model for several different feature combinations, and tested the disparate impact of each one. This approach resulted in an expensive, inefficient, and an ineffective process that could've been avoided if there were tools to effectively search for alternate models using a pipeline-based approach---i.e. having tools to consider an ML system holistically and diagnosing what modeling choices may be exacerbating biases---the ML pracitioners performing the search may have been able to more easily identify effective mitigation points, instead of performing a blind, near-exhaustive search of the feature space. And, a pipeline-based approach would still evade the legal problem of relying on protected attributes during model training.

It is imperative that this does not become standard or accepted in the credit industry. Developing tools to operationalize a pipeline-based approach will allow model practitioners to create more efficient, and exhaustive searches for models which perform similarly to a baseline but have lesser disparate impact. Beyond searching for better models, tools informed by a pipeline-based approach may also aid in creating more standard and rigorous approaches to algorithmic audits more broadly. 

\rgdelete{
who would gain access to Upstart's model. During this monitorship, Relman Colfax would test whether Upstart models did in fact lead to disparate impact, and see if they could find (and thus recommend that Upstart replace their model with) a less discriminatory alternative model (LDA). While the NAACP notes this historic agreement will serve as ``guidepost to align industry underwriting and fair lending testing practices with the goals of equity and financial inclusion,'' it is likely that this process will influence and set a precedent for the search of LDAs more broadly.

After establishing that Upstart's model did have statistically significant differences in approval for Black and white applicants~\cite{colfax2021report2report3}, the ML practitioners crafted a method to search for an LDA. 

Fearful of using any of the most popular algorithmic fairness approaches (e.g. adversarial data debiasing, adding constraints to model training) over concerns that they would bring about their own legal problems by relying on the protected attribute during model creation~\cite{colfax2021report2}, they instead employed a ``more traditional statistical approach'' which simply intervened at the feature selection step, and searched the feature space for a model with a subset of features that was less discriminatory. That is, the practitioners created a model for several different feature combinations, and tested the disparate impact of each one. 

This approach is expensive, inefficient, and inexhaustive. 
Firstly, while earlier reports suggest plans for collecting new data to mitigate disparity, or investigating other areas of the decision pipeline affect disparity, the final report establishes that the only avenue for searching for LDAs undertaken is searching among various feature combinations---suggesting that the monitorship ran out of time and funds to effectively search for an LDA using this approach. 
Secondly, by the time an LDA was discovered with this method (two years later), Upstart already changed its underwriting model, rendering the search effectively useless for suggesting an LDA.
Thirdly, while an LDA was found, it had slightly worse business performance than the original model---which raises the legal question of how much cost Upstart can be asked to incur for implementing that alternative model~\cite{colfax2022report3}. This LDA was chosen based off of searching only \emph{one} point of intervention---if there had been time and money for a more exhaustive search of interventions in other areas of the modeling process, it is likely a better LDA could have been found. 
}

%As the authors of the report noted, there was insufficient budget and capacity to even test all possible feature combinations~\cite{}

%involved effectively something approaching a pipeline-based approach to search for a LDA: however, there was available no infrastructure to do so, and so the practitioners 

% For years, civil rights activists expressed concerns over the potential for discriminatory effects of Upstart Inc's credit granting platform. Upstart is a consumer finance firm which attempts to expend access to credit by including non-standard variables in its assessment of creditworthiness. 
% Years of expression of concern from civil rights activists on the possibility of discriminatory lending practices  Upstart, Inc. and the NAACP entered a legal agreement 
% for Upstart to undergo a monitoship by Relman Colfax, a civil rights law firm, to serve as an independent fair lending Monitor to evaluate and make recommendations regarding the fair lending implications of Upstart’s lending platform. 

% Upstart is a 


% Specifically, a recent advanced notice of proposed rulemaking (ANPR) from the Federal Trade Comission (FTC) suggests the possibility of stricter rules around the deployment of discriminatory systems~\cite{ftcproposed}.
% One of the questions of the ANPR asks: "Should [the commission] consider new trade regulation rules that bar or somehow limit the deployment of any system that produces discrimination, irrespective of the data or processes on which those outcomes are based? ". Additionally, a recent update to the Consumer Finance Protection Bureau (CFPB) examination manuals  suggests discrimination can now be seen unfair as it’s defined under the Dodd-Frank Act, again suggesting a turn towards more enforcement of reducing discrimination in algorithmic systems~\cite{cfpb_2022}.\footnote{ In other words, ''Discrimination may meet the criteria for ``unfairness'' by causing substantial harm to consumers that they cannot reasonably avoid, where that harm is not outweighed by countervailing benefits to consumers or competition.''~\cite{cfpb_2022} \ebcomment{must check with logan} This is in contrast with other interpretations of unfairness that only require that the discriminatory practice services a business need.} This means that companies which use machine learning systems relating to credit, housing, employment, and other applications covered by the disparate impact standard may be more likely to be held legally responsible if a model is shown to be discriminatory. Additionally, if a \emph{less discriminatory alternative} (LDA)---an alternate model which meets business needs but displays less discriminatory behavior against protected groups--- is found, it may be legally required to use this model.

% The fact that the discovery of an LDA may lead to legal repercussions for companies, as well as a requirement to adopt the model, has the possibility to give plaintiffs a point of leverage to combat discrimination in deployed models in a variety of contexts, and also further provides incentive companies to prevent the deployment of discriminatory algorithms for which an LDA could be easily found. While the task of finding an LDA may seem daunting, recent work around the concept of \emph{model multiplicity}---the phenomenon of multiple models for a given prediction task which equivalent accuracy but various other  properties, such as fairness---suggests that LDAs may be plentiful. 

% To date, there are no examples of legal action taken under the disparate impact standard against a company due to the behavior of an ML model. However, in 2020, the Upstart Network, Inc., a consumer finance company which attempts to 
% %is one example of an ML system that was investigated for discrimination under the disparate impact standard:

==> versions/pip_fair_1.tex <==
\section{Defining Pipeline Fairness}


\subsection{The AI Pipeline.} 
%The abstraction-based view of fairness can draw attention away from the fact that each step made along the \emph{AI model creation pipeline} can influence the fairness of a model's behavior.
To understand pipeline fairness, we need to understand the AI pipeline, or the process of creating an AI model for a given application. 
%The process of creating AI models for a given application 
This process is complex:
myriad choices are made during model creation, from the profound to the seemingly inconsequential. 
%We outline the major steps of the AI pipeline, and give examples of some of the many choices that are made within each step, in Figure~\ref{pics/pipeline_fig}. 
For example, in order to construct a loan decision model for a bank, a decision has to be made about how to translate the bank's overall objective, i.e., deciding who to grant loans to, into a prediction target. Some examples for what might be chosen may include: predicting the probability of the client's default, or the amount of money gained by the bank per client, or something else entirely. This process is known as \emph{problem formulation}~\cite{passi2019problem}. There has been a string of work enumerating fairness problems that arise from problem formulation, particularly through connecting to the social science concept of \emph{validity}~\cite{hoda, othervalid}. 

Next, the data to train the model has to be chosen, potentially linked across several sources, and cleaned. This involves making choices---or implicitly accepting previously made choices---about how to sample, label, link, and omit data. There are many opportunities for bias throughout these steps: 
\begin{itemize}
    \item Sampling
    \begin{itemize}
    \item Only available based on condition (e.g., released from jail in risk assessment tool datasets)
    \item Demographically unrepresentative (e.g. gender shades)
    \item Temporally unrepresentative (based on policy changes, etc)
\end{itemize}
    \item Labeling
    \begin{itemize}
    \item Measurement error differing across demographic populations (e.g. non-native speakers responding to survey)
    \item Societal bias making data unreliable across demographic populations (e.g. criminal justice arrest data)
\end{itemize}
    \item Cleaning
    \begin{itemize}
    \item Non-IID data dropping (e.g., dropping names with undefined characters in a dataset)
    \item Links across datasets may be differentially reliable across populations
\end{itemize}
\end{itemize}

Practitioners must then decide how to construct features from available information for use in the model, and which of the constructed features to for prediction, often referred to as \emph{feature engineering}. 


On a lower level, model practitioners must decide what type of model will be used, the learning rule and objective function, regularizers, the values of hyper-parameters determining normalization and training procedures, how the dataset will be split into train-test- and validation folds, among many other decisions made continuously throughout model development~\cite{lehr2017playing, kim2022race}. Practitioners will also have to decide what performance metrics will be used to evaluate models, and finally, how the model will be used in practice (e.g., with or without human involvement, how model predictions will be communicated and integrated into a larger decision system). (We define the steps of the AI pipeline in more detail in Section~\ref{pipeline}). 
All of these decisions then impact how it makes its own decisions, and thus its prediction behavior. 

\paragraph{Pipeline Fairness}
A pipeline-based view of fairness, then, considers each step of the AI pipeline as an intervention point to achieve a given fairness goal---and considers the effects of each choice during model creation on system behavior.
Importantly, those modeling choices are often practically changeable. While modeling choices are often made in search of the most accurate possible model, recent work has shown that there are usually many potential models--made with different modeling choices---with equivalent performance that can be created for any given prediction problem, while displaying considerably different fairness behavior~\cite{black2022model,blackleave2021,marx2019,rodolfa2021empirical}.

\paragraph{Benefits of Pipeline Fairness}
The pipeline approach to fairness is a method of augmenting our understanding of how to address fairness problems, not replacing the current most popular methods. 
Firstly, the pipeline approach to fairness can often unearth root causes of bias in a system, and thus point directly to mitigation techniques: e.g., if a faulty prediction target is chosen for a problem, choosing a different one can decrease discrimination~\cite{obermeyer2019dissecting,black}. Additionally, since the anti-bias intervention directly targets a source of bias, instead of putting an additional constraint on top of the system, this can lead to mitigation techniques that have lower performance-accuracy tradeoffs than abstraction-based methods~\cite{irs}. 
Further, while pipeline-based fairness mitigation is separate from creating definitions of fairness, many have pointed out that not all fairness problems are encapsulated by these abstracted, largely input/output based ideas of fairness. 
By reducing the problem of unfairness to a question of inputs and outputs, we may narrow our perception of what unfair behavior means to only include those factors. By using a pipeline-based approach, may naturally uncover unfairness which may arise not only from a system's outcomes, but also by the process by which it reaches a given decision. For example, a decision process may rely on attributes that seem normatively or legally dubious--- such as a recidivism prediction model which determines a defendant's ability to walk free between their arrest and their court date based on the criminal history of their parents and friends~\cite{angwin2016machine}; or a decision process may be unfair because it is highly
arbitrary or unstable—--such as a bank effectively flipping a coin to determine who gets a loan~\cite{blackleave2021}.
Further, while the transportability between contexts which comes from abstraction is useful, this generality can come at a cost to specificity, thus at times harming the applicability of common fairness metrics in real-world contexts---paying attention to the details of the system as pipeline fairness requires can also serve as a method of unearthing more contexutalized notions of fairness.


%DO WE WANT THIS SOMEWHERE%%
We note that ``pipeline fairness'' is simply a name for a mode of investigation that has already been underway in the algorithmic fairness literature since its inception---however, to the author's knowledge, there is no explicit paper tying the dispersed works that leverage the AI pipeline for fairness interventions together, connecting and collecting them under one roof. The goal of this paper is to do so, drawing attention to the phenomenon of pipeline fairness, as we believe that this technique is a promising future direction for expanding the algorithmic fairness toolbox, and deserves the focus and attention of the academic community. 

==> versions/pipeline_fairness.tex <==
\section{The ML Pipeline and Sources of Unfairness}
\label{sec:pipfair}

%\subsection{The ML Pipeline.} 
\begin{figure}
    \centering
    %\includegraphics[scale=0.5]{pics/base_pipeline.png}
    \includegraphics[width=\textwidth]{pics/Pipeline Fairness Figs.png}
    \caption{The pipeline--will make this better.}
    \label{fig:pipeline}
\end{figure}

%The abstraction-based view of fairness can draw attention away from the fact that each step made along the \emph{AI model creation pipeline} can influence the fairness of a model's behavior.
To understand the Pipeline-aware approach to fair-ML, we need to understand the ML pipeline, or the process of creating an ML system for a given application.\footnote{We note that many works have already outlined the machine learning pipeline in general terms and include sources of bias, but cover it here for completeness.}
%The process of creating ML models for a given application 
This process is complex and iterative:
myriad choices are made at each step, which we give examples of below, as well as in Figure~\ref{fig:pipeline}.\footnote{We do not list every possible choice that is made during ML model creation, but encourage researchers and practitioners to add to examples of what choices can be necessary to make during the ML creation pipeline at *link here*} We first present the steps of the ML pipeline, and then delve into examples of fairness problems that can arise along each step of the pipeline. 
We note that the ML pipeline itself is also embedded within a larger social context, and the boundaries of these systems can be fuzzy. It is true---and discussed in the literature[CITE]---that the larger social context into which an ML system is embedded has affects its behavior. However, in this work we focus on the pipeline more narrowly defined, in our attempt on drawing attention to, and further discovering, the mapping between modeling choices and fairness impacts. 

We break down the ML pipeline into the following steps: 
\begin{enumerate}
\item \textbf{Viability Assessments:}  Deciding whether or not to include an ML component within the decision-making system. 
%Decisions here include determining if the benefits of introducing an ML system in the given system outweigh the costs, and determining if there is organizational capacity to maintain an ML system appropriately. 
Some of the sources of harm in this step include skipping this step entirely, or allocating inappropriate resources towards developing, integrating, and maintaining the tool \hhedit{before establishing its net benefit} (e.g., for training staff, monitoring the system throughout deplyoment). 
\item \textbf{Problem formulation:} Translating the complex policy or business problem into a \hhedit{predictive} problem. 
\rgdelete{As Passi and Barocas point out, business and policy problems ``must be made into questions that data science can answer''~\cite{passi2019problem}. 
For example, in order to construct a loan decision model for a bank, a decision has to be made about how to translate the bank's overall objective, i.e., deciding who to grant loans to, into a prediction target. Some examples for what might be chosen may include: predicting the probability of the client's default, or the amount of money gained by the bank per client, or something else entirely. Additionally, what attributes should be used to predict this target are often decided upon as well. }There has been a string of work enumerating fairness problems that arise from problem formulation, particularly through connecting to the social science concept of \emph{validity}~\cite{akpinar2022sandbox, othervalid, passi2019problem}. Some problems of bias that may come up here include: (1)  The choice of a biased proxy for a prediction target (e.g. re-arrest or re-conviction for a recidivism prediction model, since whether or not someone committed a crime cannot reliably be observed).
(2) The use of non-causally related or otherwise arbitrary factors in the prediction task.
    
\item \textbf{Data collection:}  Collecting or compiling data to train the model.
%The data to train the model has to be collected or compiled, often by linking data across several sources. 
This involves making choices---or implicitly accepting previously made choices---about how to sample, label, link, and omit data. Some questions include---What population will we sample to build our model? How will we collect this data? How will we measure our prediction task? How will we define a positive label based on the prediction task? Who will label our data?  How will we link across data sources? 
%Continuing with the example of the loan decision model, this may bring up the following decisions:
%supposing the prediction task is whether a client will miss a payment within the first 90 days, this involves deciding: what years of client repayment data should be used? How should incomplete files be treated? How should unreadable files be treated? How do we define and label missing a payment? Do we want to li

%\marginpar{\textcolor{blue}{I'm worried about repetition between here and the survey. How deep should we go into the discussion of things that can go wrong here, i.e. the fairness problems? Should we just define the pipeline? I also worry about the overlap between this and Suresh \& Guttag, EAAMO 2021 ~\cite{suresh2021framework}.}} \hhedit{I think this section shouldn't be more than a page long---all details need to go to an appendix. We should quickly get to our new contributions.}

There are many opportunities for bias throughout these steps such as Sampling Bias\citep{}, Labeling Bias\cite{}, and Linking Bias \cite{}.

\rgdelete{
\begin{itemize}
    \item Sampling Bias
    \begin{itemize}
    \item Only available based on condition (e.g., only those who filled out information release form when applying for loan can be a part of dataset)%(e.g., released from jail in risk assessment tool datasets)
    \item Demographically unrepresentative (e.g. data algorithm is trained on has fewer women than is represented in the applicant pool)%(e.g. gender shades)
    \item Temporally unrepresentative (e.g. based on policy changes, such as the bank changed minimum payment between collecting training data and deployment) % (based on policy changes, etc)
\end{itemize}
    \item Labeling Bias 
    \begin{itemize}
    \item Measurement error differing across demographic populations (e.g. non-native speakers responding to survey)
    \item Societal bias making data unreliable across demographic populations (e.g. criminal justice arrest data)
\end{itemize}
    \item Linking Bias
    \begin{itemize}
    \item Non-IID data dropping when linking (e.g., dropping names with undefined characters in a dataset)
    \item Links across datasets may be differentially reliable across populations
\end{itemize}

\end{itemize}
}
\item \textbf{Data pre-processing:} Steps to make data usable by the ML model--e.g., dropping or imputing missing values, transforming (standardizing or normalizing data), as well as feature engineering, i.e. deciding how to construct features from available information for use in the model, and which of the constructed features to use for prediction. 
%Continuing with the example of the loan decision model, this may bring up the following decisions: which client attributes should be used for prediction? Suppose one attribute is the number of past defaults. How is this computed--in the past year, five years, ten years?
Again, there are myriad ways for biases to enter through feature engineering decisions such as building features from data that is likely to be of higher quality for some groups, using data transformations with differential error rates across groups, imputing missing data in ways that have differential accuracy across groups, selecting features which are differentially informative across demographic populations, or choosing normatively objectionable features to use for a prediction task, such as whether or not the family members of a defendant have criminal records to determine whether they are recommended for release or to be jailed.

%How should incomplete entries be treated? Will we normalize or standardize data? 
\rgdelete{
\begin{itemize}
    \item Feature Creation and Imputation
    \begin{itemize}
    \item Building features from data that is likely to be of higher quality for some groups (e.g., distance-based features relative to a home address that is less likely to be stable/current for more vulnerable populations)
    \item Using data transformations with differential error rates across groups (e.g., using word embeddings trained on an English corpus for user-generated text that may contain submissions in other languages)
    \item Imputing missing data in ways that have differential accuracy across groups, or make minority group members look more like majority group members
    \item \ebcomment{help}
    \end{itemize}
    \item Feature Selection
    \begin{itemize}
    \item Choosing features which are differentially informative across demographic populations
    \item Choosing features which are proxies for a protected attribute \krcomment{I would probably remove this since this information can just as easily improve fairness as reduce it}
    \item Choosing normatively objectionable features for a prediction task, such as whether or not the family members of a defendant have criminal records to determine whether they are recommended for release or to be jailed
    \end{itemize}
\end{itemize}
}
\item \textbf{Statistical modeling:} Determining what type of model will be used and how it will be trained. Decisions here include: choosing the model type, learning rule and loss function, regularizers, and the values of hyper-parameters determining normalization and training procedures~\cite{lehr2017playing, kim2022race}. For example, choosing between linear, forest-based, or deep models; choosing the architecture of deep models; what constraints to add to the loss function, how to optimize that loss function (e.g. SGD or momentum), etc. Each decision here can lead to downstream bias such as choose a learning rule which is biased toward a certain subset of individuals in the data or over- or under-emphasizes outliers or minority populations.
\hhcomment{I would consider the choice of the optimization procedure as part of the model selection, not statistical modeling.}
\rgdelete{
\begin{itemize}
\item Hypothesis Class
\begin{itemize}
    \item Choosing a model with insuffient or too much power for the prediction task
\end{itemize}

\item Learning Rule
\begin{itemize}
    \item Chose a learning rule which is unstable for the given dataset
    \item Chose a learning rule which is biased towards a certain class (e.g., a the class with more features correlated with it)
    \item Choose a learning rule that over- or under-emphasizes outliers or minority populations (e.g. differentially private learning rules under-emphasize minority populations)
    \item Choosing a learning rule with inductive bias towards or against certain feautures
\end{itemize}
\end{itemize}
}

\item \textbf{Model selection and validation:} The processes by which a model is determined to be performing well, both in relation to other models in the training set, but also on unseen data. Common sources of bias here include metric underspecification or misspecification (not including notions of bias or including inappropriate notions of bias for example)  as well as using improper data for testing or validation (typically that is not representative of the deployment scenario)

% For example, will a model be evaluated only on its predictive accuracy? AUC? F1 score? On fairness metrics as well (which)? Some notion of privacy or robustness? 
\item \textbf{Deployment and integration:} How will the model be used as a component of the decision system into which it is embedded? Will the model's predictions directly become the final decision? If there is human involvement, where and how? How much discretion do humans have over adhering to model recommendations? How are model predictions communicated to decision-makers? Each of these choices cause bias in the eventual decisions being made and on the people being affected.
%(e.g., with or without human involvement, how model predictions will be communicated and integrated into a larger decision system). 



\hhdelete{A pipeline-based view of fairness, then, considers each step of the ML pipeline as an intervention point to achieve a given fairness goal---and considers the effects of each choice during model creation on system behavior.}

%We outline the major steps of the ML pipeline, and give examples of some of the many choices that are made within each step, in Figure~\ref{pics/pipeline_fig}. 
%\paragraph{Viability Assessments}
%Viability assessments refer to the process an organization goes through when deciding whether or not to include an ML system within its decision-making framework. Decisions here include determining if the benefits of introducing an ML system in the given system outweigh the costs, and determining if there is organizational capacity to maintain an ML system appropriately. Some of the sources of harm in this step include skipping this step entirely, or allocating inappropriate resources towards developing, integrating, and maintaining the tool (e.g. for training staff, monitoring the system throughout deplyoment). 


%Passi and Barocas~\cite{passi2019problem} provide an in-depth explanation of problem formulation and the choices that are made within this process. 

%There has been a string of work enumerating fairness problems that arise from problem formulation, particularly through connecting to the social science concept of \emph{validity}~\cite{hoda, othervalid}. 




% \hhcomment{I suggest we move a summarized version of the following arguments (i.e., 2.2 and 2.3) to the intro. It feels out of place here.}
% \subsection{Benefits of Pipeline Fairness}
%  Firstly, the pipeline approach to fairness can often unearth root causes of bias in a system, and thus point directly to mitigation techniques: e.g., if a faulty prediction target is chosen for a problem, choosing a different one can decrease discrimination~\cite{obermeyer2019dissecting,black2022algorithmic}. Additionally, since the anti-bias intervention directly targets a source of bias, instead of putting an additional constraint on top of the system, this can lead to mitigation techniques that have lower performance-accuracy tradeoffs than abstraction-based methods~\cite{black2022algorithmic}. 
% Further, while pipeline-based fairness mitigation is separate from creating definitions of fairness, many have pointed out that not all fairness problems are encapsulated by these abstracted, largely input/output based ideas of fairness. 
% By reducing the problem of unfairness to a question of inputs and outputs, we may narrow our perception of what unfair behavior means to only include those factors. 

% A pipeline-based approach may naturally uncover unfairness which may arise not only from a system's outcomes, but also by the process by which it reaches a given decision. For example, a decision process may rely on attributes that seem normatively or legally dubious--- such as a recidivism prediction model which determines a defendant's ability to walk free between their arrest and their court date based on the criminal history of their parents and friends~\cite{angwin2016machine}; or a decision process may be unfair because it is highly
% arbitrary or unstable—--such as a bank effectively flipping a coin to determine who gets a loan~\cite{blackleave2021}.
% Further, while the transportability between contexts which comes from abstraction is useful, this generality can come at a cost to specificity, thus at times harming the applicability of common fairness metrics in real-world contexts---paying attention to the details of the system as pipeline fairness requires can also serve as a method of unearthing more contexutalized notions of fairness.

% \subsection{Limitations of Pipeline Fairness}
% \begin{itemize}
%     \item Symmetrically, pipeline fairness suffers from a lack of abstraction, often leading to a lack of generalizability. However, we take this as a challenge for the field: how can we generalize techniques from a pipeline-based approach? 
%     \item One step is to interrogate pipelines over many, many implementation contexts, and see where patterns emerge--this is why we have created a collaborative document to document the effects of various modeling choices on fairness behaviors in a variety of contexts
    
 \end{enumerate}

==> versions/redone_survey.tex <==
\section{A Survey of Pipeline-Fairness}
\label{sec:litreview}

\ebedit{As a first step towards operationalizing the pipeline-based approach to fairness in ML, we provide a review of the ML fairness literature focused on creating a taxonomy of fairness work that locates, measures, or mitigates problems along the ML pipeline. In addition to serving as a first step towards a resource that ML practitioners can use to identify ways to diagnose and mitigate problems in their pipeline, our survey of the work already done allows us to point to the gaps in the literature that must be addressed in order to have a full understanding of how choices made along the ML pipeline translate to model behavior-- and then build tools which operationalize this understanding to build more effective systems.}

%We focus on work that does not fall into the category of adding an optimization constraint to a model in order to enforce a fairness metric, or resampling data, in order to highlight how 


\subsection{Survey Methods and Organization.}

\hhcomment{I think we can justify our focus on ML venues by saying that we were interested in measures and remedies that could be useful to ML practitioners; hence the focus on these venues.}

In order to better understand the current landscape of algorithmic fairness research throughout the ML pipeline, we performed a thorough survey of the recent \krdelete{algorithmic fairness }literature, which we classified depending upon which area of the pipeline they analyze. We gathered papers from NEURIPS, ICML, ICLR, FAccT, and AIES, for the past five years, i.e. 2018-2022, that contain any of the following terms in their title, abstract, or keywords: "fairness", "fair", "discrimination", "disparity", "equity".\footnote{When available: this is with the exception of NEURIPS, which we gather for years 2017-2021 due to the date of the conference relative to the time writing this work, and EAAMO, which started in 2021.} In addition, we performed a series of Google Scholar searches to ensure our survey did not miss high-impact work published in other venues: One search used the keywords listed above and included papers published in any venue in the past five years with over 50 citations, through the top 50 results returned by this Google Scholar search. \krdelete{This is to ensure that we do not miss any high-impact work from other venues. Finally, we perform} Additional Google Scholar searches used keywords from each step in the pipeline individually, to attempt to find papers targeted at each stage: for example, "data collection" and "fairness" and "machine learning". This results in \textcolor{orange}{\textasciitilde1000} papers overall. 

We then manually inspect each paper to understand whether and how the reported research is an instance of a pipeline\hhedit{-aware} approach to fairness. That is, does it identify, measure, or mitigate a concrete cause of unfairness due to choices made in a specific stage of the ML pipeline. If so, we categorize the paper along two axes: what part of the pipeline it corresponds to (problem formulation, data choice, feature engineering, statistical modeling, testing and validation, or organizational realities), and whether it identifies, measures, or mitigates a pipeline fairness problem. 

\rgdelete{While we acknowledge that adding optimization or loss constraints to a model to enforce a given definition of fairness is in itself a modeling choice and thus fits in to the ``pipeline'' notion of fairness \hhedit{(specifically, under the statistical modeling, choice of the objective function)}, we separate these more traditional fairness papers from our understanding of pipeline-based fairness papers for the sake of this survey by giving them their own category, which we call ``Algorithm''. }\krcomment{Not too sure I see the necessity of calling out this distinction separately -- aren't we just saying the choice of algorithm is one component of the pipeline? Especially given the length, maybe just cut?}
\rgcomment{i agree with Kit - deleted that for now in the text}


\subsection{High-Level Overview and Takeaways}
\begin{itemize}
    \item Our first observation is that the number of fairness papers that adopt a pipeline perspective to fairness is far outnumbered by the more traditional, abstracted approach to fairness: XXX papers versus XXX papers overall. \hhcomment{Might be nice to do a histogram, showing numbers per pipeline stage.}
    \item The algorithmic fairness literature has a dearth of knowledge about what on-the-ground pipelines look like: although there are many papers that outline abstracted pipelines (including our own), the actual model creation steps taken by practitioners for a variety of real-world systems (e.g. in consumer finance, healthcare, hiring systems) are at the very least not cataloged in any centralized place. 
    \hhcomment{The point being made here is not clear to me.}
    \item Even within the list of papers that do take a pipeline-based approach, the majority of them are \emph{proof-of-concept}: there is much work to be done to take the solution proposed in the work into an implementable and generalizable fix for pipeline problems.
    \item Most fairness-related papers focus on \emph{one issue} in the pipeline, but fail to provide insight into how these different aspects of the pipeline interact. Does solving each issue in isolation work?
    \item Within those papers, the majority investigate problems with data collection and pre-processing as an arbitrary approach to ``fixing'' fairness.
    \item Many of the pipeline papers still engage with one particular notion of fairness (often demographic disparity). It would be helpful to create a more generalized mapping of how modeling choices change prediction behavior, beyond a single metric.
    \item There is a dearth of case studies of bias mitigation in the fairness literature. Though case studies may often be disregarded as ``simply implementing old methods'' and thus not novel, it is crucial that we give them more attention so that we can learn about the failure modes of the techniques that we create. While there are \hhedit{notable} papers about the overall problems of production teams, e.g. ~\cite{madaio2020co,holstein2019improving,sambasivan2021everyone}, these still do not provide in depth-detail of the bias mitigation process in deployed systems. 
\end{itemize}



\subsection{Viability Assessments}
To the author's knowledge, there is very little work within the fairness literature on documenting, or detailing the bias that can arise out of, or mitigating bias from the viability assessment process

\rgdelete{: how we investigate the benefits and downsides of the current decision-making system in place in comparison to what an ML-based solution could provide, and assessing organizational capacity for effective system \hhedit{evaluation, design, and deployment. Important considerations in this category include (but are not limited to) access to high-quality data, sufficient ML expertise, capacity for continued monitoring.}}

Viability assessments provide an avenue for refusal to build an ML system, which is understudied in the fairness literature\hhedit{~\citep{raji2022fallacy}}. Though there have been discussions in the community around when to refuse to build~\cite{barocas2020not}, there is little published work on case studies detailing how the decision to build or not build was made. --- et al~\cite{find_that_paper} point to the fact that ML researchers and practitioners do not often consider the option to not build a system because it is taken as the default, given the pressures (and funding) coming from the tech industry. Indeed, many works that point to how organizational factors---such as lack of a company's support for ethical AI approaches, or time pressure, or focusing only on client demands~\cite{passi2020making} can lead to pushing ML systems ahead without careful consideration of whether or not deploying a system in that domain is a net benefit in the given context. One resource, Data Science for Social Good Scoping Guide \cite{DataScienceScoping} highlights some of these issues  and gives practitioners some questions to ask at the viability assessment stage of a project.
\krcomment{Not published in an academic venue, but perhaps we should point to the DSaPP Scoping Guide here, as well as specific fairness/inclusion issues it details? http://www.datasciencepublicpolicy.org/our-work/tools-guides/data-science-project-scoping-guide/}

\paragraph{Key Takeaways:}
\begin{itemize}
    \item Work around the fairness implications of viability assessments for ML systems is almost entirely lacking in the FairML literature, leaving appreciable open questions around decisions of whether or not to build a system, stakeholder engagement, and identification of overall goals of a project.
\end{itemize}


\subsection{Problem Formulation}
Problem formulation encapsulates the decisions made when translating a nebulous policy or business goal into an ML task and often consists of various decisions made: e.g. deciding who is in the cohort that the ML system will be used on, translating ``predicting creditworthiness'' into ``predicting loan default''~\cite{passi2019problem}. 

Problem formulation is also a time to assess whether a proposed ML system will address the actual needs of the organization to which it will be deployed. 
While not describing this process as problem formulation per se, Katell et al. detail how their design ideas changed over time through their engagement with community stakeholders while building an Algorithmic Equity Toolkit to aid activists in participating in public comment session when evaluating ML systems to be used by the Seattle city government~\cite{katell2020toward}; and Suresh et al~\cite{suresh2022towards} detail how they co-designed a tool for collecting news articles documenting cases of femicide. Creators of ML for Public Policy Lab class at CMU \cite{MLPolicyclass} highlight several decisions that need to be made in the problem formulation stage of the pipeline.

\paragraph{Selection of Prediction Target} 
While there is helpful discussion on how prediction target selection may lead to bias, often drawing from the social science literature of validity theory~\cite{passi2019problem,jacobs2021measurement,coston2022validity},
as well as examples of disparities stemming from prediction target selection selection~\cite{black2022algorithmic,obermeyer2019dissecting,human_rights_watch_2020}, to the author's knowledge, there is little work in the ML fairness literature detailing the process of problem formulation in practice, or leveraging fair ML tools to measure or mitigate the potential bias of the selection of a given prediction target ex-ante. 
Developing protocols for assessing problems of various notions of validity (internal, external, content, predictive) of the target variable and predictive attributes is a promising and necessary avenue of future work. There is preliminary work along this axis in the form of checklists and protocols, e.g.~\cite{coston2022validity}, but we suggest it may be possible to make a suite of quantitative tests as well.
For example, access to appropriate data, ML practitioners could leverage existing model-level bias-testing frameworks~\cite{AIF360,saleiro2018aequitas} to test for bias across a series of potential prediction tasks to inform the decision of which to choose. Tests for predictive validity simply require investigating whether the proposed target variable is predictive of other related outcomes. Obermeyer et al.~\cite{obermeyer2019dissecting} used such a test to uncover the racial bias behind using health care cost as a proxy for health care need, by regressing health care cost on other metrics of illness (e.g. the number of active chronic conditions a patient has), finding that there was a disparity in the correlation between health care costs and sickness in white patients versus that in Black patients. Investigating the extent to which questions of construct validity and reliability can be operationalized into a set of tests (e.g., testing correlations between potential prediction tasks, or checking for consistent model performance across two different methods of measuring the output) may be a promising area for utilizing tools and methods from social sciences.

\paragraph{Selection of Prediction Universe}
\krcomment{The choice of cohort/universe for analysis and when to make a prediction actually seems pretty salient in terms of formulation as well. Here I'm talking about things like up-front decisions about who to make predictions on: Suicide risk among everyone in the population or just people with some history of mental health needs? Do I predict the likelihood of not graduating high school as of 2nd grade, 9th grade, 11th grade, etc? I'm certainly not aware of anything in the literature that actually looks at this (either systematically or via case study). Did you identify anything there?}\hhcomment{This is a very good point, and it reminds me of a related but distinct set of recommendations around 'studying up'~\citep{barabas2020studying}.}

\paragraph{Selection of Predictive Attributes}
\ebcomment{Help.} \hhedit{The discussions of validity and reliability outlined in the previous paragraph are just as well applicable to the features utilized for prediction. Many such features may aim to reflect social constructs such as race or gender~\citep{}. Additionally, Prior work has observed that trained models may rely on spurious correlations, that renders their predictions unreliable in presence of confounders and slight changes to the data distribution. We believe that close deliberation with domain experts would allow for the appropriate selection of features.} \hhcomment{We can mention the DoWhy package as a tool here.} \krcomment{To avoid confusion, I might actually integrate this into the data acquisition or feature selection/engineering discussion -- I feel like in practice it's generally difficult to get to the detail of choosing specific predictors this early in the process}

\paragraph{Determining Behavioral Desiderata}
\hhcomment{I think the following paragraph should be moved to "testing and validation" section. The details of the examples you mention can be moved to an appendix. Citation to these pieces suffice.} \krcomment{I'm a little on the fence there -- generally I think it's important for some of this goal/fairness metric definition to happen up front, but it's hard to avoid some repetition. I guess in the interest of space, consolidating with testing and validation might be cleanest?}
While we leave the question of finding an appropriate fairness metric to other work and focus instead on bias mitigation techniques, we wish to highlight the importance of finding \emph{contextualized} notions of bias and fairness to encourage in a system. For example, Black et al.~\cite{black2022algorithmic} show how \emph{vertical equity}, the public finance notion that individuals with different incomes and wealth must be treated differently in order to achieve fairness overall, is not achieved by enforcing traditional fairness metrics--- instead, the authors favor audit selection models with more monotonic audit selection distributions, which also display high selection overlap with an oracle model which selects individuals in order of highest tax misreport (i.e. most money not reported to the Internal Revenue Service). Mattei et al.~\cite{mattei2018fairness} consider the unique fairness requirements of organ-matching systems, noting that it was important for younger organs to be matched to younger recipients, and also to ensure that individuals did not receive different probabilities of getting an organ due to their blood type. Other examples of contextualized fairness desiderata include [CITE HERE]. \ebcomment{This is not the best example because it's a matching system instead of an ML system-- does anyone else have a more contextualized notion of fairness in a prediction system example?}
%we briefly note that a pipeline fairness approach can also naturally lead to a more in-depth, contextualized understanding of the ML system, making it more natural to define more context-specific model behavior desiderata than the most common fairness metrics. 
%Case studies of fairness problems in real-world deployed systems are especially helpful in understanding what 

\paragraph{Key Takeaways:}
\begin{itemize}
    \item Although some work does exist on the importance of label choice to system fairness, including compelling case studies, little is available to practitioners in terms of operationalized tools to help inform this choice.
    \item Despite the significance of the choices surrounding the definition of the prediction universe for defining who might have an opportunity to receive a benefit, we were unable to find any work in the literature exploring the downstream fairness implications of these choices.
    \item \krcomment{Probably move predictors / desiderata to sections below?}
\end{itemize}

\subsection{Data Collection}
Far and away, besides enforcing fairness constraints on models during training or prediction, the aspect of the pipeline that has received the most attention is data collection.  

\paragraph{Mapping effects of faulty data collection to model behavior} Several papers in the algorithmic fairness literature have pointed to the problems of disparate performance and selection across demographic groups stemming from datasets which are unbalanced across demographic groups, i.e. have sampling bias, both in terms of sheer representation, and representation conditional on outcomes~\cite{buolamwini2018gender, mishler2019modeling}; or have data that is \hhedit{disparately noisy} or perturbed in some way~\cite{wang2021fair}. Li et al.~\cite{li2022data} do a particularly thorough job of testing how potential results of data collection problems---e.g. unrepresentative samples, insufficiently small data samples, differing group base rates\footnote{Which could be true or the result of measurement error}---influence machine learning model behavior from the perspective of accuracy and fairness. They test the influence of these sources of collection bias comparing performance across models  trained on subsamples of \krdelete{an enormous, novel,} a criminal justice dataset (1.5M rows). Interestingly, they find that increasing dataset size, or even reducing the disparity in base rates, does not always reduce disparities in selection, false positive, or false negative rates. Other recent work introducing new datasets for testing fairness interventions find similar results~\cite{ding2021retiring,akpinar2022sandbox}. These papers are an excellent start to mapping data bias issues in the pipeline and immediately brings to mind more questions---how do these sampling and measurement errors impact other fairness desiderata, how do they interact with other pipleline choices such as model selection, loss function selection, and hyperparameter tuning? 

\paragraph{Mitigating biased model behavior on biased data}Proposed techniques for mitigating the effects of unrepresentative data include a variety of synthetic data augmentation techniques~\cite{sharma2020data, van2021decaf, chawla2002smote}, data re-weighting techniques~\cite{kallus2018residual}, and specialized optimization functions for creating fair classifiers (according to traditional metrics) with unbalanced data~\cite{jiang2021towards, li2021autobalance}. Coston et al. introduce a model training approach that can mitigate the effects of the selective labels problem~\cite{coston2021characterizing}.


Some argue that using modeling techniques such as re-weighting or using special loss functions serve as a band-aid solution, and argue that data problems should be solved by intervening on the data. Liu et al.~\cite{liu2021can} show how to find which subgroup in the data is likely to have noisy labels, and then introduce a technique of inserting \emph{more} noise into the labels of other subgroups in order to increase fairness and generalization, and often accuracy as well. Chen et al.~\cite{chen2018my} introduce methods of estimating the value of adding additional training samples from the perspective of thus improving many fairness outcomes such as equalized accuracy---potentially allowing for practitioners to decide whether searching for extra training examples or features is worthwhile.  


Several methods are also available for creating fair classifiers with noisy, corrupted or perturbed data~\cite{liu2021can}. 
Wei et al~\cite{wei2021learning} provide an interesting counterpoint to the papers which discuss creating fair classifiers on noisy data: they point to the differences in model behavior when trained with artificially noised data (i.e., following some specific noise distribution, such as Gaussian), as opposed to noisy data that is mislabeled by human annotators: for example, they show that harmful model memorization is much more common on models trained with mistakes in human annotations, since the human annotators mislabel examples that are inherently more confusing and thus informative for the model (e.g. a hard-to-distinguish photo).
As a form of solution, they provide a new noised version of CIFAR-10 and CIFAR-100 with errors by human annotators to better study the problem of noisy data in practice. 
This paper points to the peril of training and evaluating models on ``sterile'' data: they point out that our intuitions about the effects of noisy data on model behavior may be flawed, underscoring the need to test for pipeline-based problems and solutions on pipelines data to be used during deployment.
\krcomment{Seems like we should discuss approaches that focus on resampling/balancing the training data here as well -- similar to the inconsistency above, in our method comparison work (https://arxiv.org/pdf/2105.06442.pdf), we found a lot of variability across datasets and parameters in the ability of resampling to have any impact on model fairness. Some of the references there are a bit older, but we could also point to them for others looking at resampling (see the "Resampling" heading on page 2)}



%Cai et al~\cite{} suggest to a method of selecting individuals to seek labels for in order to improve the system the most from an equity standpoint. 
%Sharma et al.~\cite{sharma2020data} introduce a method of data augmentation which guarantees improvements in reducing demointroduces data with perturbations to the demographic group (i.e., switching demographic group) while keeping other feature and labels constant, as well as keeping demographic group constant and flipping outcome labels, crucially, slowly in order of likelihood within the probability distribution--- creating a family of datasets

\paragraph{Sources of bias in the sampling and labeling process} While several of these papers do show how machine learning systems change their behavior as a result of different kinds of data noise or unrepresentativeness~\cite{wang2021fair}, they do not speak to the source of bias in the sampling or labeling process, and how to correct it at the source. The Human and Computer Interaction community has done a much more thorough job of considering what failure modes can occur in the data collection process itself, especially as a result of crowd sourcing data set labels with workers from platforms such as Mechanical Turk~\cite{sen2015turkers,hube2019understanding,miceli2020subjectivity}. For example, Diaz et al~\cite{diaz2022crowdworksheets} point to the fact that crowdworker identities influence how they answer labeling prompts~\cite{sen2015turkers} \krcomment{The references here are confusing -- how does the Sen 2015 reference relate to this sentence?}, and introduce CrowdWorkSheets, a worksheet to help guide practitioners through, and allow them to document, the process of creating a dataset with crowdsourced labels with crowdworker identity in mind, from specifying the question of what crowdworkers are to label, to accounting for demographic differences in crowdworkers, determining compensation, among other considerations. However, they do not test the use of their worksheet on production teams. 
An exemplary paper by Sambasivan et al.~\cite{sambasivan2021everyone} provides a wider set of examples of real-life sampling bias and labeling bias, and importantly, \emph{how they entered a real-world system}.  In one set of examples, ``physical world brittleness'' brought about several senses in which deployment data was distributionally different from training data, leading to failure modes, and often abandonment of the AI project: e.g. ``hardware drifts'', where hardware systems which were the source of medical imaging data were not updated over time, leading models to give inaccurate results; or ''human drifts'' where human behavior changed over time leaving models useless, such as models build to predict disease spread over the course of the Covid-19 pandemic.  Another large failure mode identified was a lack of ``cross-organizational documentation'', which lead ML practitioners to make assumptions about aspects of the data, such as timestamps, introducing severe noise into the training data. 

The above papers are a great source of general pointers to data collection problems ignored in the ML literature, but there is still a dearth of deep investigations into \emph{specific} data creation pipelines and the particular sources of bias that show up in those systems, as well as contextualized mitigation strategies. 
There are some exceptions: Marda and Narayan~\cite{marda2020data}, show sources of historical bias, sampling bias, measurement bias, and direct discrimination as well as arbitrariness in the collection of data for the creation of Delhi's predictive policing system: for example, for measurement bias, they explain how the techniques used to map Delhi were inconsistent over the development of the tool, since the police department's ArcGIS system license expired; that there were often no formal addresses for less wealthy parts of the city thus identifying call location was largely guesswork; and that women who made calls were less likely to know their address since they often largely stay inside and are less aware of their surroundings.

More generally, while this literature does an excellent job of illuminating failure modes that can be surfaced through engaging with practitioners---since many papers in this area are structured around interviews---they may elide more low-level technical sources of data collection problems, such as record linkage issues leading to non-IID data dropping. While they are extremely helpful in the important first step of identifying problems, they provide little direction for creating operationalizable solutions to these problems, or even sufficiently detailed information about each system studied to be able to understand the mapping between data collection problems and model behavior.\krdelete{

Operationalization of a pipeline-based approach to fairness necessitates harnessing both the outcomes- and solution- focused algorithmic fairness literature which ignores the sources of problems, and the problem identification prowess of the HCI, CSCW, and other literatures. 
}
One paper by Goel et al.~\cite{goel2019crowdsourcing} comes closer to operationalization of a solution for a specific problem in the data collection pipeline: differential accuracy of crowdworkers in labeling tasks. They introduce a technique for assigning Mechanical Turk workers to labeling tasks in order to decrease disparity in false positive and false negative labels. It requires a subsample of datapoints (gold tasks) where the researchers know the true label of the data to be labeled in order to estimate the group-wise accuracy of each labeler. However, crucially, they do not test their technique in their own labeling task, but use datasets already annotated with Mechanical Turk workers as well as synthetic data---such approaches must be tested within actual labeling processes. 

\krcomment{There's a lot here on crowdsourced labels -- I guess because it's an easy system where the researchers have control over the label generation process -- and I think we can shorten it down to a paragraph or so. Seems like we should also point to some of the more real-world instances of label and sampling biases: differential enforcement of drug laws and biases in traffic stops come to mind as some of the important examples there. Of course, much harder to address without fixing the world. Likewise, seems like some of the work around biases in facial recognition arising from lack of representation in training data fits in here as well. 

\url{https://drive.google.com/file/d/1B58Os2Hb2v__YQ8whdWRULY9mgxxsHoO/view}

@Rayid -- I'm having trouble finding the drug arrests paper I'm thinking of right away (I think it looked at Oakland vs Berkeley?) but you might know it off-hand?

http://proceedings.mlr.press/v81/buolamwini18a/buolamwini18a.pdf
}
 
\krdelete{As a whole, we first note that while there is some excellent work in this area, data collection pipelines---and pipelines in general--continue to be poorly mapped, and thus not all sources of bias or failure are even identified. Secondly, there is a disconnect between problem discovery and mitigation techniques. While it may be that checklists, questions, and datasheets are the best solution to some sources of errors and bias in the data collection pipeline, (and the pipeline overall), there may be some more objective tests that can be performed to test whether data is being sampled, labeled, and measured in a defensible way. Thirdly, the work of mapping pipelines, identifying potential sources of bias within the choices therein, testing to see under what circumstances biases arises, and creating and testing mitigation techniques, is work that, to the extent that is has been done, is spread across multiple disciplines: from machine learning to database management. We should search for, study, and adopt techniques from these areas in order to create a mapping of machine learning pipelines for bias prevention.  
Finally, and perhaps most importantly, \emph{proposed methods should be tested in a variety of real-world systems} to see where they fail and when they are helpful. }

\paragraph{Key Takeaways:}
\begin{itemize}
    \item While there is some excellent work in this area, data collection pipelines---and pipelines in general--continue to be poorly mapped, and thus not all sources of bias or failure have likely even been identified.
    \item There is a disconnect between problem discovery and mitigation techniques. Although checklists and datasheets may be a solution to some sources of data collection bias, there is a lack of more objective tests to ascertain whether data is being sampled, labeled, and measured in a defensible way.
    \item Empirical work the relationship between between dataset size as well as group and label balance has shown inconsistent results in terms of impacts on downstream disparities, highlighting the complexity of the problem and limitations of solving model fairness issues at the level of data alone.
    \item What work that has been done in this area is spread across multiple disciplines: from machine learning to human-computer interaction to database management. We should search for, study, and adopt techniques from these areas in order to create a mapping of machine learning pipelines for bias prevention.
    \item Most importantly, proposed methods should be tested in a variety of real-world systems to see where they fail and when they are helpful. \krcomment{maybe rephrase these last two more as gaps and move the calls to action to research agenda?}
\end{itemize}

\hhcomment{I think Datasheets is one paper that should definitely be discussed in this section. }

%posit that we must combine the literature of problem discovery from a variety of literatures and work towards potential mitigation tactics, crucially, tested in real-world systems. While this may not lead to generalizable results at first, another active area of research may be what aspects of prediction problems or pipelines lend themselves to certain types of solutions.

%Beyond these instructive examples, Sambasivan et al. also provide a helpful overview of available methods and attempts to prevent such problems from a variety of literatures, including human-computer interaction, and data management science, including methods of logging data cleaning steps~\cite{wrangler}, enforcing validity constraints on data~\cite{}, incentivising 


%, and given insights from Sambasivan et al.~\cite{sambasivan2021everyone}, it seems 
%points to the need to evaluate models on data with noise distributions , and the investigation of the fairness effects of real-world noisy data.

%The computer science literature is solution-focused, and often develops a technique to mitigate the problem identified---but often in the form of a generalized band-aid, not investigating the causes of the problem in the data. On the other hand, HCI and related literatures delve
%There have been very few papers which lay out the entire end-to-end process of 


%Both literatures suffer from focusing too much on painting a general picture---overarching themes of failure points in processes and generalized solution techniques. We also need a taxonomy of examples of specific problems that have occurred, and how they have been solved

%However, despite this literature being rich in documenting overall patterns of 

\subsection{Data Preprocessing}

While there are many papers in the fairness literature that discuss how to \emph{leverage} preprocessing for bias mitigation~\cite{Zhao2020Conditional,cheng2021fairfil,balunovic2022fair,zemel2013learning}, to the author's knowledge, there is little work detailing how preprocessing steps may \emph{introduce} bias. 

\paragraph{Feature Encoding and Missing Values} A body of work has explored how preprocessing steps---such as data representation (e.g. discretized or continuous numerical values) normalization techniques, and strategies for data dropping and imputation---can influence classification model behavior~\cite{alshdaifat2021effect,biswas2021fair,crone2006impact,zheng2003existence} in a model-dependant manner. These effects can often be significant: Crone et al~\cite{crone2006impact} state that that the performance differences between preprocessing steps often rivaled that of the differences between using different models (SVM versus NN). In the context of predicting purchase behavior online, Zheng et al.~\cite{zheng2003existence} state that different methods of encoding the unit of analysis (what consititutes a purchase session) lead to ``radically different conclusions'' from model behavior.
Given that preprocessing can drastically influence model prediction performance, it must influence fairness behaviors as well. However, there is little work in this area. Biswas et al.~\cite{biswas2021fair} perform an analysis of how different preprocessing steps can influence fairness behavior, and show, among other effects, that dropping rows of a dataset with missing values instead of imputing those rows can lead to sizable differences in fairness behavior due to the changes to the training distribution. While this paper is an excellent first step, it would be instructive to understand how a larger array of (potentially context-specific) preprocessing steps lead to changes in model behavior---for example, how exactly different features are defined, e.g. encoding attributes such as age in various datasets in continuous or binned. Other avenues for future work include investigating fairness impacts beyond the metrics discussed in the paper,  how these data preprocessing steps interact with the inductive biases of a larger variety of models, and developing methods for how to choose between preprocessing options given information about the data and the modeling pipeline.
%Another large area of focus is methods for ``debiasing'' data by making a representation of the training data which is independent of the protected attribute~\cite{Zhao2020Conditional,cheng2021fairfil,balunovic2022fair,zemel2013learning}, which we do not focus on in detail. \ebcomment{ugh this doesn't really feel relevant: it's not a result of data collection bias}. 

Wan~\cite{wan2022fairness} presents an interesting case study of how data representation can affect bias in NLP translation models, and an interesting mitigation technique. They show that differences in translation performance between different languages may not have to do with the structure of language itself, but instead with the granularity of the representation of the language: for example, word length (longer words lead to lower performance), and how many bytes it takes to represent characters in a word. This performance disparity can be mitigated by using more granular representations of language pieces to equalize representation length across languages (e.g. subwords, different representations for characters). They also call for the creation of a new character encoding system that  encodes characters outside the English alphabet more efficiently than current methods to further mitigate bias stemming from representation length. 

Despite the capacity for feature engineering and imputation choices to affect model fairness, our survey failed to identify any tools that assist practitioners in mapping out the effects of their prepossessing choices from the perspective of preventing bias and suggesting mitigations. However, there may be some potential for adapting tools that have been developed for more general data exploration and preprocessing to incorporate fairness contributions as well. For instance, Breck et al.~\cite{breck2019data} describe a data validation pipeline for ML used at Google that proactively searches for data problems such as outliers and inconsistencies; and there are several data-cleaning tools which even suggest transformations according to best practices~\cite{hynes2017data, krishnan2016activeclean}. Further exploring the landscape of these more general tools and their potential applicability to questions of model fairness seems to be a fruitful avenue for future work. Crucially, however, we note that we are unaware of any such systems that presently account for bias-related desiderata.

%\paragraph{Preprocessing Opacity} 
% Koesten et al~\cite{koesten2019collaborative} point to sources of failure in collaborative data use, such as passing data sets between research groups or collaboratively creating data sets---for example, one failure mode they point to is having an incomplete understanding of data cleaning steps that took place before working on a dataset created by another group. They point to user needs of such collaborative data pipelines, such as open channels of communication and version control, but do not create tools to operationalize these needs. 

% There are other mitigation techniques for some of the problems that result from collection: for example, Wrangler~\cite{kandel2011wrangler} provides a method of logging data cleaning steps for review, documentation, and reproducability; Breck et al.~\cite{breck2019data} introduce a data validation pipeline for ML used at Google; and there are several data-cleaning tools which even suggest transformations according to best practices~\cite{hynes2017data, krishnan2016activeclean}. We acknowledge that this literature review does not go deep enough into these other areas. We leave this for fruitful areas of future work. Crucially, however, we note that these systems do not take explicitly take bias-related desiderata into account.

\paragraph{Feature Selection}
Despite some evidence suggesting the choice of features used for inference also impacts model fairness behavior, a number of important open questions remain in this area as well. A fair amount of work has considered the impact of spurious correlations at the intersection of fairness and robustness: many papers that argue about the danger of spuriously correlated features, especially from the perspective of fairness in its relation to causality, and propose methods to remove them~\cite{wang2020towards}, however, Khani et al~\cite{khani2021removing} show that removing spurious features can often increase accuracy disparity across demographic groups. 
There has also been research into how input features influence selection disparity~\cite{emelianov2022fair,bartik2016deleting,garg2020dropping} in a model. For example, Emelianov et al.~\cite{emelianov2022fair} show that that group-wise differences in variance over a model's feature set influence selection disparity, and show under what conditions groups with higher and lower feature variance will be under or over selected. 

%Evidence from the recent monitorship of Upstart, a finance firm which, which involved an in-depth investigation of their model in the search for less discriminatory alternatives, suggests that which features are used for prediction have a statistically significant impact on prediction disparities. 

\krdelete{\paragraph{Methods and Tools for Feature Selection}
Certainly, from a legal perspective, using race or other protected attributes in a model often leads to a violation of disparate treatment~\cite{}. }\krcomment{Disparate treatment is only relevant in certain contexts and even so I personally think leans too much into a misplaced notion of fairness along the lines of anti-classification ideas, but rather than getting into that debate here, maybe just omit the sentence?} While removing race from the model--as a feature and via proxies--may not be an effective method to achieve fairness~\cite{lipton2018does} \krcomment{probably cite our methods comparisons paper here as well?}, in situations where it is useful, Yeom et al.~\cite{yeom2018hunting} provide methods for searching for and removing discriminatory proxies in regression models, and 
%Robertson et al.~\cite{robertson2022bio} provide a method for searching for which features may be producing bias, by showing how features--and importantly, their interactions---can lead to latent encodings of protected attributes. 
Frye et al~\cite{frye2020asymmetric} introduce Asymmetric Shapley Values, a technique which can be used on a wider range of models to determine whether a feature is allowing a protected attribute to causally influence the model outcome, so that the feature can then be pruned. 
Additionally, the FlipTest technique~\cite{fliptest} also produces suggestions of which features may be the source of disparate outcomes across any two populations the user may wish to compare, without attention to causality---this may be especially helpful in narrowing down the list of features to further investigate for impacts on differences in selection rate, or simply to find statistical, and not causal, discrimination.  Finally, Belitz et al.~\cite{belitz2021automating} provide an automatic feature selection framework which only selects features which improve accuracy without reducing a user-specified notion of fairness. However, this method saw considerable drops in accuracy when selecting features in this manner. 

While there is promising work outlining how various aspects of model inputs---such as their variance and causal relationship to protected attributes---influence various notions of model fairness behavior, again there is a lack of testing these results and techniques on on-the-ground pipelines, over a variety of datasets, and also searching for feature selection impacts on a wider set of fairness-related model behavior desiderata.
%there is a large gap between the research completed and a set of ready-to-use tools which can inform model practitioners on how feature selection choices influence model behavior. 
\ebcomment{Some better concluding statement here}.

% \begin{mdframed}
% Tools: Automated Data Validation \textasciitilde ~\cite{breck2019data} $\cdot$ Searching Features for Proxies/Bias \textasciitilde ~\cite{yeom2018hunting,frye2020asymmetric,fliptest}
% $\cdot$ Feature pruning for lowered bias amplification \textasciitilde ~\cite{leino2019feature} $\cdot$ 
% Automatic Feature Selection to improve traditional fairness techniques \textasciitilde ~\cite{belitz2021automating} 
% \end{mdframed}

\paragraph{Key Takeaways:}
\begin{itemize}
    \item Little work has been done exploring the impact of feature engineering and missing value imputation on model fairness, let alone operationalizing tools to help practitioners probe the impact of these decisions in their systems.
    \item Existing tools for data exploration and feature engineering do not account for fairness-related desiderata of downstream systems.
    \item A number of tools have been developed to consider the impact of feature selection on model fairness, but with little empirical testing in real-world contexts and some evidence of limited performance.
\end{itemize}

\subsection{Statistical Modeling}

\paragraph{Hypothesis Class Selection}
There is increasing work pointing out the fairness impacts of using models with increased variance~\cite{blackleave2021}, especially deep models---for example, these models can be more unstable to small perturbations in training setup~\cite{blackleave2021} leading to procedural fairness concerns about the nature of the decision process. 

\paragraph{Optimization Function Selection}
A growing number of works have pointed to degredations of fairness behavior in robust models~\cite{} and differentially private models~\cite{bagdasaryan2019differential, suriyakumar2021chasing}. 
Of course, there is also a vast body of work creating optimization functions to train models satisfy conventional fairness metrics, which we do not discuss in depth~\cite{}. 

Symmetrically, there has also been a fair amount of criticism for conventional group and individual fairness metrics imposed as top-down constraints on a system~\cite{akpinar2022sandbox,suresh2021framework}, and evidence showing that enforcing such constraints can actually degrade fairness according to those same metrics~\cite{}.
\krcomment{Could maybe also point to our tradeoffs paper, the comparison paper, and Emily's vertical equity paper as some examples of where these tools aren't well-suited to real-world use cases, such as where the decision boundary in real life is far away from the decision boundary these models tend to optimize fairness around under the hood?}

However, there is little work investigating the differences in model behavior without additional constraints, simply from changing the optimization functions used---such as Adam versus SGD in deep models, or lbfgs versus SAGA in Logistic Regression. There is preliminary evidence to suggest that differences in optimization functions do lead to differences in fairness behavior: Leino et al~\cite{leino2019feature} show that SGD over-emphasizes high-variance features, especially early on in training, which can lead to increased bias amplification. Investigating how other optimization biases impact fairness behavior may be interesting grounds for future work. 

\paragraph{Hyperparameter Search} Perrone et al~\cite{perrone2021fair} and Islam et al~\cite{islam2021can} show the promise of hyperparameter tuning towards finding fairer classification models. Islam et al~\cite{islam2021can} focus on showing that hyperparameter tuning can lead to increased fairness (differential fairness~\cite{foulds2020intersectional} and demographic parity) at no cost to accuracy. Perrone et al~\cite{perrone2021fair} introduce a technique, Fair Baysian Optimization (FBO), which is model and fairness-definition agnostic, to select hyperparameters which optimize accuracy subject to the fairness constraint. They also experimentally demonstrate that regularization parameters are the most influential for fairness performance, and that higher regularization leads to higher fairness performance in their experiments. We hope that this technique can used to understand further relationships between hyperparameter changes and fairness behaviors over a variety of different models, metrics, and deployment scenarios.

% \krcomment{How are we handling the tools here? Just include a review of all the in-processing methods?}
% \begin{mdframed}
% Tools: ~\cite{perrone2021fair} 
% \end{mdframed}

\paragraph{Key Takeaways:}
\begin{itemize}
    \item Accounting for fairness considerations in the modeling process itself is the most mature area of the FairML literature.
    \item Nevertheless, methods that have been proposed to date are generally built in the abstract and rely on assumptions that fail to translate well to real-world settings.
    \item The proliferation of these methods also pose a challenge for practitioners to navigate the many options and determine which (if any) should be considered in their setting (which may carry appreciable costs when code is either not available or only ``research'' code is available).
\end{itemize}

\subsection{Testing and Validation}

\paragraph{Validation Datasets} Several papers have discussed the perils of evaluating systems on the same benchmark data sets: this can lead to overfitting to specific data sets~\cite{deb_raji} that almost guarantees distribution shift to deployment domains, meaning that results are unrepresentative for many real-world fairness applications~\cite{sambasivan2021everyone}, and suggests that several experimental results in the fairness literature---including those related to pipeline interventions---may be incorrect~\cite{ding2021retiring,li2022data}. Other papers still have drawn attention to specific distributional problems within commonly used fairness benchmarking datasets, such as an under-represetnation of older individuals~\cite{park2021understanding}. 

%Ding et al~\cite{ding2021retiring} introduce a new suite of datasets, based on census data (a superset of the Adult dataset) for benchmarking FairML approaches. Based on this new data, they demonstrate that the effects of fairness interventions vary wildly with geography, and that common truths accepted in the community---such as increasing data size should reduce prediction disparities---do not always hold. While this is a good step, it's important for there to be large, diverse datasets in several domains (healthcare, consumer credit, insurance, education, among others), and beyond this even, to prioritize evaluating fairness approaches \emph{in the systems where where they will actually be used}. 

\paragraph{Model Selection Criteria} 
D'Amour et al.~\cite{d2020underspecification} bring attention to the problem of underspecification, where a model developer insufficiently specifies desirable deployment behavior, leading to biases and other problems during deployment. They argue that most of the model selection metrics currently used in practice---accuracy, robust accuracy, or other metrics--- on a test set insufficiently specifies desirable deployment behavior, and they demonstrate this problem in the context of several models with equivalent accuracies and robust accuracies on a test set having vastly different performance on naturally occurring 
out of distribution samples which the models came across in  deployment.
Black et al.~\cite{black2022model} describe a related phenomenon, model multiplicity, which is when there exist multiple equivalently accurate models for a given prediction task. They argue that there are multiple equally accurate models for almost all real-world prediction tasks, and show how this fact can be be leveraged to push practitioners to search for the least discriminatory model from those available with equivalent accuracy by leveraging legal pressure from the disparate impact doctrine. However, \emph{if model multiplicity is not explicitly harnessed}, it means that model evaluated on the basis of accuracy alone, the current default in machine learning, are almost certainly sub-optimally fair models even when constrained to only consider models with equivalent predictive performance.

\krcomment{Seems like the various fairness audit tools -- AI Fair 360, aequitas, etc fit in here somewhere?}

\paragraph{Key Takeaways:}
\begin{itemize}
    \item A growing body of work has illustrated how choices of validation data and model selection strategies can affect model fairness, however little of this work has been operationalized into tools or methods that can assist ML practitioners in navigating these choices.
\end{itemize}


\subsection{Deployment and Integration}

\paragraph{Accounting for Distribution Shift} A series of recent papers have introduced methods to make models invariant to distribution shift from the perspective of accuracy as well as fairness~\cite{singh2021fairness,coston2019fair,biswas2021ensuring}. Coston et al.~\cite{coston2019fair} develop two methods, one that does not require protected attributes in the training set, and one that does not require protected attributes in the deployment set. 
However, practical evaluations of these methods in deployed systems is still needed to characterize their real-world performance. Additionally, there are several open questions in this area of research: when do we want to ensure fairness criteria over data-drift, and when do we want to alert that the model practitioner that the distributional differences are so large that the model is not suitable for the deployment context?
Are there formulations of data drift were performance can be maintained through updates, but fairness cannot? When these drifts do occur what are best steps for a pracitioner to take to mitigate their impact? How do these systems perform relative to slowly-drifting distributions versus abrupt discontinuitys (such as a global pandemic or significant change in policy or practice)?
\ebcomment{Need help with further questions.}

 
\paragraph{Monitoring}
\krcomment{Would it maybe make sense to merge distribution shifts and monitoring sections? Seems like they're closely related.}
Even when using methods with guarantees on being resistant to distribution shift \textit{in situ}, it is still important for systems to monitor their fairness behavior over time. Two recent papers~\cite{albarghouthi2019fairness,ghosh2022faircanary} propose tools for fairness monitoring over time in deployment. Albarghouthi and Vinitsky~\cite{albarghouthi2019fairness} develop a technique called fairness-aware programming (implemented in Python), which allows programmers to enforce probabilistic statements over the behaviors of their functions, and get notified for violations of those statements---their framework is flexible to many behavioral desiderata even beyond fairness, and can also combine several probabilistic statements and check them simultaneously. The flexibility of the system potentially allows for a wide range of contextualized fairness desiderata to be enforced-- however, it does have limitations; for example, it cannot implement notions of fairness over individual inputs such as individual fairness. %At run time, the system continuously monitors if there is a violation of any of the desired properties and notifies the developer if so. 
Ghosh et al~\cite{ghosh2022faircanary} implement a system that measure the Quantile Demographic Drift metric at run time, a notion of fairness that can shift between group and individual conceptions of fairness based on the granularity of the bins it calculates discrepancies over. Their system also offers automatic mitigation strategies (normalizing model outputs across demographic groups) and explanation techniques to understand mechanisms of bias. Additionally, Amazon's SageMaker Clarify framework allows for the tracking of a variety of traditional fairness metrics to be monitored at runtime~\cite{}. 

However, to the author's knowledge, there is no work that address what fairness problems may come \emph{as a result} of this section of the pipeline: for example, are there examples of model updates from non-fairness aware monitoring pipelines that have degraded fairness performance? \krcomment{Fair point, but maybe a little too nuanced?}
%\ebcomment{What's the punchline here? some ideas: we need to test these on real systems, it's important to see failure modes--how intuitive are they for pracitioners to use, and how flexible *are* they for contextualized notions of fairness? Any other questions we have about the pipeline stage?}

\paragraph{Human-Computer Hand off}
Many algorithmic systems have been built with the ability to defer certain predictions to a human in the case of uncertainty~\cite{black2021selective}, assuming that including humans in decision-making systems will make them less biased. However, there are conflicting results as to whether human-in-the-loop systems out-preform models on their own when it comes to bias. Green and Chen~\cite{green2019principles,green2019disparate} show that including Mechanical Turk workers to aid algorithmic decisions consistently decreased accuracy relative to the algorithm's performance alone, and that humans in the loop also exhibited racial bias when interacting with ML predictions. However, others~\cite{cheng2022child, de2020case} have found that in the case of child welfare screenings, allowing call screen workers \emph{did} reduce disparity in the screen in rates of Black versus white children. 
Symmetrically, Jacobs et al.~\cite{jacobs2021machine} show that including machine learning recommendations in selecting antidepressants for patients did not improve clinician's treatment decision performance, and in fact, interacting with incorrect recommendations---even when supplied with explanations---lead to decreased performance. 

Taken together, as many have noted, these results show that ML decision systems which include human intervention must be tested for accuracy and bias as a whole rather than on algorithm outputs alone. These results also suggest that the efficacy of human intervention is very context-dependent. However, there little progress on how to infer when handoff problems will occur, or how to mitigate these inefficiencies. 
\marginpar{can someone add some papers that show that explanations don't really help either?} 

There has been a stream of theoretical work from the algorithmic fairness literature trying to model or guarantee fairness in a joint human-ML system~\cite{keswani2021towards,madras2018predict}. For example, Keswani et al~\cite{keswani2021towards} learn a classifier and a deferral system for low-confidence outputs, with the deferral system taking into account the biases of the humans in the loop. Donahue et al.\cite{donahue2022human} develop a theoretical framework for understanding when and when not human and machine error will complement each other, i.e. when human and machine error will occur in different areas of the distribution and cancel each other out, leading to increased performance, and suggest how this can inform the design of human-in-the-loop systems. While this initial largely theoretical work is promising, these techniques should be tested and compared on deployed systems---when do deferral systems work in practice, and can they lead to biases of their own? Do the human-in-the-loop design suggestions work in practice?



%\marginpar{Do we need to look at CHI for this?}
%Little attention has been paid to organizational integration in the fairness literature surveyed. 
%There has been some work showing that humans and machines working together can often compound errors rather than prevent them~\cite{I think some ben green stuff, maybe something from jen and hannah wallach}, but little progress on how to infer when handoff problems will occur, or how to mitigate these inefficiencies. 


\paragraph{Organizational Biases}
Organizational biases can enter an ML decision system through other means than deferring to a human in the loop. While there is evidence of the fact that organizational biases influence algorithm conception and the pipeline wholistically e.g.~\cite{passi2020making} from interview-based studies, there are is little documentation of examples of when and how this occurs and how it specifically influences predictions. Lum et al.~\cite{lum2020impact} document one such example, showing that inputs to risk assessment models, specifically, the charges that a defendant it booked for, are often over-exaggerated for Black defendants, and thus incur bias against Black defendants in model usage. (Presumably, this would happen even if the underlying model is ``fair''). \krcomment{Lum here actually seems like it might fit into the discussion of data or label biases above? What seems distinct here might be more along the lines of biases in intervention effectiveness or implementation, such as conducting outreach calls only in English or providing after school programs that can't be utilized by students that need to work or care for siblings after school, etc. However, most of these issues won't really show up in the ML literature we surveyed (more likely in the policy literature), so perhaps it would make more sense  to add a sentence or two about these broader organizational questions under the human-computer handoff heading rather than having a separate sub-section here?}

Overall, organizational integration especially lacks in \emph{measurement and mitigation} of fairness problems arising from this section of the pipeline. In addition, the literature on human-computer interaction and organizational biases do not come near understanding all of the (fairness-related) failure modes of organizational integration. For example, is just one ML system used in the decision system? Some systems in government, for example, use multiple models to inform decisions~\cite{blackIRS2022}. In these situations, how are these predictions combined, and are the models built to be used in unison? What are the impacts of rule-based decision frameworks imposed on top of algorithms predictions, such as those use in pretrial risk assessment tools\~cite{}? 

\ebcomment{It would be great to have some help pointing out what is missing here---mapping organizational frameworks, other ways of model integration into a larger decison-making framework can lead to problems.}

\paragraph{Key Takeaways:}
\begin{itemize}
    \item Recent developments in methods robust to distribution shifts seems promising but need more testing in applied settings and several questions remain for both research and practice.
    \item Monitoring and maintenance of a deployed system is just as important meeting fairness desiderata in the initial development. A growing number of monitoring tools can facilitate this process for practitioners and users of these systems.
    \item Particularly in high-stakes settings, many ML models are being used to inform human decision-making rather than acting autonomously. In these settings, it is critical to understand not only the fairness properties of the model, but those of the entire human-ML system acting together.
    \item The deployment context and specific decisions being informed by a given model also matter deeply in terms of how a model's fairness properties---as narrowly defined with respect to metrics relating to its predictions---will relate to the actual impact on people affected by the model's outputs.
\end{itemize}

\subsection{Documentation}
Several works have pointed to the need for documentation in machine learning pipelines~\cite{gebru2018datasheets, koesten2019collaborative, black2022model}. For example, Koesten et al~\cite{koesten2019collaborative} point to lack of documentation as a source of failure in collaborative data use, such as passing data sets between research groups or collaboratively creating data sets---for example, incomplete documentation may lead to a misunderstanding of data cleaning steps that took place. 
Checklists for how to document machine learning systems abound~\cite{}, but automated tools for documentation would severely decrease the load on practitioners.  While such tools are few and far between in the fairness literature, they exist in other spaces: for example, Wrangler~\cite{kandel2011wrangler} provides a method of logging data cleaning steps for review, documentation, and reproducability. However, there is a need to find such tools and convert them to include model fairness specific functionality.

\krcomment{I see why you split this out here, but it also doesn't really feel like it fits as a distinct pipeline step. Perhaps we could make it a separate sub-heading under Deployment and Integration instead? Also seems like some of the model cards stuff would fit here:

\url{https://dl.acm.org/doi/pdf/10.1145/3287560.3287596?casa_token=DyLeBck72WgAAAAA:E3xvjZ4p5tM629YLYCQqq3HVB29HCQMaC_7Ua41FxXbAFOnCqn1nfvsAfRtUWVKp2pYWghkjMV7IGzo}

\url{https://dl.acm.org/doi/pdf/10.1145/3531146.3533108?casa_token=Dv5l8KuMpbQAAAAA:IAXd1Z1dM1vDuzRxzn1XPkOIEEJz3v0pWcniqMfz8g693eApvA7Vlc7wmQYgC2E2SrAaA6vWxbrkWgk}
}

\paragraph{Key Takeaways:}
\begin{itemize}
    \item Several papers have called for better documentation of models and datasets, both for research and practice, and various proposals have been made for more standardized formats. However, these efforts would be assisted by adapting some of the tools and automation that exist in other spaces to lower the barriers to developing good documentation in the ML space.
\end{itemize}
 
 %Koesten et al~\cite{koesten2019collaborative} point to sources of failure in collaborative data use, such as passing data sets between research groups or collaboratively creating data sets---for example, one failure mode they point to is having an incomplete understanding of data cleaning steps that took place before working on a dataset created by another group. They point to user needs of such collaborative data pipelines, such as open channels of communication and version control, but do not create tools to operationalize these needs. 


\subsection{Consideration of the total pipeline}
%One notable recent work by Donahue et al.\cite{donahue2022human} develops a theoretical framework for understanding when and when not human and machine error will complement each other, i.e. 

\ebcomment{Help finding works and tools that consider the entire pipeline at once?}

\krcomment{I don't think there's really a lot out there---certainly this is the gap that the sandbox toolkit is seeking to fill in part. Likewise, our method comparison paper looked at pre-, post-, and in-processing methods separately, but didn't attempt to consider their interactive effects. I'd probably suggest removing the heading here and commenting on the need for more research in this direction as a major element of the research agenda (while noting that operationalization of the different components would also make this a lot more tractable)}



\input{survey_table.tex}
%\input{survey_table_simple.tex}


==> versions/survey.tex <==
\section{A Survey of Pipeline-Fairness}
\label{sec:litreview}

\ebedit{As a first step towards operationalizing the pipeline-based approach to fairness in ML, we provide a review of the ML fairness literature focused on creating a taxonomy of fairness work that locates, measures, or mitigates problems along the ML pipeline. In addition to serving as a first step towards a resource that ML practitioners can use to identify ways to diagnose and mitigate problems in their pipeline, our survey of the work already done allows us to point to the gaps in the literature that must be addressed in order to have a full understanding of how choices made along the ML pipeline translate to model behavior-- and then build tools which operationalize this understanding to build more effective systems.}

%We focus on work that does not fall into the category of adding an optimization constraint to a model in order to enforce a fairness metric, or resampling data, in order to highlight how 


\subsection{Survey Methods and Organization.}

\hhcomment{I think we can justify our focus on ML venues by saying that we were interested in measures and remedies that could be useful to ML practitioners; hence the focus on these venues.}

In order to better understand the current landscape of algorithmic fairness research throughout the ML pipeline, we performed a thorough survey of the recent \krdelete{algorithmic fairness }literature, which we classified depending upon which area of the pipeline they analyze. We gathered papers from NEURIPS, ICML, ICLR, FAccT, and AIES, for the past five years, i.e. 2018-2022, that contain any of the following terms in their title, abstract, or keywords: "fairness", "fair", "discrimination", "disparity", "equity".\footnote{When available: this is with the exception of NEURIPS, which we gather for years 2017-2021 due to the date of the conference relative to the time writing this work, and EAAMO, which started in 2021.} In addition, we performed a series of Google Scholar searches to ensure our survey did not miss high-impact work published in other venues: One search used the keywords listed above and included papers published in any venue in the past five years with over 50 citations, through the top 50 results returned by this Google Scholar search. \krdelete{This is to ensure that we do not miss any high-impact work from other venues. Finally, we perform} Additional Google Scholar searches used keywords from each step in the pipeline individually, to attempt to find papers targeted at each stage: for example, "data collection" and "fairness" and "machine learning". This results in \textcolor{orange}{\textasciitilde1000} papers overall. 

We then manually inspect each paper to understand whether and how the reported research is an instance of a pipeline\hhedit{-aware} approach to fairness. That is, does it identify, measure, or mitigate a concrete cause of unfairness due to choices made in a specific stage of the ML pipeline. If so, we categorize the paper along two axes: what part of the pipeline it corresponds to (problem formulation, data choice, feature engineering, statistical modeling, testing and validation, or organizational realities), and whether it identifies, measures, or mitigates a pipeline fairness problem. 

\rgdelete{While we acknowledge that adding optimization or loss constraints to a model to enforce a given definition of fairness is in itself a modeling choice and thus fits in to the ``pipeline'' notion of fairness \hhedit{(specifically, under the statistical modeling, choice of the objective function)}, we separate these more traditional fairness papers from our understanding of pipeline-based fairness papers for the sake of this survey by giving them their own category, which we call ``Algorithm''. }\krcomment{Not too sure I see the necessity of calling out this distinction separately -- aren't we just saying the choice of algorithm is one component of the pipeline? Especially given the length, maybe just cut?}
\rgcomment{i agree with Kit - deleted that for now in the text}


\subsection{High-Level Overview and Takeaways}
\begin{itemize}
    \item Our first observation is that the number of fairness papers that adopt a pipeline perspective to fairness is far outnumbered by the more traditional, abstracted approach to fairness: XXX papers versus XXX papers overall. \hhcomment{Might be nice to do a histogram, showing numbers per pipeline stage.}
    \item The algorithmic fairness literature has a dearth of knowledge about what on-the-ground pipelines look like: although there are many papers that outline abstracted pipelines (including our own), the actual model creation steps taken by practitioners for a variety of real-world systems (e.g. in consumer finance, healthcare, hiring systems) are at the very least not cataloged in any centralized place. 
    \hhcomment{The point being made here is not clear to me.}
    \item Even within the list of papers that do take a pipeline-based approach, the majority of them are \emph{proof-of-concept}: there is much work to be done to take the solution proposed in the work into an implementable and generalizable fix for pipeline problems.
    \item Most fairness-related papers focus on \emph{one issue} in the pipeline, but fail to provide insight into how these different aspects of the pipeline interact. Does solving each issue in isolation work?
    \item Within those papers, the majority investigate problems with data collection and pre-processing as an arbitrary approach to ``fixing'' fairness.
    \item Many of the pipeline papers still engage with one particular notion of fairness (often demographic disparity). It would be helpful to create a more generalized mapping of how modeling choices change prediction behavior, beyond a single metric.
    \item There is a dearth of case studies of bias mitigation in the fairness literature. Though case studies may often be disregarded as ``simply implementing old methods'' and thus not novel, it is crucial that we give them more attention so that we can learn about the failure modes of the techniques that we create. While there are \hhedit{notable} papers about the overall problems of production teams, e.g. ~\cite{madaio2020co,holstein2019improving,sambasivan2021everyone}, these still do not provide in depth-detail of the bias mitigation process in deployed systems. 
\end{itemize}



\subsection{Viability Assessments}
To the author's knowledge, there is very little work within the fairness literature on documenting, or detailing the bias that can arise out of, or mitigating bias from the viability assessment process

\rgdelete{: how we investigate the benefits and downsides of the current decision-making system in place in comparison to what an ML-based solution could provide, and assessing organizational capacity for effective system \hhedit{evaluation, design, and deployment. Important considerations in this category include (but are not limited to) access to high-quality data, sufficient ML expertise, capacity for continued monitoring.}}

Viability assessments provide an avenue for refusal to build an ML system, which is understudied in the fairness literature\hhedit{~\citep{raji2022fallacy}}. Though there have been discussions in the community around when to refuse to build~\cite{barocas2020not}, there is little published work on case studies detailing how the decision to build or not build was made. --- et al~\cite{find_that_paper} point to the fact that ML researchers and practitioners do not often consider the option to not build a system because it is taken as the default, given the pressures (and funding) coming from the tech industry. Indeed, many works that point to how organizational factors---such as lack of a company's support for ethical AI approaches, or time pressure, or focusing only on client demands~\cite{passi2020making} can lead to pushing ML systems ahead without careful consideration of whether or not deploying a system in that domain is a net benefit in the given context. One resource, Data Science for Social Good Scoping Guide \cite{DataScienceScoping} highlights some of these issues  and gives practitioners some questions to ask at the viability assessment stage of a project.
\krcomment{Not published in an academic venue, but perhaps we should point to the DSaPP Scoping Guide here, as well as specific fairness/inclusion issues it details? http://www.datasciencepublicpolicy.org/our-work/tools-guides/data-science-project-scoping-guide/}

\paragraph{Key Takeaways:}
\begin{itemize}
    \item Work around the fairness implications of viability assessments for ML systems is almost entirely lacking in the FairML literature, leaving appreciable open questions around decisions of whether or not to build a system, stakeholder engagement, and identification of overall goals of a project.
\end{itemize}


\subsection{Problem Formulation}
Problem formulation encapsulates the decisions made when translating a nebulous policy or business goal into an ML task and often consists of various decisions made: e.g. deciding who is in the cohort that the ML system will be used on, translating ``predicting creditworthiness'' into ``predicting loan default''~\cite{passi2019problem}. 

Problem formulation is also a time to assess whether a proposed ML system will address the actual needs of the organization to which it will be deployed. 
While not describing this process as problem formulation per se, Katell et al. detail how their design ideas changed over time through their engagement with community stakeholders while building an Algorithmic Equity Toolkit to aid activists in participating in public comment session when evaluating ML systems to be used by the Seattle city government~\cite{katell2020toward}; and Suresh et al~\cite{suresh2022towards} detail how they co-designed a tool for collecting news articles documenting cases of femicide. Creators of ML for Public Policy Lab class at CMU \cite{MLPolicyclass} highlight several decisions that need to be made in the problem formulation stage of the pipeline.

\paragraph{Selection of Prediction Target} 
While there is helpful discussion on how prediction target selection may lead to bias, often drawing from the social science literature of validity theory~\cite{passi2019problem,jacobs2021measurement,coston2022validity},
as well as examples of disparities stemming from prediction target selection selection~\cite{black2022algorithmic,obermeyer2019dissecting,human_rights_watch_2020}, to the author's knowledge, there is little work in the ML fairness literature detailing the process of problem formulation in practice, or leveraging fair ML tools to measure or mitigate the potential bias of the selection of a given prediction target ex-ante. 
Developing protocols for assessing problems of various notions of validity (internal, external, content, predictive) of the target variable and predictive attributes is a promising and necessary avenue of future work. There is preliminary work along this axis in the form of checklists and protocols, e.g.~\cite{coston2022validity}, but we suggest it may be possible to make a suite of quantitative tests as well.
For example, access to appropriate data, ML practitioners could leverage existing model-level bias-testing frameworks~\cite{AIF360,saleiro2018aequitas} to test for bias across a series of potential prediction tasks to inform the decision of which to choose. Tests for predictive validity simply require investigating whether the proposed target variable is predictive of other related outcomes. Obermeyer et al.~\cite{obermeyer2019dissecting} used such a test to uncover the racial bias behind using health care cost as a proxy for health care need, by regressing health care cost on other metrics of illness (e.g. the number of active chronic conditions a patient has), finding that there was a disparity in the correlation between health care costs and sickness in white patients versus that in Black patients. Investigating the extent to which questions of construct validity and reliability can be operationalized into a set of tests (e.g., testing correlations between potential prediction tasks, or checking for consistent model performance across two different methods of measuring the output) may be a promising area for utilizing tools and methods from social sciences.

\paragraph{Selection of Prediction Universe}
\krcomment{The choice of cohort/universe for analysis and when to make a prediction actually seems pretty salient in terms of formulation as well. Here I'm talking about things like up-front decisions about who to make predictions on: Suicide risk among everyone in the population or just people with some history of mental health needs? Do I predict the likelihood of not graduating high school as of 2nd grade, 9th grade, 11th grade, etc? I'm certainly not aware of anything in the literature that actually looks at this (either systematically or via case study). Did you identify anything there?}\hhcomment{This is a very good point, and it reminds me of a related but distinct set of recommendations around 'studying up'~\citep{barabas2020studying}.}

\paragraph{Selection of Predictive Attributes}
\ebcomment{Help.} \hhedit{The discussions of validity and reliability outlined in the previous paragraph are just as well applicable to the features utilized for prediction. Many such features may aim to reflect social constructs such as race or gender~\citep{}. Additionally, Prior work has observed that trained models may rely on spurious correlations, that renders their predictions unreliable in presence of confounders and slight changes to the data distribution. We believe that close deliberation with domain experts would allow for the appropriate selection of features.} \hhcomment{We can mention the DoWhy package as a tool here.} \krcomment{To avoid confusion, I might actually integrate this into the data acquisition or feature selection/engineering discussion -- I feel like in practice it's generally difficult to get to the detail of choosing specific predictors this early in the process}

\paragraph{Determining Behavioral Desiderata}
\hhcomment{I think the following paragraph should be moved to "testing and validation" section. The details of the examples you mention can be moved to an appendix. Citation to these pieces suffice.} \krcomment{I'm a little on the fence there -- generally I think it's important for some of this goal/fairness metric definition to happen up front, but it's hard to avoid some repetition. I guess in the interest of space, consolidating with testing and validation might be cleanest?}
While we leave the question of finding an appropriate fairness metric to other work and focus instead on bias mitigation techniques, we wish to highlight the importance of finding \emph{contextualized} notions of bias and fairness to encourage in a system. For example, Black et al.~\cite{black2022algorithmic} show how \emph{vertical equity}, the public finance notion that individuals with different incomes and wealth must be treated differently in order to achieve fairness overall, is not achieved by enforcing traditional fairness metrics--- instead, the authors favor audit selection models with more monotonic audit selection distributions, which also display high selection overlap with an oracle model which selects individuals in order of highest tax misreport (i.e. most money not reported to the Internal Revenue Service). Mattei et al.~\cite{mattei2018fairness} consider the unique fairness requirements of organ-matching systems, noting that it was important for younger organs to be matched to younger recipients, and also to ensure that individuals did not receive different probabilities of getting an organ due to their blood type. Other examples of contextualized fairness desiderata include [CITE HERE]. \ebcomment{This is not the best example because it's a matching system instead of an ML system-- does anyone else have a more contextualized notion of fairness in a prediction system example?}
%we briefly note that a pipeline fairness approach can also naturally lead to a more in-depth, contextualized understanding of the ML system, making it more natural to define more context-specific model behavior desiderata than the most common fairness metrics. 
%Case studies of fairness problems in real-world deployed systems are especially helpful in understanding what 

\paragraph{Key Takeaways:}
\begin{itemize}
    \item Although some work does exist on the importance of label choice to system fairness, including compelling case studies, little is available to practitioners in terms of operationalized tools to help inform this choice.
    \item Despite the significance of the choices surrounding the definition of the prediction universe for defining who might have an opportunity to receive a benefit, we were unable to find any work in the literature exploring the downstream fairness implications of these choices.
    \item \krcomment{Probably move predictors / desiderata to sections below?}
\end{itemize}

\subsection{Data Collection}
Far and away, besides enforcing fairness constraints on models during training or prediction, the aspect of the pipeline that has received the most attention is data collection.  

\paragraph{Mapping effects of faulty data collection to model behavior} Several papers in the algorithmic fairness literature have pointed to the problems of disparate performance and selection across demographic groups stemming from datasets which are unbalanced across demographic groups, i.e. have sampling bias, both in terms of sheer representation, and representation conditional on outcomes~\cite{buolamwini2018gender, mishler2019modeling}; or have data that is \hhedit{disparately noisy} or perturbed in some way~\cite{wang2021fair}. Li et al.~\cite{li2022data} do a particularly thorough job of testing how potential results of data collection problems---e.g. unrepresentative samples, insufficiently small data samples, differing group base rates\footnote{Which could be true or the result of measurement error}---influence machine learning model behavior from the perspective of accuracy and fairness. They test the influence of these sources of collection bias comparing performance across models  trained on subsamples of \krdelete{an enormous, novel,} a criminal justice dataset (1.5M rows). Interestingly, they find that increasing dataset size, or even reducing the disparity in base rates, does not always reduce disparities in selection, false positive, or false negative rates. Other recent work introducing new datasets for testing fairness interventions find similar results~\cite{ding2021retiring,akpinar2022sandbox}. These papers are an excellent start to mapping data bias issues in the pipeline and immediately brings to mind more questions---how do these sampling and measurement errors impact other fairness desiderata, how do they interact with other pipleline choices such as model selection, loss function selection, and hyperparameter tuning? 

\paragraph{Mitigating biased model behavior on biased data}Proposed techniques for mitigating the effects of unrepresentative data include a variety of synthetic data augmentation techniques~\cite{sharma2020data, van2021decaf, chawla2002smote}, data re-weighting techniques~\cite{kallus2018residual}, and specialized optimization functions for creating fair classifiers (according to traditional metrics) with unbalanced data~\cite{jiang2021towards, li2021autobalance}. Coston et al. introduce a model training approach that can mitigate the effects of the selective labels problem~\cite{coston2021characterizing}.


Some argue that using modeling techniques such as re-weighting or using special loss functions serve as a band-aid solution, and argue that data problems should be solved by intervening on the data. Liu et al.~\cite{liu2021can} show how to find which subgroup in the data is likely to have noisy labels, and then introduce a technique of inserting \emph{more} noise into the labels of other subgroups in order to increase fairness and generalization, and often accuracy as well. Chen et al.~\cite{chen2018my} introduce methods of estimating the value of adding additional training samples from the perspective of thus improving many fairness outcomes such as equalized accuracy---potentially allowing for practitioners to decide whether searching for extra training examples or features is worthwhile.  


Several methods are also available for creating fair classifiers with noisy, corrupted or perturbed data~\cite{liu2021can}. 
Wei et al~\cite{wei2021learning} provide an interesting counterpoint to the papers which discuss creating fair classifiers on noisy data: they point to the differences in model behavior when trained with artificially noised data (i.e., following some specific noise distribution, such as Gaussian), as opposed to noisy data that is mislabeled by human annotators: for example, they show that harmful model memorization is much more common on models trained with mistakes in human annotations, since the human annotators mislabel examples that are inherently more confusing and thus informative for the model (e.g. a hard-to-distinguish photo).
As a form of solution, they provide a new noised version of CIFAR-10 and CIFAR-100 with errors by human annotators to better study the problem of noisy data in practice. 
This paper points to the peril of training and evaluating models on ``sterile'' data: they point out that our intuitions about the effects of noisy data on model behavior may be flawed, underscoring the need to test for pipeline-based problems and solutions on pipelines data to be used during deployment.
\krcomment{Seems like we should discuss approaches that focus on resampling/balancing the training data here as well -- similar to the inconsistency above, in our method comparison work (https://arxiv.org/pdf/2105.06442.pdf), we found a lot of variability across datasets and parameters in the ability of resampling to have any impact on model fairness. Some of the references there are a bit older, but we could also point to them for others looking at resampling (see the "Resampling" heading on page 2)}



%Cai et al~\cite{} suggest to a method of selecting individuals to seek labels for in order to improve the system the most from an equity standpoint. 
%Sharma et al.~\cite{sharma2020data} introduce a method of data augmentation which guarantees improvements in reducing demointroduces data with perturbations to the demographic group (i.e., switching demographic group) while keeping other feature and labels constant, as well as keeping demographic group constant and flipping outcome labels, crucially, slowly in order of likelihood within the probability distribution--- creating a family of datasets

\paragraph{Sources of bias in the sampling and labeling process} While several of these papers do show how machine learning systems change their behavior as a result of different kinds of data noise or unrepresentativeness~\cite{wang2021fair}, they do not speak to the source of bias in the sampling or labeling process, and how to correct it at the source. The Human and Computer Interaction community has done a much more thorough job of considering what failure modes can occur in the data collection process itself, especially as a result of crowd sourcing data set labels with workers from platforms such as Mechanical Turk~\cite{sen2015turkers,hube2019understanding,miceli2020subjectivity}. For example, Diaz et al~\cite{diaz2022crowdworksheets} point to the fact that crowdworker identities influence how they answer labeling prompts~\cite{sen2015turkers} \krcomment{The references here are confusing -- how does the Sen 2015 reference relate to this sentence?}, and introduce CrowdWorkSheets, a worksheet to help guide practitioners through, and allow them to document, the process of creating a dataset with crowdsourced labels with crowdworker identity in mind, from specifying the question of what crowdworkers are to label, to accounting for demographic differences in crowdworkers, determining compensation, among other considerations. However, they do not test the use of their worksheet on production teams. 
An exemplary paper by Sambasivan et al.~\cite{sambasivan2021everyone} provides a wider set of examples of real-life sampling bias and labeling bias, and importantly, \emph{how they entered a real-world system}.  In one set of examples, ``physical world brittleness'' brought about several senses in which deployment data was distributionally different from training data, leading to failure modes, and often abandonment of the AI project: e.g. ``hardware drifts'', where hardware systems which were the source of medical imaging data were not updated over time, leading models to give inaccurate results; or ''human drifts'' where human behavior changed over time leaving models useless, such as models build to predict disease spread over the course of the Covid-19 pandemic.  Another large failure mode identified was a lack of ``cross-organizational documentation'', which lead ML practitioners to make assumptions about aspects of the data, such as timestamps, introducing severe noise into the training data. 

The above papers are a great source of general pointers to data collection problems ignored in the ML literature, but there is still a dearth of deep investigations into \emph{specific} data creation pipelines and the particular sources of bias that show up in those systems, as well as contextualized mitigation strategies. 
There are some exceptions: Marda and Narayan~\cite{marda2020data}, show sources of historical bias, sampling bias, measurement bias, and direct discrimination as well as arbitrariness in the collection of data for the creation of Delhi's predictive policing system: for example, for measurement bias, they explain how the techniques used to map Delhi were inconsistent over the development of the tool, since the police department's ArcGIS system license expired; that there were often no formal addresses for less wealthy parts of the city thus identifying call location was largely guesswork; and that women who made calls were less likely to know their address since they often largely stay inside and are less aware of their surroundings.

More generally, while this literature does an excellent job of illuminating failure modes that can be surfaced through engaging with practitioners---since many papers in this area are structured around interviews---they may elide more low-level technical sources of data collection problems, such as record linkage issues leading to non-IID data dropping. While they are extremely helpful in the important first step of identifying problems, they provide little direction for creating operationalizable solutions to these problems, or even sufficiently detailed information about each system studied to be able to understand the mapping between data collection problems and model behavior.\krdelete{

Operationalization of a pipeline-based approach to fairness necessitates harnessing both the outcomes- and solution- focused algorithmic fairness literature which ignores the sources of problems, and the problem identification prowess of the HCI, CSCW, and other literatures. 
}
One paper by Goel et al.~\cite{goel2019crowdsourcing} comes closer to operationalization of a solution for a specific problem in the data collection pipeline: differential accuracy of crowdworkers in labeling tasks. They introduce a technique for assigning Mechanical Turk workers to labeling tasks in order to decrease disparity in false positive and false negative labels. It requires a subsample of datapoints (gold tasks) where the researchers know the true label of the data to be labeled in order to estimate the group-wise accuracy of each labeler. However, crucially, they do not test their technique in their own labeling task, but use datasets already annotated with Mechanical Turk workers as well as synthetic data---such approaches must be tested within actual labeling processes. 

\krcomment{There's a lot here on crowdsourced labels -- I guess because it's an easy system where the researchers have control over the label generation process -- and I think we can shorten it down to a paragraph or so. Seems like we should also point to some of the more real-world instances of label and sampling biases: differential enforcement of drug laws and biases in traffic stops come to mind as some of the important examples there. Of course, much harder to address without fixing the world. Likewise, seems like some of the work around biases in facial recognition arising from lack of representation in training data fits in here as well. 

\url{https://drive.google.com/file/d/1B58Os2Hb2v__YQ8whdWRULY9mgxxsHoO/view}

@Rayid -- I'm having trouble finding the drug arrests paper I'm thinking of right away (I think it looked at Oakland vs Berkeley?) but you might know it off-hand?

http://proceedings.mlr.press/v81/buolamwini18a/buolamwini18a.pdf
}
 
\krdelete{As a whole, we first note that while there is some excellent work in this area, data collection pipelines---and pipelines in general--continue to be poorly mapped, and thus not all sources of bias or failure are even identified. Secondly, there is a disconnect between problem discovery and mitigation techniques. While it may be that checklists, questions, and datasheets are the best solution to some sources of errors and bias in the data collection pipeline, (and the pipeline overall), there may be some more objective tests that can be performed to test whether data is being sampled, labeled, and measured in a defensible way. Thirdly, the work of mapping pipelines, identifying potential sources of bias within the choices therein, testing to see under what circumstances biases arises, and creating and testing mitigation techniques, is work that, to the extent that is has been done, is spread across multiple disciplines: from machine learning to database management. We should search for, study, and adopt techniques from these areas in order to create a mapping of machine learning pipelines for bias prevention.  
Finally, and perhaps most importantly, \emph{proposed methods should be tested in a variety of real-world systems} to see where they fail and when they are helpful. }

\paragraph{Key Takeaways:}
\begin{itemize}
    \item While there is some excellent work in this area, data collection pipelines---and pipelines in general--continue to be poorly mapped, and thus not all sources of bias or failure have likely even been identified.
    \item There is a disconnect between problem discovery and mitigation techniques. Although checklists and datasheets may be a solution to some sources of data collection bias, there is a lack of more objective tests to ascertain whether data is being sampled, labeled, and measured in a defensible way.
    \item Empirical work the relationship between between dataset size as well as group and label balance has shown inconsistent results in terms of impacts on downstream disparities, highlighting the complexity of the problem and limitations of solving model fairness issues at the level of data alone.
    \item What work that has been done in this area is spread across multiple disciplines: from machine learning to human-computer interaction to database management. We should search for, study, and adopt techniques from these areas in order to create a mapping of machine learning pipelines for bias prevention.
    \item Most importantly, proposed methods should be tested in a variety of real-world systems to see where they fail and when they are helpful. \krcomment{maybe rephrase these last two more as gaps and move the calls to action to research agenda?}
\end{itemize}

\hhcomment{I think Datasheets is one paper that should definitely be discussed in this section. }

%posit that we must combine the literature of problem discovery from a variety of literatures and work towards potential mitigation tactics, crucially, tested in real-world systems. While this may not lead to generalizable results at first, another active area of research may be what aspects of prediction problems or pipelines lend themselves to certain types of solutions.

%Beyond these instructive examples, Sambasivan et al. also provide a helpful overview of available methods and attempts to prevent such problems from a variety of literatures, including human-computer interaction, and data management science, including methods of logging data cleaning steps~\cite{wrangler}, enforcing validity constraints on data~\cite{}, incentivising 


%, and given insights from Sambasivan et al.~\cite{sambasivan2021everyone}, it seems 
%points to the need to evaluate models on data with noise distributions , and the investigation of the fairness effects of real-world noisy data.

%The computer science literature is solution-focused, and often develops a technique to mitigate the problem identified---but often in the form of a generalized band-aid, not investigating the causes of the problem in the data. On the other hand, HCI and related literatures delve
%There have been very few papers which lay out the entire end-to-end process of 


%Both literatures suffer from focusing too much on painting a general picture---overarching themes of failure points in processes and generalized solution techniques. We also need a taxonomy of examples of specific problems that have occurred, and how they have been solved

%However, despite this literature being rich in documenting overall patterns of 

\subsection{Data Preprocessing}

While there are many papers in the fairness literature that discuss how to \emph{leverage} preprocessing for bias mitigation~\cite{Zhao2020Conditional,cheng2021fairfil,balunovic2022fair,zemel2013learning}, to the author's knowledge, there is little work detailing how preprocessing steps may \emph{introduce} bias. 

\paragraph{Feature Encoding and Missing Values} A body of work has explored how preprocessing steps---such as data representation (e.g. discretized or continuous numerical values) normalization techniques, and strategies for data dropping and imputation---can influence classification model behavior~\cite{alshdaifat2021effect,biswas2021fair,crone2006impact,zheng2003existence} in a model-dependant manner. These effects can often be significant: Crone et al~\cite{crone2006impact} state that that the performance differences between preprocessing steps often rivaled that of the differences between using different models (SVM versus NN). In the context of predicting purchase behavior online, Zheng et al.~\cite{zheng2003existence} state that different methods of encoding the unit of analysis (what consititutes a purchase session) lead to ``radically different conclusions'' from model behavior.
Given that preprocessing can drastically influence model prediction performance, it must influence fairness behaviors as well. However, there is little work in this area. Biswas et al.~\cite{biswas2021fair} perform an analysis of how different preprocessing steps can influence fairness behavior, and show, among other effects, that dropping rows of a dataset with missing values instead of imputing those rows can lead to sizable differences in fairness behavior due to the changes to the training distribution. While this paper is an excellent first step, it would be instructive to understand how a larger array of (potentially context-specific) preprocessing steps lead to changes in model behavior---for example, how exactly different features are defined, e.g. encoding attributes such as age in various datasets in continuous or binned. Other avenues for future work include investigating fairness impacts beyond the metrics discussed in the paper,  how these data preprocessing steps interact with the inductive biases of a larger variety of models, and developing methods for how to choose between preprocessing options given information about the data and the modeling pipeline.
%Another large area of focus is methods for ``debiasing'' data by making a representation of the training data which is independent of the protected attribute~\cite{Zhao2020Conditional,cheng2021fairfil,balunovic2022fair,zemel2013learning}, which we do not focus on in detail. \ebcomment{ugh this doesn't really feel relevant: it's not a result of data collection bias}. 

Wan~\cite{wan2022fairness} presents an interesting case study of how data representation can affect bias in NLP translation models, and an interesting mitigation technique. They show that differences in translation performance between different languages may not have to do with the structure of language itself, but instead with the granularity of the representation of the language: for example, word length (longer words lead to lower performance), and how many bytes it takes to represent characters in a word. This performance disparity can be mitigated by using more granular representations of language pieces to equalize representation length across languages (e.g. subwords, different representations for characters). They also call for the creation of a new character encoding system that  encodes characters outside the English alphabet more efficiently than current methods to further mitigate bias stemming from representation length. 

Despite the capacity for feature engineering and imputation choices to affect model fairness, our survey failed to identify any tools that assist practitioners in mapping out the effects of their prepossessing choices from the perspective of preventing bias and suggesting mitigations. However, there may be some potential for adapting tools that have been developed for more general data exploration and preprocessing to incorporate fairness contributions as well. For instance, Breck et al.~\cite{breck2019data} describe a data validation pipeline for ML used at Google that proactively searches for data problems such as outliers and inconsistencies; and there are several data-cleaning tools which even suggest transformations according to best practices~\cite{hynes2017data, krishnan2016activeclean}. Further exploring the landscape of these more general tools and their potential applicability to questions of model fairness seems to be a fruitful avenue for future work. Crucially, however, we note that we are unaware of any such systems that presently account for bias-related desiderata.

%\paragraph{Preprocessing Opacity} 
% Koesten et al~\cite{koesten2019collaborative} point to sources of failure in collaborative data use, such as passing data sets between research groups or collaboratively creating data sets---for example, one failure mode they point to is having an incomplete understanding of data cleaning steps that took place before working on a dataset created by another group. They point to user needs of such collaborative data pipelines, such as open channels of communication and version control, but do not create tools to operationalize these needs. 

% There are other mitigation techniques for some of the problems that result from collection: for example, Wrangler~\cite{kandel2011wrangler} provides a method of logging data cleaning steps for review, documentation, and reproducability; Breck et al.~\cite{breck2019data} introduce a data validation pipeline for ML used at Google; and there are several data-cleaning tools which even suggest transformations according to best practices~\cite{hynes2017data, krishnan2016activeclean}. We acknowledge that this literature review does not go deep enough into these other areas. We leave this for fruitful areas of future work. Crucially, however, we note that these systems do not take explicitly take bias-related desiderata into account.

\paragraph{Feature Selection}
Despite some evidence suggesting the choice of features used for inference also impacts model fairness behavior, a number of important open questions remain in this area as well. A fair amount of work has considered the impact of spurious correlations at the intersection of fairness and robustness: many papers that argue about the danger of spuriously correlated features, especially from the perspective of fairness in its relation to causality, and propose methods to remove them~\cite{wang2020towards}, however, Khani et al~\cite{khani2021removing} show that removing spurious features can often increase accuracy disparity across demographic groups. 
There has also been research into how input features influence selection disparity~\cite{emelianov2022fair,bartik2016deleting,garg2020dropping} in a model. For example, Emelianov et al.~\cite{emelianov2022fair} show that that group-wise differences in variance over a model's feature set influence selection disparity, and show under what conditions groups with higher and lower feature variance will be under or over selected. 

%Evidence from the recent monitorship of Upstart, a finance firm which, which involved an in-depth investigation of their model in the search for less discriminatory alternatives, suggests that which features are used for prediction have a statistically significant impact on prediction disparities. 

\krdelete{\paragraph{Methods and Tools for Feature Selection}
Certainly, from a legal perspective, using race or other protected attributes in a model often leads to a violation of disparate treatment~\cite{}. }\krcomment{Disparate treatment is only relevant in certain contexts and even so I personally think leans too much into a misplaced notion of fairness along the lines of anti-classification ideas, but rather than getting into that debate here, maybe just omit the sentence?} While removing race from the model--as a feature and via proxies--may not be an effective method to achieve fairness~\cite{lipton2018does} \krcomment{probably cite our methods comparisons paper here as well?}, in situations where it is useful, Yeom et al.~\cite{yeom2018hunting} provide methods for searching for and removing discriminatory proxies in regression models, and 
%Robertson et al.~\cite{robertson2022bio} provide a method for searching for which features may be producing bias, by showing how features--and importantly, their interactions---can lead to latent encodings of protected attributes. 
Frye et al~\cite{frye2020asymmetric} introduce Asymmetric Shapley Values, a technique which can be used on a wider range of models to determine whether a feature is allowing a protected attribute to causally influence the model outcome, so that the feature can then be pruned. 
Additionally, the FlipTest technique~\cite{fliptest} also produces suggestions of which features may be the source of disparate outcomes across any two populations the user may wish to compare, without attention to causality---this may be especially helpful in narrowing down the list of features to further investigate for impacts on differences in selection rate, or simply to find statistical, and not causal, discrimination.  Finally, Belitz et al.~\cite{belitz2021automating} provide an automatic feature selection framework which only selects features which improve accuracy without reducing a user-specified notion of fairness. However, this method saw considerable drops in accuracy when selecting features in this manner. 

While there is promising work outlining how various aspects of model inputs---such as their variance and causal relationship to protected attributes---influence various notions of model fairness behavior, again there is a lack of testing these results and techniques on on-the-ground pipelines, over a variety of datasets, and also searching for feature selection impacts on a wider set of fairness-related model behavior desiderata.
%there is a large gap between the research completed and a set of ready-to-use tools which can inform model practitioners on how feature selection choices influence model behavior. 
\ebcomment{Some better concluding statement here}.

% \begin{mdframed}
% Tools: Automated Data Validation \textasciitilde ~\cite{breck2019data} $\cdot$ Searching Features for Proxies/Bias \textasciitilde ~\cite{yeom2018hunting,frye2020asymmetric,fliptest}
% $\cdot$ Feature pruning for lowered bias amplification \textasciitilde ~\cite{leino2019feature} $\cdot$ 
% Automatic Feature Selection to improve traditional fairness techniques \textasciitilde ~\cite{belitz2021automating} 
% \end{mdframed}

\paragraph{Key Takeaways:}
\begin{itemize}
    \item Little work has been done exploring the impact of feature engineering and missing value imputation on model fairness, let alone operationalizing tools to help practitioners probe the impact of these decisions in their systems.
    \item Existing tools for data exploration and feature engineering do not account for fairness-related desiderata of downstream systems.
    \item A number of tools have been developed to consider the impact of feature selection on model fairness, but with little empirical testing in real-world contexts and some evidence of limited performance.
\end{itemize}

\subsection{Statistical Modeling}

\paragraph{Hypothesis Class Selection}
There is increasing work pointing out the fairness impacts of using models with increased variance~\cite{blackleave2021}, especially deep models---for example, these models can be more unstable to small perturbations in training setup~\cite{blackleave2021} leading to procedural fairness concerns about the nature of the decision process. 

\paragraph{Optimization Function Selection}
A growing number of works have pointed to degredations of fairness behavior in robust models~\cite{} and differentially private models~\cite{bagdasaryan2019differential, suriyakumar2021chasing}. 
Of course, there is also a vast body of work creating optimization functions to train models satisfy conventional fairness metrics, which we do not discuss in depth~\cite{}. 

Symmetrically, there has also been a fair amount of criticism for conventional group and individual fairness metrics imposed as top-down constraints on a system~\cite{akpinar2022sandbox,suresh2021framework}, and evidence showing that enforcing such constraints can actually degrade fairness according to those same metrics~\cite{}.
\krcomment{Could maybe also point to our tradeoffs paper, the comparison paper, and Emily's vertical equity paper as some examples of where these tools aren't well-suited to real-world use cases, such as where the decision boundary in real life is far away from the decision boundary these models tend to optimize fairness around under the hood?}

However, there is little work investigating the differences in model behavior without additional constraints, simply from changing the optimization functions used---such as Adam versus SGD in deep models, or lbfgs versus SAGA in Logistic Regression. There is preliminary evidence to suggest that differences in optimization functions do lead to differences in fairness behavior: Leino et al~\cite{leino2019feature} show that SGD over-emphasizes high-variance features, especially early on in training, which can lead to increased bias amplification. Investigating how other optimization biases impact fairness behavior may be interesting grounds for future work. 

\paragraph{Hyperparameter Search} Perrone et al~\cite{perrone2021fair} and Islam et al~\cite{islam2021can} show the promise of hyperparameter tuning towards finding fairer classification models. Islam et al~\cite{islam2021can} focus on showing that hyperparameter tuning can lead to increased fairness (differential fairness~\cite{foulds2020intersectional} and demographic parity) at no cost to accuracy. Perrone et al~\cite{perrone2021fair} introduce a technique, Fair Baysian Optimization (FBO), which is model and fairness-definition agnostic, to select hyperparameters which optimize accuracy subject to the fairness constraint. They also experimentally demonstrate that regularization parameters are the most influential for fairness performance, and that higher regularization leads to higher fairness performance in their experiments. We hope that this technique can used to understand further relationships between hyperparameter changes and fairness behaviors over a variety of different models, metrics, and deployment scenarios.

% \krcomment{How are we handling the tools here? Just include a review of all the in-processing methods?}
% \begin{mdframed}
% Tools: ~\cite{perrone2021fair} 
% \end{mdframed}

\paragraph{Key Takeaways:}
\begin{itemize}
    \item Accounting for fairness considerations in the modeling process itself is the most mature area of the FairML literature.
    \item Nevertheless, methods that have been proposed to date are generally built in the abstract and rely on assumptions that fail to translate well to real-world settings.
    \item The proliferation of these methods also pose a challenge for practitioners to navigate the many options and determine which (if any) should be considered in their setting (which may carry appreciable costs when code is either not available or only ``research'' code is available).
\end{itemize}

\subsection{Testing and Validation}

\paragraph{Validation Datasets} Several papers have discussed the perils of evaluating systems on the same benchmark data sets: this can lead to overfitting to specific data sets~\cite{deb_raji} that almost guarantees distribution shift to deployment domains, meaning that results are unrepresentative for many real-world fairness applications~\cite{sambasivan2021everyone}, and suggests that several experimental results in the fairness literature---including those related to pipeline interventions---may be incorrect~\cite{ding2021retiring,li2022data}. Other papers still have drawn attention to specific distributional problems within commonly used fairness benchmarking datasets, such as an under-represetnation of older individuals~\cite{park2021understanding}. 

%Ding et al~\cite{ding2021retiring} introduce a new suite of datasets, based on census data (a superset of the Adult dataset) for benchmarking FairML approaches. Based on this new data, they demonstrate that the effects of fairness interventions vary wildly with geography, and that common truths accepted in the community---such as increasing data size should reduce prediction disparities---do not always hold. While this is a good step, it's important for there to be large, diverse datasets in several domains (healthcare, consumer credit, insurance, education, among others), and beyond this even, to prioritize evaluating fairness approaches \emph{in the systems where where they will actually be used}. 

\paragraph{Model Selection Criteria} 
D'Amour et al.~\cite{d2020underspecification} bring attention to the problem of underspecification, where a model developer insufficiently specifies desirable deployment behavior, leading to biases and other problems during deployment. They argue that most of the model selection metrics currently used in practice---accuracy, robust accuracy, or other metrics--- on a test set insufficiently specifies desirable deployment behavior, and they demonstrate this problem in the context of several models with equivalent accuracies and robust accuracies on a test set having vastly different performance on naturally occurring 
out of distribution samples which the models came across in  deployment.
Black et al.~\cite{black2022model} describe a related phenomenon, model multiplicity, which is when there exist multiple equivalently accurate models for a given prediction task. They argue that there are multiple equally accurate models for almost all real-world prediction tasks, and show how this fact can be be leveraged to push practitioners to search for the least discriminatory model from those available with equivalent accuracy by leveraging legal pressure from the disparate impact doctrine. However, \emph{if model multiplicity is not explicitly harnessed}, it means that model evaluated on the basis of accuracy alone, the current default in machine learning, are almost certainly sub-optimally fair models even when constrained to only consider models with equivalent predictive performance.

\krcomment{Seems like the various fairness audit tools -- AI Fair 360, aequitas, etc fit in here somewhere?}

\paragraph{Key Takeaways:}
\begin{itemize}
    \item A growing body of work has illustrated how choices of validation data and model selection strategies can affect model fairness, however little of this work has been operationalized into tools or methods that can assist ML practitioners in navigating these choices.
\end{itemize}


\subsection{Deployment and Integration}

\paragraph{Accounting for Distribution Shift} A series of recent papers have introduced methods to make models invariant to distribution shift from the perspective of accuracy as well as fairness~\cite{singh2021fairness,coston2019fair,biswas2021ensuring}. Coston et al.~\cite{coston2019fair} develop two methods, one that does not require protected attributes in the training set, and one that does not require protected attributes in the deployment set. 
However, practical evaluations of these methods in deployed systems is still needed to characterize their real-world performance. Additionally, there are several open questions in this area of research: when do we want to ensure fairness criteria over data-drift, and when do we want to alert that the model practitioner that the distributional differences are so large that the model is not suitable for the deployment context?
Are there formulations of data drift were performance can be maintained through updates, but fairness cannot? When these drifts do occur what are best steps for a pracitioner to take to mitigate their impact? How do these systems perform relative to slowly-drifting distributions versus abrupt discontinuitys (such as a global pandemic or significant change in policy or practice)?
\ebcomment{Need help with further questions.}

 
\paragraph{Monitoring}
\krcomment{Would it maybe make sense to merge distribution shifts and monitoring sections? Seems like they're closely related.}
Even when using methods with guarantees on being resistant to distribution shift \textit{in situ}, it is still important for systems to monitor their fairness behavior over time. Two recent papers~\cite{albarghouthi2019fairness,ghosh2022faircanary} propose tools for fairness monitoring over time in deployment. Albarghouthi and Vinitsky~\cite{albarghouthi2019fairness} develop a technique called fairness-aware programming (implemented in Python), which allows programmers to enforce probabilistic statements over the behaviors of their functions, and get notified for violations of those statements---their framework is flexible to many behavioral desiderata even beyond fairness, and can also combine several probabilistic statements and check them simultaneously. The flexibility of the system potentially allows for a wide range of contextualized fairness desiderata to be enforced-- however, it does have limitations; for example, it cannot implement notions of fairness over individual inputs such as individual fairness. %At run time, the system continuously monitors if there is a violation of any of the desired properties and notifies the developer if so. 
Ghosh et al~\cite{ghosh2022faircanary} implement a system that measure the Quantile Demographic Drift metric at run time, a notion of fairness that can shift between group and individual conceptions of fairness based on the granularity of the bins it calculates discrepancies over. Their system also offers automatic mitigation strategies (normalizing model outputs across demographic groups) and explanation techniques to understand mechanisms of bias. Additionally, Amazon's SageMaker Clarify framework allows for the tracking of a variety of traditional fairness metrics to be monitored at runtime~\cite{}. 

However, to the author's knowledge, there is no work that address what fairness problems may come \emph{as a result} of this section of the pipeline: for example, are there examples of model updates from non-fairness aware monitoring pipelines that have degraded fairness performance? \krcomment{Fair point, but maybe a little too nuanced?}
%\ebcomment{What's the punchline here? some ideas: we need to test these on real systems, it's important to see failure modes--how intuitive are they for pracitioners to use, and how flexible *are* they for contextualized notions of fairness? Any other questions we have about the pipeline stage?}

\paragraph{Human-Computer Hand off}
Many algorithmic systems have been built with the ability to defer certain predictions to a human in the case of uncertainty~\cite{black2021selective}, assuming that including humans in decision-making systems will make them less biased. However, there are conflicting results as to whether human-in-the-loop systems out-preform models on their own when it comes to bias. Green and Chen~\cite{green2019principles,green2019disparate} show that including Mechanical Turk workers to aid algorithmic decisions consistently decreased accuracy relative to the algorithm's performance alone, and that humans in the loop also exhibited racial bias when interacting with ML predictions. However, others~\cite{cheng2022child, de2020case} have found that in the case of child welfare screenings, allowing call screen workers \emph{did} reduce disparity in the screen in rates of Black versus white children. 
Symmetrically, Jacobs et al.~\cite{jacobs2021machine} show that including machine learning recommendations in selecting antidepressants for patients did not improve clinician's treatment decision performance, and in fact, interacting with incorrect recommendations---even when supplied with explanations---lead to decreased performance. 

Taken together, as many have noted, these results show that ML decision systems which include human intervention must be tested for accuracy and bias as a whole rather than on algorithm outputs alone. These results also suggest that the efficacy of human intervention is very context-dependent. However, there little progress on how to infer when handoff problems will occur, or how to mitigate these inefficiencies. 
\marginpar{can someone add some papers that show that explanations don't really help either?} 

There has been a stream of theoretical work from the algorithmic fairness literature trying to model or guarantee fairness in a joint human-ML system~\cite{keswani2021towards,madras2018predict}. For example, Keswani et al~\cite{keswani2021towards} learn a classifier and a deferral system for low-confidence outputs, with the deferral system taking into account the biases of the humans in the loop. Donahue et al.\cite{donahue2022human} develop a theoretical framework for understanding when and when not human and machine error will complement each other, i.e. when human and machine error will occur in different areas of the distribution and cancel each other out, leading to increased performance, and suggest how this can inform the design of human-in-the-loop systems. While this initial largely theoretical work is promising, these techniques should be tested and compared on deployed systems---when do deferral systems work in practice, and can they lead to biases of their own? Do the human-in-the-loop design suggestions work in practice?



%\marginpar{Do we need to look at CHI for this?}
%Little attention has been paid to organizational integration in the fairness literature surveyed. 
%There has been some work showing that humans and machines working together can often compound errors rather than prevent them~\cite{I think some ben green stuff, maybe something from jen and hannah wallach}, but little progress on how to infer when handoff problems will occur, or how to mitigate these inefficiencies. 


\paragraph{Organizational Biases}
Organizational biases can enter an ML decision system through other means than deferring to a human in the loop. While there is evidence of the fact that organizational biases influence algorithm conception and the pipeline wholistically e.g.~\cite{passi2020making} from interview-based studies, there are is little documentation of examples of when and how this occurs and how it specifically influences predictions. Lum et al.~\cite{lum2020impact} document one such example, showing that inputs to risk assessment models, specifically, the charges that a defendant it booked for, are often over-exaggerated for Black defendants, and thus incur bias against Black defendants in model usage. (Presumably, this would happen even if the underlying model is ``fair''). \krcomment{Lum here actually seems like it might fit into the discussion of data or label biases above? What seems distinct here might be more along the lines of biases in intervention effectiveness or implementation, such as conducting outreach calls only in English or providing after school programs that can't be utilized by students that need to work or care for siblings after school, etc. However, most of these issues won't really show up in the ML literature we surveyed (more likely in the policy literature), so perhaps it would make more sense  to add a sentence or two about these broader organizational questions under the human-computer handoff heading rather than having a separate sub-section here?}

Overall, organizational integration especially lacks in \emph{measurement and mitigation} of fairness problems arising from this section of the pipeline. In addition, the literature on human-computer interaction and organizational biases do not come near understanding all of the (fairness-related) failure modes of organizational integration. For example, is just one ML system used in the decision system? Some systems in government, for example, use multiple models to inform decisions~\cite{blackIRS2022}. In these situations, how are these predictions combined, and are the models built to be used in unison? What are the impacts of rule-based decision frameworks imposed on top of algorithms predictions, such as those use in pretrial risk assessment tools\~cite{}? 

\ebcomment{It would be great to have some help pointing out what is missing here---mapping organizational frameworks, other ways of model integration into a larger decison-making framework can lead to problems.}

\paragraph{Key Takeaways:}
\begin{itemize}
    \item Recent developments in methods robust to distribution shifts seems promising but need more testing in applied settings and several questions remain for both research and practice.
    \item Monitoring and maintenance of a deployed system is just as important meeting fairness desiderata in the initial development. A growing number of monitoring tools can facilitate this process for practitioners and users of these systems.
    \item Particularly in high-stakes settings, many ML models are being used to inform human decision-making rather than acting autonomously. In these settings, it is critical to understand not only the fairness properties of the model, but those of the entire human-ML system acting together.
    \item The deployment context and specific decisions being informed by a given model also matter deeply in terms of how a model's fairness properties---as narrowly defined with respect to metrics relating to its predictions---will relate to the actual impact on people affected by the model's outputs.
\end{itemize}

\subsection{Documentation}
Several works have pointed to the need for documentation in machine learning pipelines~\cite{gebru2018datasheets, koesten2019collaborative, black2022model}. For example, Koesten et al~\cite{koesten2019collaborative} point to lack of documentation as a source of failure in collaborative data use, such as passing data sets between research groups or collaboratively creating data sets---for example, incomplete documentation may lead to a misunderstanding of data cleaning steps that took place. 
Checklists for how to document machine learning systems abound~\cite{}, but automated tools for documentation would severely decrease the load on practitioners.  While such tools are few and far between in the fairness literature, they exist in other spaces: for example, Wrangler~\cite{kandel2011wrangler} provides a method of logging data cleaning steps for review, documentation, and reproducability. However, there is a need to find such tools and convert them to include model fairness specific functionality.

\krcomment{I see why you split this out here, but it also doesn't really feel like it fits as a distinct pipeline step. Perhaps we could make it a separate sub-heading under Deployment and Integration instead? Also seems like some of the model cards stuff would fit here:

\url{https://dl.acm.org/doi/pdf/10.1145/3287560.3287596?casa_token=DyLeBck72WgAAAAA:E3xvjZ4p5tM629YLYCQqq3HVB29HCQMaC_7Ua41FxXbAFOnCqn1nfvsAfRtUWVKp2pYWghkjMV7IGzo}

\url{https://dl.acm.org/doi/pdf/10.1145/3531146.3533108?casa_token=Dv5l8KuMpbQAAAAA:IAXd1Z1dM1vDuzRxzn1XPkOIEEJz3v0pWcniqMfz8g693eApvA7Vlc7wmQYgC2E2SrAaA6vWxbrkWgk}
}

\paragraph{Key Takeaways:}
\begin{itemize}
    \item Several papers have called for better documentation of models and datasets, both for research and practice, and various proposals have been made for more standardized formats. However, these efforts would be assisted by adapting some of the tools and automation that exist in other spaces to lower the barriers to developing good documentation in the ML space.
\end{itemize}
 
 %Koesten et al~\cite{koesten2019collaborative} point to sources of failure in collaborative data use, such as passing data sets between research groups or collaboratively creating data sets---for example, one failure mode they point to is having an incomplete understanding of data cleaning steps that took place before working on a dataset created by another group. They point to user needs of such collaborative data pipelines, such as open channels of communication and version control, but do not create tools to operationalize these needs. 


\subsection{Consideration of the total pipeline}
%One notable recent work by Donahue et al.\cite{donahue2022human} develops a theoretical framework for understanding when and when not human and machine error will complement each other, i.e. 

\ebcomment{Help finding works and tools that consider the entire pipeline at once?}

\krcomment{I don't think there's really a lot out there---certainly this is the gap that the sandbox toolkit is seeking to fill in part. Likewise, our method comparison paper looked at pre-, post-, and in-processing methods separately, but didn't attempt to consider their interactive effects. I'd probably suggest removing the heading here and commenting on the need for more research in this direction as a major element of the research agenda (while noting that operationalization of the different components would also make this a lot more tractable)}



\input{survey_table.tex}
%\input{survey_table_simple.tex}


==> versions/survey_2.tex <==
\section{A Survey of Pipeline-Fairness}
\label{sec:litreview}

\ebedit{As a first step towards operationalizing the pipeline-based approach to fairness in ML, we provide a review of the ML fairness literature focused on creating a taxonomy of fairness work that locates, measures, or mitigates problems along the ML pipeline. In addition to serving as a first step towards a tool that ML practitioners can use to identify ways to diagnose and mitigate problems in their pipeline, our survey of the work already done allows us to point to the gaps in the literature that must be addressed in order to have a full understanding of how choices made along the ML pipeline translate to model behavior-- and then build tools which operationalize this understanding to build less harmful pipelines.}

%We focus on work that does not fall into the category of adding an optimization constraint to a model in order to enforce a fairness metric, or resampling data, in order to highlight how 


\subsection{Survey Methods and Organization.}

\hhcomment{I think we can justify our focus on ML venues by saying that we were interested in measures and remedies that could be useful to ML practitioners; hence the focus on these venues.}
\kredit{In order to better understand the current landscape of algorithmic fairness research throughout the ML pipeline, w}e performed a thorough survey of the recent \krdelete{algorithmic fairness }literature, which we classified into categories depending upon which area of the pipeline they analyze. We gathered papers from NEURIPS, ICML, ICLR, FAccT, and AIES, for the past five years, i.e. 2018-2022, that contain any of the following terms in their title, abstract, or keywords: "fairness", "fair", "discrimination", "disparity", "equity".\footnote{When available: this is with the exception of NEURIPS, which we gather for years 2017-2021 due to the date of the conference relative to the time writing this work, and EAAMO, which started in 2021.} In addition, we performed a series of Google Scholar searches to ensure our survey did not miss high-impact work published in other venues: One search used the keywords listed above and included papers published in any venue in the past five years with over 50 citations, through the top 50 results returned by this Google Scholar search. \krdelete{This is to ensure that we do not miss any high-impact work from other venues. Finally, we perform} Additional Google Scholar searches used keywords from each step in the pipeline individually, to attempt to find papers targeted at each stage: for example, "data collection" and "fairness" and "machine learning". This results in \textcolor{orange}{\textasciitilde1000} papers overall. 

\marginpar{\textcolor{blue}{Here, I try to define what pipeline fairness is again. Do we want a better definition?}}
We then manually inspect each paper to understand whether and how the reported research is an instance of a pipeline\hhedit{-aware} approach to fairness. \textcolor{blue}{That is, does it identify, measure, or mitigate a fairness problem that arose as a result of a choice made along the AI model creation pipeline?} \hhedit{Alternative framing: That is, does it locate, measure, or mitigate a concrete cause of unfairness along specific stages of the ML pipeline?} If so, we categorize the paper along two axes: what part of the pipeline it corresponds to (problem formulation, data choice, feature engineering, statistical modeling, testing and validation, or organizational realities), and whether it identifies, measures, or mitigates a pipeline fairness problem. 

While we acknowledge that adding optimization or loss constraints to a model to enforce a given definition of fairness is in itself a modeling choice and thus fits in to the ``pipeline'' notion of fairness \hhedit{(specifically, under the statistical modeling, choice of the objective function)}, we separate these more traditional fairness papers from our understanding of pipeline-based fairness papers for the sake of this survey by giving them their own category, which we call ``Algorithm''. \krcomment{Not too sure I see the necessity of calling out this distinction separately -- aren't we just saying the choice of algorithm is one component of the pipeline? Especially given the length, maybe just cut?}


\subsection{High-Level Overview and Takeaways}
\begin{itemize}
    \item Our first observation is that the number of fairness papers which adopt a pipeline perspective to fairness is far outnumbered by the more traditional, abstracted approach to fairness: XXX papers versus XXX papers overall. \hhcomment{Might be nice to do a histogram, showing numbers per pipeline stage.}
    \item The algorithmic fairness literature has a dearth of knowledge about what on-the-ground pipelines look like: although there are many papers that outline abstracted pipelines (including our own), the actual model creation steps taken by practitioners for a variety of real-world systems (e.g. in consumer finance, healthcare, hiring systems) are at the very least not catalogued in any centralized place. 
    \hhcomment{The point being made here is not clear to me.}
    \item Even within the list of papers that do take a pipeline-based approach, the majority of them are \emph{proof-of-concept}: there is much work to be done to take the solution proposed in the work into an implementable \hhcomment{generalizable?} fix for pipeline problems. To start, it would be excellent if papers with solution techniques had code available to implement their approaches. 
    \item Within pipeline-fairness oriented papers, the majority investigate problems with data collection and pre-processing.  
    \item Most pipeline-related papers focus on \emph{one issue} in the pipeline, but fail to provide insight into how these different aspects of the pipeline interact. Does solving each issue in isolation work?
    \item Many of the pipeline papers still engage with one particular notion of fairness (often demographic disparity). It would be helpful to create a more generalized mapping of how modeling choices change prediction behavior, beyond a single metric.
    \item There is a dearth of case studies of bias mitigation in the fairness literature. Though case studies may often be disregarded as ``simply implementing old methods'' and thus not novel, it is crucial that we give them more attention so that we can learn about the failure modes of the techniques that we create. While there are \hhedit{notable} papers about the overall problems of production teams, e.g. ~\cite{madaio2020co,holstein2019improving,sambasivan2021everyone}, these still do not provide in depth-detail of the bias mitigation process in deployed systems. 
\end{itemize}



\subsection{Viability Assessments}
To the author's knowledge, there is very little work within the fairness literature on documenting, detailing the bias that can arise out of, or mitigating bias from the viability assessment process: how we investigate the benefits and downsides of the current decision-making system in place in comparison to what an ML-based solution could provide, and assess organizational capacity for effective system evaluation, design, and deployment. Important considerations in this category include (but are not limited to) community buy-in, access to high-quality data, sufficient organizational ML expertise, capacity for continued monitoring. 

Viability assessments provide an avenue for refusal to build an ML system, which is understudied in the fairness literature~\citep{raji2022fallacy}. Though there have been discussions in the community around when to refuse to build~\cite{barocas2020not}, there is little published work on case studies detailing how the decision to build or not build was made. 
%--- et al~\cite{find_that_paper} point to the fact that ML researchers and practitioners do not often consider the option to not build a system because it is taken as the default, given the pressures (and funding) coming from the tech industry. 
Indeed, many works that point to how 
organizational factors---such as lack of a company's support for ethical AI approaches, or time pressure, or focusing only on client demands~\cite{passi2020making} can lead to pushing ML systems ahead without careful consideration of whether or not deploying a system in that domain is a net benefit in the given context. \krcomment{Not published in an academic venue, but perhaps we should point to the DSaPP Scoping Guide here, as well as specific fairness/inclusion issues it details? http://www.datasciencepublicpolicy.org/our-work/tools-guides/data-science-project-scoping-guide/}

\paragraph{Key Takeaways:}
\begin{itemize}
    \item Work around the fairness implications of viability assessments for ML systems is almost entirely lacking in the FairML literature, leaving appreciable open questions around decisions of whether or not to build a system, stakeholder engagement, and identification of overall goals of a project.
\end{itemize}


\subsection{Problem Formulation}
Problem formulation encapsulates the decisions made when translating a nebulous policy or business goal into a prediction task: e.g. translating ``predicting creditworthiness'' into ``predicting loan default''~\cite{passi2019problem}. 

Problem formulation is also a time to access whether a proposed ML system will address the actual needs of the organization to which it will be deployed. 
While not describing this process as problem formulation per se, Katell et al. detail how their design ideas changed over time through their engagement with community stakeholders while building an Algorithmic Equity Toolkit to aid activists in participating in public comment session when evaluating ML systems to be used by the Seattle city government~\cite{katell2020toward}; and Suresh et al~\cite{suresh2022towards} detail how they co-designed a tool for collecting news articles documenting cases of femicide.  


\paragraph{Selection of Prediction Target} 
While there is helpful discussion on how prediction target selection may lead to bias, often drawing from the social science literature of validity theory~\cite{passi2019problem,jacobs2021measurement,coston2022validity},
as well as examples of disparities stemming from prediction target selection selection~\cite{black2022algorithmic,obermeyer2019dissecting,human_rights_watch_2020}, to the author's knowledge, there is little work in the ML fairness literature detailing the process of problem formulation in practice, or leveraging fair ML tools to measure or mitigate the potential bias of the selection of a given prediction target ex-ante. 
Developing protocols for assessing problems of various notions of validity (internal, external, content, predictive) of the target variable and predictive attributes is a promising and necessary avenue of future work. There is preliminary work along this axis in the form of checklists and protocols, e.g.~\cite{coston2022validity}, but we suggest it may be possible to make a suite of quantitative tests as well.
For example, access to appropriate data, ML practitioners could leverage existing model-level bias-testing frameworks~\cite{AIF360} to test for bias across a series of potential prediction tasks to inform the decision of which to choose. Tests for predictive validity simply require investigating whether the proposed target variable is predictive of other related outcomes. Obermeyer et al.~\cite{obermeyer2019dissecting} used such a test to uncover the racial bias behind using health care cost as a proxy for health care need, by regressing health care cost on other metrics of illness (e.g. the number of active chronic conditions a patient has), finding that there was a disparity in the correlation between health care costs and sickness in white patients versus that in Black patients. Investigating the extent to which questions of construct validity and reliability can be operationalized into a set of tests (e.g., testing correlations between potential prediction tasks, or checking for consistent model performance across two different methods of measuring the output) may be a promising area for utilizing tools and methods from social sciences.

\paragraph{Selection of Prediction Universe}
\krcomment{The choice of cohort/universe for analysis and when to make a prediction actually seems pretty salient in terms of formulation as well. Here I'm talking about things like up-front decisions about who to make predictions on: Suicide risk among everyone in the population or just people with some history of mental health needs? Do I predict the likelihood of not graduating high school as of 2nd grade, 9th grade, 11th grade, etc? I'm certainly not aware of anything in the literature that actually looks at this (either systematically or via case study). Did you identify anything there?}\hhcomment{This is a very good point, and it reminds me of a related but distinct set of recommendations around 'studying up'~\citep{barabas2020studying}.}

\paragraph{Selection of Predictive Attributes}
\ebcomment{Help.} \hhedit{The discussions of validity and reliability outlined in the previous paragraph are just as well applicable to the features utilized for prediction. Many such features may aim to reflect social constructs such as race or gender~\citep{}. Additionally, Prior work has observed that trained models may rely on spurious correlations, that renders their predictions unreliable in presence of confounders and slight changes to the data distribution. We believe that close deliberation with domain experts would allow for the appropriate selection of features.} \hhcomment{We can mention the DoWhy package as a tool here.} \krcomment{To avoid confusion, I might actually integrate this into the data acquisition or feature selection/engineering discussion -- I feel like in practice it's generally difficult to get to the detail of choosing specific predictors this early in the process}

\paragraph{Determining Behavioral Desiderata}
\hhcomment{I think the following paragraph should be moved to "testing and validation" section. The details of the examples you mention can be moved to an appendix. Citation to these pieces suffice.} \krcomment{I'm a little on the fence there -- generally I think it's important for some of this goal/fairness metric definition to happen up front, but it's hard to avoid some repetition. I guess in the interest of space, consolidating with testing and validation might be cleanest?}
While we leave the question of finding an appropriate fairness metric to other work and focus instead on bias mitigation techniques, we wish to highlight the importance of finding \emph{contextualized} notions of bias and fairness to encourage in a system. For example, Black et al.~\cite{black2022algorithmic} show how \emph{vertical equity}, the public finance notion that individuals with different incomes and wealth must be treated differently in order to achieve fairness overall, is not achieved by enforcing traditional fairness metrics--- instead, the authors favor audit selection models with more monotonic audit selection distributions, which also display high selection overlap with an oracle model which selects individuals in order of highest tax misreport (i.e. most money not reported to the Internal Revenue Service). Mattei et al.~\cite{mattei2018fairness} consider the unique fairness requirements of organ-matching systems, noting that it was important for younger organs to be matched to younger recipients, and also to ensure that individuals did not receive different probabilities of getting an organ due to their blood type. Other examples of contextualized fairness desiderata include [CITE HERE]. \ebcomment{This is not the best example because it's a matching system instead of an ML system-- does anyone else have a more contextualized notion of fairness in a prediction system example?}
%we briefly note that a pipeline fairness approach can also naturally lead to a more in-depth, contextualized understanding of the ML system, making it more natural to define more context-specific model behavior desiderata than the most common fairness metrics. 
%Case studies of fairness problems in real-world deployed systems are especially helpful in understanding what 

\paragraph{Key Takeaways:}
\begin{itemize}
    \item Although some work does exist on the importance of label choice to system fairness, including compelling case studies, little is available to practitioners in terms of operationalized tools to help inform this choice.
    \item Despite the significance of the choices surrounding the definition of the prediction universe for defining who might have an opportunity to receive a benefit, we were unable to find any work in the literature exploring the downstream fairness implications of these choices.
    \item \krcomment{Probably move predictors / desiderata to sections below?}
\end{itemize}

\subsection{Data Collection}
Far and away, besides enforcing fairness constraints on models during training or prediction, the aspect of the pipeline that has received the most attention is data collection.  

\paragraph{Mapping effects of faulty data collection to model behavior} Several papers in the algorithmic fairness literature have pointed to the problems of disparate performance and selection across demographic groups stemming from datasets which are unbalanced across demographic groups, i.e. have sampling bias, both in terms of sheer representation, and representation conditional on outcomes~\cite{buolamwini2018gender, mishler2019modeling}; or have data that is \hhedit{disparately noisy} or perturbed in some way~\cite{wang2021fair}. Li et al.~\cite{li2022data} do a particularly thorough job of testing how potential results of data collection problems---e.g. unrepresentative samples, insufficiently small data samples, differing group base rates\footnote{Which could be true or the result of measurement error}---influence machine learning model behavior from the perspective of accuracy and fairness. They test the influence of these sources of collection bias comparing performance across models  trained on subsamples of \krdelete{an enormous, novel,} a criminal justice dataset (1.5M rows). Interestingly, they find that increasing dataset size, or even reducing the disparity in base rates, does not always reduce disparities in selection, false positive, or false negative rates. Other recent work introducing new datasets for testing fairness interventions find similar results~\cite{ding2021retiring,akpinar2022sandbox}. These papers are an excellent start to mapping data bias issues in the pipeline and immediately brings to mind more questions---how do these sampling and measurement errors impact other fairness desiderata, how do they interact with other pipleline choices such as model selection, loss function selection, and hyperparameter tuning? 

\paragraph{Mitigating biased model behavior on biased data}Proposed techniques for mitigating the effects of unrepresentative data include a variety of synthetic data augmentation techniques~\cite{sharma2020data, van2021decaf, chawla2002smote}, data re-weighting techniques~\cite{kallus2018residual}, and specialized optimization functions for creating fair classifiers (according to traditional metrics) with unbalanced data~\cite{jiang2021towards, li2021autobalance}. Coston et al. introduce a model training approach that can mitigate the effects of the selective labels problem~\cite{coston2021characterizing}.


Some argue that using modeling techniques such as re-weighting or using special loss functions serve as a band-aid solution, and argue that data problems should be solved by intervening on the data. Liu et al.~\cite{liu2021can} show how to find which subgroup in the data is likely to have noisy labels, and then introduce a technique of inserting \emph{more} noise into the labels of other subgroups in order to increase fairness and generalization, and often accuracy as well. Chen et al.~\cite{chen2018my} introduce methods of estimating the value of adding additional training samples from the perspective of thus improving many fairness outcomes such as equalized accuracy---potentially allowing for practitioners to decide whether searching for extra training examples or features is worthwhile.  


Several methods are also available for creating fair classifiers with noisy, corrupted or perturbed data~\cite{liu2021can}. 
Wei et al~\cite{wei2021learning} provide an interesting counterpoint to the papers which discuss creating fair classifiers on noisy data: they point to the differences in model behavior when trained with artificially noised data (i.e., following some specific noise distribution, such as Gaussian), as opposed to noisy data that is mislabeled by human annotators: for example, they show that harmful model memorization is much more common on models trained with mistakes in human annotations, since the human annotators mislabel examples that are inherently more confusing and thus informative for the model (e.g. a hard-to-distinguish photo).
As a form of solution, they provide a new noised version of CIFAR-10 and CIFAR-100 with errors by human annotators to better study the problem of noisy data in practice. 
This paper points to the peril of training and evaluating models on ``sterile'' data: they point out that our intuitions about the effects of noisy data on model behavior may be flawed, underscoring the need to test for pipeline-based problems and solutions on pipelines data to be used during deployment.
\krcomment{Seems like we should discuss approaches that focus on resampling/balancing the training data here as well -- similar to the inconsistency above, in our method comparison work (https://arxiv.org/pdf/2105.06442.pdf), we found a lot of variability across datasets and parameters in the ability of resampling to have any impact on model fairness. Some of the references there are a bit older, but we could also point to them for others looking at resampling (see the "Resampling" heading on page 2)}



%Cai et al~\cite{} suggest to a method of selecting individuals to seek labels for in order to improve the system the most from an equity standpoint. 
%Sharma et al.~\cite{sharma2020data} introduce a method of data augmentation which guarantees improvements in reducing demointroduces data with perturbations to the demographic group (i.e., switching demographic group) while keeping other feature and labels constant, as well as keeping demographic group constant and flipping outcome labels, crucially, slowly in order of likelihood within the probability distribution--- creating a family of datasets

\paragraph{Sources of bias in the sampling and labeling process} While several of these papers do show how machine learning systems change their behavior as a result of different kinds of data noise or unrepresentativeness~\cite{wang2021fair}, they do not speak to the source of bias in the sampling or labeling process, and how to correct it at the source. The Human and Computer Interaction community has done a much more thorough job of considering what failure modes can occur in the data collection process itself, especially as a result of crowd sourcing data set labels with workers from platforms such as Mechanical Turk~\cite{sen2015turkers,hube2019understanding,miceli2020subjectivity}. For example, Diaz et al~\cite{diaz2022crowdworksheets} point to the fact that crowdworker identities influence how they answer labeling prompts~\cite{sen2015turkers} \krcomment{The references here are confusing -- how does the Sen 2015 reference relate to this sentence?}, and introduce CrowdWorkSheets, a worksheet to help guide practitioners through, and allow them to document, the process of creating a dataset with crowdsourced labels with crowdworker identity in mind, from specifying the question of what crowdworkers are to label, to accounting for demographic differences in crowdworkers, determining compensation, among other considerations. However, they do not test the use of their worksheet on production teams. 
An exemplary paper by Sambasivan et al.~\cite{sambasivan2021everyone} provides a wider set of examples of real-life sampling bias and labeling bias, and importantly, \emph{how they entered a real-world system}.  In one set of examples, ``physical world brittleness'' brought about several senses in which deployment data was distributionally different from training data, leading to failure modes, and often abandonment of the AI project: e.g. ``hardware drifts'', where hardware systems which were the source of medical imaging data were not updated over time, leading models to give inaccurate results; or ''human drifts'' where human behavior changed over time leaving models useless, such as models build to predict disease spread over the course of the Covid-19 pandemic.  Another large failure mode identified was a lack of ``cross-organizational documentation'', which lead ML practitioners to make assumptions about aspects of the data, such as timestamps, introducing severe noise into the training data. 

The above papers are a great source of general pointers to data collection problems ignored in the ML literature, but there is still a dearth of deep investigations into \emph{specific} data creation pipelines and the particular sources of bias that show up in those systems, as well as contextualized mitigation strategies. 
There are some exceptions: Marda and Narayan~\cite{marda2020data}, show sources of historical bias, sampling bias, measurement bias, and direct discrimination as well as arbitrariness in the collection of data for the creation of Delhi's predictive policing system: for example, for measurement bias, they explain how the techniques used to map Delhi were inconsistent over the development of the tool, since the police department's ArcGIS system license expired; that there were often no formal addresses for less wealthy parts of the city thus identifying call location was largely guesswork; and that women who made calls were less likely to know their address since they often largely stay inside and are less aware of their surroundings.

More generally, while this literature does an excellent job of illuminating failure modes that can be surfaced through engaging with practitioners---since many papers in this area are structured around interviews---they may elide more low-level technical sources of data collection problems, such as record linkage issues leading to non-IID data dropping. While they are extremely helpful in the important first step of identifying problems, they provide little direction for creating operationalizable solutions to these problems, or even sufficiently detailed information about each system studied to be able to understand the mapping between data collection problems and model behavior.\krdelete{

Operationalization of a pipeline-based approach to fairness necessitates harnessing both the outcomes- and solution- focused algorithmic fairness literature which ignores the sources of problems, and the problem identification prowess of the HCI, CSCW, and other literatures. 
}
One paper by Goel et al.~\cite{goel2019crowdsourcing} comes closer to operationalization of a solution for a specific problem in the data collection pipeline: differential accuracy of crowdworkers in labeling tasks. They introduce a technique for assigning Mechanical Turk workers to labeling tasks in order to decrease disparity in false positive and false negative labels. It requires a subsample of datapoints (gold tasks) where the researchers know the true label of the data to be labeled in order to estimate the group-wise accuracy of each labeler. However, crucially, they do not test their technique in their own labeling task, but use datasets already annotated with Mechanical Turk workers as well as synthetic data---such approaches must be tested within actual labeling processes. 

\krcomment{There's a lot here on crowdsourced labels -- I guess because it's an easy system where the researchers have control over the label generation process -- and I think we can shorten it down to a paragraph or so. Seems like we should also point to some of the more real-world instances of label and sampling biases: differential enforcement of drug laws and biases in traffic stops come to mind as some of the important examples there. Of course, much harder to address without fixing the world. Likewise, seems like some of the work around biases in facial recognition arising from lack of representation in training data fits in here as well. 

\url{https://drive.google.com/file/d/1B58Os2Hb2v__YQ8whdWRULY9mgxxsHoO/view}

@Rayid -- I'm having trouble finding the drug arrests paper I'm thinking of right away (I think it looked at Oakland vs Berkeley?) but you might know it off-hand?

http://proceedings.mlr.press/v81/buolamwini18a/buolamwini18a.pdf
}
 
\krdelete{As a whole, we first note that while there is some excellent work in this area, data collection pipelines---and pipelines in general--continue to be poorly mapped, and thus not all sources of bias or failure are even identified. Secondly, there is a disconnect between problem discovery and mitigation techniques. While it may be that checklists, questions, and datasheets are the best solution to some sources of errors and bias in the data collection pipeline, (and the pipeline overall), there may be some more objective tests that can be performed to test whether data is being sampled, labeled, and measured in a defensible way. Thirdly, the work of mapping pipelines, identifying potential sources of bias within the choices therein, testing to see under what circumstances biases arises, and creating and testing mitigation techniques, is work that, to the extent that is has been done, is spread across multiple disciplines: from machine learning to database management. We should search for, study, and adopt techniques from these areas in order to create a mapping of machine learning pipelines for bias prevention.  
Finally, and perhaps most importantly, \emph{proposed methods should be tested in a variety of real-world systems} to see where they fail and when they are helpful. }

\paragraph{Key Takeaways:}
\begin{itemize}
    \item While there is some excellent work in this area, data collection pipelines---and pipelines in general--continue to be poorly mapped, and thus not all sources of bias or failure have likely even been identified.
    \item There is a disconnect between problem discovery and mitigation techniques. Although checklists and datasheets may be a solution to some sources of data collection bias, there is a lack of more objective tests to ascertain whether data is being sampled, labeled, and measured in a defensible way.
    \item Empirical work the relationship between between dataset size as well as group and label balance has shown inconsistent results in terms of impacts on downstream disparities, highlighting the complexity of the problem and limitations of solving model fairness issues at the level of data alone.
    \item What work that has been done in this area is spread across multiple disciplines: from machine learning to human-computer interaction to database management. We should search for, study, and adopt techniques from these areas in order to create a mapping of machine learning pipelines for bias prevention.
    \item Most importantly, proposed methods should be tested in a variety of real-world systems to see where they fail and when they are helpful. \krcomment{maybe rephrase these last two more as gaps and move the calls to action to research agenda?}
\end{itemize}

\hhcomment{I think Datasheets is one paper that should definitely be discussed in this section. }

%posit that we must combine the literature of problem discovery from a variety of literatures and work towards potential mitigation tactics, crucially, tested in real-world systems. While this may not lead to generalizable results at first, another active area of research may be what aspects of prediction problems or pipelines lend themselves to certain types of solutions.

%Beyond these instructive examples, Sambasivan et al. also provide a helpful overview of available methods and attempts to prevent such problems from a variety of literatures, including human-computer interaction, and data management science, including methods of logging data cleaning steps~\cite{wrangler}, enforcing validity constraints on data~\cite{}, incentivising 


%, and given insights from Sambasivan et al.~\cite{sambasivan2021everyone}, it seems 
%points to the need to evaluate models on data with noise distributions , and the investigation of the fairness effects of real-world noisy data.

%The computer science literature is solution-focused, and often develops a technique to mitigate the problem identified---but often in the form of a generalized band-aid, not investigating the causes of the problem in the data. On the other hand, HCI and related literatures delve
%There have been very few papers which lay out the entire end-to-end process of 


%Both literatures suffer from focusing too much on painting a general picture---overarching themes of failure points in processes and generalized solution techniques. We also need a taxonomy of examples of specific problems that have occurred, and how they have been solved

%However, despite this literature being rich in documenting overall patterns of 

\subsection{Data Preprocessing}

While there are many papers in the fairness literature that discuss how to \emph{leverage} preprocessing for bias mitigation~\cite{Zhao2020Conditional,cheng2021fairfil,balunovic2022fair,zemel2013learning}, to the author's knowledge, there is little work detailing how preprocessing steps may \emph{introduce} bias. 

\paragraph{Feature Encoding and Missing Values} A body of work has explored how preprocessing steps---such as data representation (e.g. discretized or continuous numerical values) normalization techniques, and strategies for data dropping and imputation---can influence classification model behavior~\cite{alshdaifat2021effect,biswas2021fair,crone2006impact,zheng2003existence} in a model-dependant manner. These effects can often be significant: Crone et al~\cite{crone2006impact} state that that the performance differences between preprocessing steps often rivaled that of the differences between using different models (SVM versus NN). In the context of predicting purchase behavior online, Zheng et al.~\cite{zheng2003existence} state that different methods of encoding the unit of analysis (what consititutes a purchase session) lead to ``radically different conclusions'' from model behavior.
Given that preprocessing can drastically influence model prediction performance, it must influence fairness behaviors as well. However, there is little work in this area. Biswas et al.~\cite{biswas2021ensuring} perform an analysis of how different preprocessing steps can influence fairness behavior, and show, among other effects, that dropping rows of a dataset with missing values instead of imputing those rows can lead to sizable differences in fairness behavior due to the changes to the training distribution. While this paper is an excellent first step, it would be instructive to understand how a larger array of (potentially context-specific) preprocessing steps lead to changes in model behavior---for example, how exactly different features are defined, e.g. encoding attributes such as age in various datasets in continuous or binned. Other avenues for future work include investigating fairness impacts beyond the metrics discussed in the paper,  how these data preprocessing steps interact with the inductive biases of a larger variety of models, and developing methods for how to choose between preprocessing options given information about the data and the modeling pipeline.
%Another large area of focus is methods for ``debiasing'' data by making a representation of the training data which is independent of the protected attribute~\cite{Zhao2020Conditional,cheng2021fairfil,balunovic2022fair,zemel2013learning}, which we do not focus on in detail. \ebcomment{ugh this doesn't really feel relevant: it's not a result of data collection bias}. 

Wan~\cite{wan2022fairness} presents an interesting case study of how data representation can affect bias in NLP translation models, and an interesting mitigation technique. They show that differences in translation performance between different languages may not have to do with the structure of language itself, but instead with the granularity of the representation of the language: for example, word length (longer words lead to lower performance), and how many bytes it takes to represent characters in a word. This performance disparity can be mitigated by using more granular representations of language pieces to equalize representation length across languages (e.g. subwords, different representations for characters). They also call for the creation of a new character encoding system that  encodes characters outside the English alphabet more efficiently than current methods to further mitigate bias stemming from representation length. 

Despite the capacity for feature engineering and imputation choices to affect model fairness, our survey failed to identify any tools that assist practitioners in mapping out the effects of their prepossessing choices from the perspective of preventing bias and suggesting mitigations. However, there may be some potential for adapting tools that have been developed for more general data exploration and preprocessing to incorporate fairness contributions as well. For instance, Breck et al.~\cite{breck2019data} describe a data validation pipeline for ML used at Google that proactively searches for data problems such as outliers and inconsistencies; and there are several data-cleaning tools which even suggest transformations according to best practices~\cite{hynes2017data, krishnan2016activeclean}. Further exploring the landscape of these more general tools and their potential applicability to questions of model fairness seems to be a fruitful avenue for future work. Crucially, however, we note that we are unaware of any such systems that presently account for bias-related desiderata.

%\paragraph{Preprocessing Opacity} 
% Koesten et al~\cite{koesten2019collaborative} point to sources of failure in collaborative data use, such as passing data sets between research groups or collaboratively creating data sets---for example, one failure mode they point to is having an incomplete understanding of data cleaning steps that took place before working on a dataset created by another group. They point to user needs of such collaborative data pipelines, such as open channels of communication and version control, but do not create tools to operationalize these needs. 

% There are other mitigation techniques for some of the problems that result from collection: for example, Wrangler~\cite{kandel2011wrangler} provides a method of logging data cleaning steps for review, documentation, and reproducability; Breck et al.~\cite{breck2019data} introduce a data validation pipeline for ML used at Google; and there are several data-cleaning tools which even suggest transformations according to best practices~\cite{hynes2017data, krishnan2016activeclean}. We acknowledge that this literature review does not go deep enough into these other areas. We leave this for fruitful areas of future work. Crucially, however, we note that these systems do not take explicitly take bias-related desiderata into account.

\paragraph{Feature Selection}
Despite some evidence suggesting the choice of features used for inference also impacts model fairness behavior, a number of important open questions remain in this area as well. A fair amount of work has considered the impact of spurious correlations at the intersection of fairness and robustness: many papers that argue about the danger of spuriously correlated features, especially from the perspective of fairness in its relation to causality, and propose methods to remove them~\cite{wang2020towards}, however, Khani et al~\cite{khani2021removing} show that removing spurious features can often increase accuracy disparity across demographic groups. 
There has also been research into how input features influence selection disparity~\cite{emelianov2022fair,bartik2016deleting,garg2020dropping} in a model. For example, Emelianov et al.~\cite{emelianov2022fair} show that that group-wise differences in variance over a model's feature set influence selection disparity, and show under what conditions groups with higher and lower feature variance will be under or over selected. 

%Evidence from the recent monitorship of Upstart, a finance firm which, which involved an in-depth investigation of their model in the search for less discriminatory alternatives, suggests that which features are used for prediction have a statistically significant impact on prediction disparities. 

\krdelete{\paragraph{Methods and Tools for Feature Selection}
Certainly, from a legal perspective, using race or other protected attributes in a model often leads to a violation of disparate treatment~\cite{}. }\krcomment{Disparate treatment is only relevant in certain contexts and even so I personally think leans too much into a misplaced notion of fairness along the lines of anti-classification ideas, but rather than getting into that debate here, maybe just omit the sentence?} While removing race from the model--as a feature and via proxies--may not be an effective method to achieve fairness~\cite{lipton2018does} \krcomment{probably cite our methods comparisons paper here as well?}, in situations where it is useful, Yeom et al.~\cite{yeom2018hunting} provide methods for searching for and removing discriminatory proxies in regression models, and 
%Robertson et al.~\cite{robertson2022bio} provide a method for searching for which features may be producing bias, by showing how features--and importantly, their interactions---can lead to latent encodings of protected attributes. 
Frye et al~\cite{frye2020asymmetric} introduce Asymmetric Shapley Values, a technique which can be used on a wider range of models to determine whether a feature is allowing a protected attribute to causally influence the model outcome, so that the feature can then be pruned. 
Additionally, the FlipTest technique~\cite{fliptest} also produces suggestions of which features may be the source of disparate outcomes across any two populations the user may wish to compare, without attention to causality---this may be especially helpful in narrowing down the list of features to further investigate for impacts on differences in selection rate, or simply to find statistical, and not causal, discrimination.  Finally, Belitz et al.~\cite{belitz2021automating} provide an automatic feature selection framework which only selects features which improve accuracy without reducing a user-specified notion of fairness. However, this method saw considerable drops in accuracy when selecting features in this manner. 

While there is promising work outlining how various aspects of model inputs---such as their variance and causal relationship to protected attributes---influence various notions of model fairness behavior, again there is a lack of testing these results and techniques on on-the-ground pipelines, over a variety of datasets, and also searching for feature selection impacts on a wider set of fairness-related model behavior desiderata.
%there is a large gap between the research completed and a set of ready-to-use tools which can inform model practitioners on how feature selection choices influence model behavior. 
\ebcomment{Some better concluding statement here}.

\begin{mdframed}
Tools: Automated Data Validation \textasciitilde ~\cite{breck2019data} $\cdot$ Searching Features for Proxies/Bias \textasciitilde ~\cite{yeom2018hunting,frye2020asymmetric,fliptest}
$\cdot$ Feature pruning for lowered bias amplification \textasciitilde ~\cite{leino2019feature} $\cdot$ 
Automatic Feature Selection to improve traditional fairness techniques \textasciitilde ~\cite{belitz2021automating} 
\end{mdframed}

\paragraph{Key Takeaways:}
\begin{itemize}
    \item Little work has been done exploring the impact of feature engineering and missing value imputation on model fairness, let alone operationalizing tools to help practitioners probe the impact of these decisions in their systems.
    \item Existing tools for data exploration and feature engineering do not account for fairness-related desiderata of downstream systems.
    \item A number of tools have been developed to consider the impact of feature selection on model fairness, but with little empirical testing in real-world contexts and some evidence of limited performance.
\end{itemize}

\subsection{Statistical Modeling}

\paragraph{Hypothesis Class Selection}
There is increasing work pointing out the fairness impacts of using models with increased variance~\cite{blackleave2021}, especially deep models---for example, these models can be more unstable to small perturbations in training setup~\cite{blackleave2021} leading to procedural fairness concerns about the nature of the decision process. 

\paragraph{Optimization Function Selection}
A growing number of works have pointed to degredations of fairness behavior in robust models~\cite{} and differentially private models~\cite{bagdasaryan2019differential, suriyakumar2021chasing}. 
Of course, there is also a vast body of work creating optimization functions to train models satisfy conventional fairness metrics, which we do not discuss in depth~\cite{}. 

Symmetrically, there has also been a fair amount of criticism for conventional group and individual fairness metrics imposed as top-down constraints on a system~\cite{akpinar2022sandbox,suresh2021framework}, and evidence showing that enforcing such constraints can actually degrade fairness according to those same metrics~\cite{}.
\krcomment{Could maybe also point to our tradeoffs paper, the comparison paper, and Emily's vertical equity paper as some examples of where these tools aren't well-suited to real-world use cases, such as where the decision boundary in real life is far away from the decision boundary these models tend to optimize fairness around under the hood?}

However, there is little work investigating the differences in model behavior without additional constraints, simply from changing the optimization functions used---such as Adam versus SGD in deep models, or lbfgs versus SAGA in Logistic Regression. There is preliminary evidence to suggest that differences in optimization functions do lead to differences in fairness behavior: Leino et al~\cite{leino2019feature} show that SGD over-emphasizes high-variance features, especially early on in training, which can lead to increased bias amplification. Investigating how other optimization biases impact fairness behavior may be interesting grounds for future work. 

\paragraph{Hyperparameter Search} Perrone et al~\cite{perrone2021fair} and Islam et al~\cite{islam2021can} show the promise of hyperparameter tuning towards finding fairer classification models. Islam et al~\cite{islam2021can} focus on showing that hyperparameter tuning can lead to increased fairness (differential fairness~\cite{foulds2020intersectional} and demographic parity) at no cost to accuracy. Perrone et al~\cite{perrone2021fair} introduce a technique, Fair Baysian Optimization (FBO), which is model and fairness-definition agnostic, to select hyperparameters which optimize accuracy subject to the fairness constraint. They also experimentally demonstrate that regularization parameters are the most influential for fairness performance, and that higher regularization leads to higher fairness performance in their experiments. We hope that this technique can used to understand further relationships between hyperparameter changes and fairness behaviors over a variety of different models, metrics, and deployment scenarios.

\krcomment{How are we handling the tools here? Just include a review of all the in-processing methods?}
\begin{mdframed}
Tools: ~\cite{perrone2021fair} 
\end{mdframed}

\paragraph{Key Takeaways:}
\begin{itemize}
    \item Accounting for fairness considerations in the modeling process itself is the most mature area of the FairML literature.
    \item Nevertheless, methods that have been proposed to date are generally built in the abstract and rely on assumptions that fail to translate well to real-world settings.
    \item The proliferation of these methods also pose a challenge for practitioners to navigate the many options and determine which (if any) should be considered in their setting (which may carry appreciable costs when code is either not available or only ``research'' code is available).
\end{itemize}

\subsection{Testing and Validation}

\paragraph{Validation Datasets} Several papers have discussed the perils of evaluating systems on the same benchmark data sets: this can lead to overfitting to specific data sets~\cite{deb_raji} that almost guarantees distribution shift to deployment domains, meaning that results are unrepresentative for many real-world fairness applications~\cite{sambasivan2021everyone}, and suggests that several experimental results in the fairness literature---including those related to pipeline interventions---may be incorrect~\cite{ding2021retiring,li2022data}. Other papers still have drawn attention to specific distributional problems within commonly used fairness benchmarking datasets, such as an under-represetnation of older individuals~\cite{park2021understanding}. 

%Ding et al~\cite{ding2021retiring} introduce a new suite of datasets, based on census data (a superset of the Adult dataset) for benchmarking FairML approaches. Based on this new data, they demonstrate that the effects of fairness interventions vary wildly with geography, and that common truths accepted in the community---such as increasing data size should reduce prediction disparities---do not always hold. While this is a good step, it's important for there to be large, diverse datasets in several domains (healthcare, consumer credit, insurance, education, among others), and beyond this even, to prioritize evaluating fairness approaches \emph{in the systems where where they will actually be used}. 

\paragraph{Model Selection Criteria} 
D'Amour et al.~\cite{d2020underspecification} bring attention to the problem of underspecification, where a model developer insufficiently specifies desirable deployment behavior, leading to biases and other problems during deployment. They argue that most of the model selection metrics currently used in practice---accuracy, robust accuracy, or other metrics--- on a test set insufficiently specifies desirable deployment behavior, and they demonstrate this problem in the context of several models with equivalent accuracies and robust accuracies on a test set having vastly different performance on naturally occurring 
out of distribution samples which the models came across in  deployment.
Black et al.~\cite{black2022model} describe a related phenomenon, model multiplicity, which is when there exist multiple equivalently accurate models for a given prediction task. They argue that there are multiple equally accurate models for almost all real-world prediction tasks, and show how this fact can be be leveraged to push practitioners to search for the least discriminatory model from those available with equivalent accuracy by leveraging legal pressure from the disparate impact doctrine. However, \emph{if model multiplicity is not explicitly harnessed}, it means that model evaluated on the basis of accuracy alone, the current default in machine learning, are almost certainly sub-optimally fair models even when constrained to only consider models with equivalent predictive performance.

\krcomment{Seems like the various fairness audit tools -- AI Fair 360, aequitas, etc fit in here somewhere?}

\paragraph{Key Takeaways:}
\begin{itemize}
    \item A growing body of work has illustrated how choices of validation data and model selection strategies can affect model fairness, however little of this work has been operationalized into tools or methods that can assist ML practitioners in navigating these choices.
\end{itemize}


\subsection{Deployment and Integration}

\paragraph{Accounting for Distribution Shift} A series of recent papers have introduced methods to make models invariant to distribution shift from the perspective of accuracy as well as fairness~\cite{singh2021fairness,coston2019fair,biswas2021ensuring}. Coston et al.~\cite{coston2019fair} develop two methods, one that does not require protected attributes in the training set, and one that does not require protected attributes in the deployment set. 
However, practical evaluations of these methods in deployed systems is still needed to characterize their real-world performance. Additionally, there are several open questions in this area of research: when do we want to ensure fairness criteria over data-drift, and when do we want to alert that the model practitioner that the distributional differences are so large that the model is not suitable for the deployment context?
Are there formulations of data drift were performance can be maintained through updates, but fairness cannot? When these drifts do occur what are best steps for a pracitioner to take to mitigate their impact? How do these systems perform relative to slowly-drifting distributions versus abrupt discontinuitys (such as a global pandemic or significant change in policy or practice)?
\ebcomment{Need help with further questions.}

 
\paragraph{Monitoring}
\krcomment{Would it maybe make sense to merge distribution shifts and monitoring sections? Seems like they're closely related.}
Even when using methods with guarantees on being resistant to distribution shift \textit{in situ}, it is still important for systems to monitor their fairness behavior over time. Two recent papers~\cite{albarghouthi2019fairness,ghosh2022faircanary} propose tools for fairness monitoring over time in deployment. Albarghouthi and Vinitsky~\cite{albarghouthi2019fairness} develop a technique called fairness-aware programming (implemented in Python), which allows programmers to enforce probabilistic statements over the behaviors of their functions, and get notified for violations of those statements---their framework is flexible to many behavioral desiderata even beyond fairness, and can also combine several probabilistic statements and check them simultaneously. The flexibility of the system potentially allows for a wide range of contextualized fairness desiderata to be enforced-- however, it does have limitations; for example, it cannot implement notions of fairness over individual inputs such as individual fairness. %At run time, the system continuously monitors if there is a violation of any of the desired properties and notifies the developer if so. 
Ghosh et al~\cite{ghosh2022faircanary} implement a system that measure the Quantile Demographic Drift metric at run time, a notion of fairness that can shift between group and individual conceptions of fairness based on the granularity of the bins it calculates discrepancies over. Their system also offers automatic mitigation strategies (normalizing model outputs across demographic groups) and explanation techniques to understand mechanisms of bias. Additionally, Amazon's SageMaker Clarify framework allows for the tracking of a variety of traditional fairness metrics to be monitored at runtime~\cite{}. 

However, to the author's knowledge, there is no work that address what fairness problems may come \emph{as a result} of this section of the pipeline: for example, are there examples of model updates from non-fairness aware monitoring pipelines that have degraded fairness performance? \krcomment{Fair point, but maybe a little too nuanced?}
%\ebcomment{What's the punchline here? some ideas: we need to test these on real systems, it's important to see failure modes--how intuitive are they for pracitioners to use, and how flexible *are* they for contextualized notions of fairness? Any other questions we have about the pipeline stage?}

\paragraph{Human-Computer Hand off}
Many algorithmic systems have been built with the ability to defer certain predictions to a human in the case of uncertainty~\cite{black2021selective}, assuming that including humans in decision-making systems will make them less biased. However, there are conflicting results as to whether human-in-the-loop systems out-preform models on their own when it comes to bias. Green and Chen~\cite{green2019principles,green2019disparate} show that including Mechanical Turk workers to aid algorithmic decisions consistently decreased accuracy relative to the algorithm's performance alone, and that humans in the loop also exhibited racial bias when interacting with ML predictions. However, others~\cite{cheng2022child, de2020case} have found that in the case of child welfare screenings, allowing call screen workers \emph{did} reduce disparity in the screen in rates of Black versus white children. 
Symmetrically, Jacobs et al.~\cite{jacobs2021machine} show that including machine learning recommendations in selecting antidepressants for patients did not improve clinician's treatment decision performance, and in fact, interacting with incorrect recommendations---even when supplied with explanations---lead to decreased performance. 

Taken together, as many have noted, these results show that ML decision systems which include human intervention must be tested for accuracy and bias as a whole rather than on algorithm outputs alone. These results also suggest that the efficacy of human intervention is very context-dependent. However, there little progress on how to infer when handoff problems will occur, or how to mitigate these inefficiencies. 
\marginpar{can someone add some papers that show that explanations don't really help either?} 

There has been a stream of theoretical work from the algorithmic fairness literature trying to model or guarantee fairness in a joint human-ML system~\cite{keswani2021towards,madras2018predict}. For example, Keswani et al~\cite{keswani2021towards} learn a classifier and a deferral system for low-confidence outputs, with the deferral system taking into account the biases of the humans in the loop. Donahue et al.\cite{donahue2022human} develop a theoretical framework for understanding when and when not human and machine error will complement each other, i.e. when human and machine error will occur in different areas of the distribution and cancel each other out, leading to increased performance, and suggest how this can inform the design of human-in-the-loop systems. While this initial largely theoretical work is promising, these techniques should be tested and compared on deployed systems---when do deferral systems work in practice, and can they lead to biases of their own? Do the human-in-the-loop design suggestions work in practice?



%\marginpar{Do we need to look at CHI for this?}
%Little attention has been paid to organizational integration in the fairness literature surveyed. 
%There has been some work showing that humans and machines working together can often compound errors rather than prevent them~\cite{I think some ben green stuff, maybe something from jen and hannah wallach}, but little progress on how to infer when handoff problems will occur, or how to mitigate these inefficiencies. 


\paragraph{Organizational Biases}
Organizational biases can enter an ML decision system through other means than deferring to a human in the loop. While there is evidence of the fact that organizational biases influence algorithm conception and the pipeline wholistically e.g.~\cite{passi2020making} from interview-based studies, there are is little documentation of examples of when and how this occurs and how it specifically influences predictions. Lum et al.~\cite{lum2020impact} document one such example, showing that inputs to risk assessment models, specifically, the charges that a defendant it booked for, are often over-exaggerated for Black defendants, and thus incur bias against Black defendants in model usage. (Presumably, this would happen even if the underlying model is ``fair''). \krcomment{Lum here actually seems like it might fit into the discussion of data or label biases above? What seems distinct here might be more along the lines of biases in intervention effectiveness or implementation, such as conducting outreach calls only in English or providing after school programs that can't be utilized by students that need to work or care for siblings after school, etc. However, most of these issues won't really show up in the ML literature we surveyed (more likely in the policy literature), so perhaps it would make more sense  to add a sentence or two about these broader organizational questions under the human-computer handoff heading rather than having a separate sub-section here?}

Overall, organizational integration especially lacks in \emph{measurement and mitigation} of fairness problems arising from this section of the pipeline. In addition, the literature on human-computer interaction and organizational biases do not come near understanding all of the (fairness-related) failure modes of organizational integration. For example, is just one ML system used in the decision system? Some systems in government, for example, use multiple models to inform decisions~\cite{blackIRS2022}. In these situations, how are these predictions combined, and are the models built to be used in unison? What are the impacts of rule-based decision frameworks imposed on top of algorithms predictions, such as those use in pretrial risk assessment tools\~cite{}? 

\ebcomment{It would be great to have some help pointing out what is missing here---mapping organizational frameworks, other ways of model integration into a larger decison-making framework can lead to problems.}

\paragraph{Key Takeaways:}
\begin{itemize}
    \item Recent developments in methods robust to distribution shifts seems promising but need more testing in applied settings and several questions remain for both research and practice.
    \item Monitoring and maintenance of a deployed system is just as important meeting fairness desiderata in the initial development. A growing number of monitoring tools can facilitate this process for practitioners and users of these systems.
    \item Particularly in high-stakes settings, many ML models are being used to inform human decision-making rather than acting autonomously. In these settings, it is critical to understand not only the fairness properties of the model, but those of the entire human-ML system acting together.
    \item The deployment context and specific decisions being informed by a given model also matter deeply in terms of how a model's fairness properties---as narrowly defined with respect to metrics relating to its predictions---will relate to the actual impact on people affected by the model's outputs.
\end{itemize}

\subsection{Documentation}
Several works have pointed to the need for documentation in machine learning pipelines~\cite{gebru2018datasheets, koesten2019collaborative, black2022model}. For example, Koesten et al~\cite{koesten2019collaborative} point to lack of documentation as a source of failure in collaborative data use, such as passing data sets between research groups or collaboratively creating data sets---for example, incomplete documentation may lead to a misunderstanding of data cleaning steps that took place. 
Checklists for how to document machine learning systems abound~\cite{}, but automated tools for documentation would severely decrease the load on practitioners.  While such tools are few and far between in the fairness literature, they exist in other spaces: for example, Wrangler~\cite{kandel2011wrangler} provides a method of logging data cleaning steps for review, documentation, and reproducability. However, there is a need to find such tools and convert them to include model fairness specific functionality.

\krcomment{I see why you split this out here, but it also doesn't really feel like it fits as a distinct pipeline step. Perhaps we could make it a separate sub-heading under Deployment and Integration instead? Also seems like some of the model cards stuff would fit here:

\url{https://dl.acm.org/doi/pdf/10.1145/3287560.3287596?casa_token=DyLeBck72WgAAAAA:E3xvjZ4p5tM629YLYCQqq3HVB29HCQMaC_7Ua41FxXbAFOnCqn1nfvsAfRtUWVKp2pYWghkjMV7IGzo}

\url{https://dl.acm.org/doi/pdf/10.1145/3531146.3533108?casa_token=Dv5l8KuMpbQAAAAA:IAXd1Z1dM1vDuzRxzn1XPkOIEEJz3v0pWcniqMfz8g693eApvA7Vlc7wmQYgC2E2SrAaA6vWxbrkWgk}
}

\paragraph{Key Takeaways:}
\begin{itemize}
    \item Several papers have called for better documentation of models and datasets, both for research and practice, and various proposals have been made for more standardized formats. However, these efforts would be assisted by adapting some of the tools and automation that exist in other spaces to lower the barriers to developing good documentation in the ML space.
\end{itemize}
 
 %Koesten et al~\cite{koesten2019collaborative} point to sources of failure in collaborative data use, such as passing data sets between research groups or collaboratively creating data sets---for example, one failure mode they point to is having an incomplete understanding of data cleaning steps that took place before working on a dataset created by another group. They point to user needs of such collaborative data pipelines, such as open channels of communication and version control, but do not create tools to operationalize these needs. 


% \subsection{Consideration of the total pipeline}
% %One notable recent work by Donahue et al.\cite{donahue2022human} develops a theoretical framework for understanding when and when not human and machine error will complement each other, i.e. 

% \ebcomment{Help finding works and tools that consider the entire pipeline at once?}

% \krcomment{I don't think there's really a lot out there---certainly this is the gap that the sandbox toolkit is seeking to fill in part. Likewise, our method comparison paper looked at pre-, post-, and in-processing methods separately, but didn't attempt to consider their interactive effects. I'd probably suggest removing the heading here and commenting on the need for more research in this direction as a major element of the research agenda (while noting that operationalization of the different components would also make this a lot more tractable)}



\input{survey_table.tex}
%\input{survey_table_simple.tex}


==> versions/survey_table_simple.tex <==
\begin{table}[]
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
\begin{tabular}[c]{@{}l@{}}Problem\\ Formulation\end{tabular} & \begin{tabular}[c]{@{}l@{}}Data \\ Choice\end{tabular} & \begin{tabular}[c]{@{}l@{}}Feature\\ Engineering\end{tabular} & Statistical Modeling & \begin{tabular}[c]{@{}l@{}}Testing and\\ Validation\end{tabular} & Evaluation & \begin{tabular}[c]{@{}l@{}}Organizational\\ Integration\end{tabular} \\\hline 
 \citep{black2022algorithmic}, \cite{obermeyer2019dissecting}, \cite{kilby2021algorithmic}, \cite{jacobs2021measurement}, \cite{coston2022validity} , \cite{passi2019problem}  &     \cite{wang2021fair} , \cite{bias_in_word_embeddings}, \cite{buolamwini2018gender}, \cite{marda2020data}      &  \cite{khani2021removing}, \cite{leino2018featurewise}, \cite{garg2021standardized}     &  \cite{blackleave2021} \cite{marx2019}, \cite{jones2020selective}        &           &   \cite{d2020underspecification}         &           \cite{lum2020impact}                                                          
\end{tabular}
\end{table}
